SoK: Machine Learning Governance

The application of machine learning (ML) in computer systems introduces not only many benefits but also risks to society. In this paper, we develop the concept of ML governance to balance such benefits and risks, with the aim of achieving responsible applications of ML. Our approach first systematizes research towards ascertaining ownership of data and models, thus fostering a notion of identity specific to ML systems. Building on this foundation, we use identities to hold principals accountable for failures of ML systems through both attribution and auditing. To increase trust in ML systems, we then survey techniques for developing assurance, i.e., confidence that the system meets its security requirements and does not exhibit certain known failures. This leads us to highlight the need for techniques that allow a model owner to manage the life cycle of their system, e.g., to patch or retire their ML system. Put altogether, our systematization of knowledge standardizes the interactions between principals involved in the deployment of ML throughout its life cycle. We highlight opportunities for future work, e.g., to formalize the resulting game between ML principals.

==> Model%20Governance%20SoK%20draft/Contents/0_abstract.tex <==
\begin{abstract}
The application of machine learning (ML) in computer systems introduces not only many benefits but also risks to society. In this paper, we develop the concept of ML governance to balance such benefits and risks, with the aim of achieving responsible applications of ML. Our approach first systematizes research towards ascertaining ownership of data and models, thus fostering a notion of \textit{identity} specific to ML systems. Building on this foundation, we use identities to hold principals \textit{accountable} for failures of ML systems through both attribution and auditing. To  increase trust in  ML systems, we then survey techniques for developing \textit{assurance}, \ie confidence that the system meets its security requirements and does not exhibit certain known failures. This leads us to highlight the need for techniques that allow a model owner to manage the \textit{life cycle} of their system, \eg to patch or retire their ML system. Put altogether, our systematization of knowledge standardizes the interactions between principals involved in the deployment of ML throughout its life cycle. We highlight opportunities for future work, \eg to formalize the resulting game between ML principals. 
\end{abstract}

==> Model%20Governance%20SoK%20draft/Contents/1_intro.tex <==
\section{Introduction}

Like any maturing technology, machine learning (ML) is transitioning from a stage of unfettered innovation to increasing calls to mitigate the risks associated with its deployment. In the context of ML systems, these potential risks include privacy violations (\eg leaking sensitive training data), unfair predictions (\eg in facial recognition), misinformation (\eg generative models facilitating the creation of deepfakes), or a lack of integrity (\eg self-driving car accidents due to an incorrect understanding of their environment). At the societal level, there is a need to ensure that applications of ML balance these risks with the benefits brought by their improved predictive capabilities, just as practical systems security balances  the cost of protection with the risk of loss~\cite{lampson2004computer}. 

\textit{Machine learning governance} standardizes the interactions between principals involved in the deployment of ML with the aim of ensuring a responsible application of ML, \ie one that is beneficial to society.%\todo{cost benefit analysis and risk analysis in bisop p17}

Governance in ML differs from existing research in several ways. Indeed, the attack surface of ML algorithms has been the subject of many studies; for instance, work on adversarial ML~\cite{huang2011adversarial} evaluated the worst-case performance of ML under various threat models. However, this line of work often focuses on narrow aspects, such as the technical limitations of ML algorithms, and studies these limitations in isolation. For instance, while it is known how to train a model privately~\cite{chaudhuri2011differentially,abadi2016deep}, the impact of private learning on model robustness is less studied~\cite{song2019privacy} thus affecting our ability to deploy such algorithms in settings where the model must be aligned with multiple social norms. % and the associated worst-case performance guarantees need to be provided for the model predictions to be correct. 
%This multi-faceted perspective is required even in settings such as healthcare where an adversary may not be present~\cite{suriyakumar2021chasing}. 
It, thus, remains unclear how companies and institutions applying ML should manage the different risks associated with ML. This is exacerbated in the online setting where a model is not static but rather iteratively trained and deployed. %: reasoning about  risk across the lifecycle of a model is challenging. 
These difficulties have also manifested themselves in inadequate regulation, as illustrated by the focus on anonymization in privacy regulation~\cite{cummings2018role} despite its well-known limitations~\cite{narayanan2008robust}. As a result, regulators are unable to formalize, implement, and enforce regulation that contains the societal risks of ML.

In this paper, we systematize knowledge from security and privacy research on ML to outline a practical approach to ML governance. Our approach is four-fold and can be thought of as defining the types of interactions that principals (defined in  \S~\ref{sec:principals}) of an ML ecosystem will require to develop the trust needed to ensure responsible applications of ML.  While existing research on adversarial ML (and more broadly trustworthy ML) serves as a foundation for some of the approaches, our systematization identifies open problems which the computer security community needs to tackle. 

First, we observe that trust requires that one make unforgeable and undeniable claims of ownership about an ML model and its training data. This establishes the concept of \textit{identity}, which identifies a key principal in the ML application: its owner. This is a prerequisite to holding model developers accountable for the potential negative consequences of their ML algorithms: if one is unable to prove that a model belongs to a certain entity, it will be impossible to hold the entity accountable for the model's limitations. 

Once ownership of the model is established, the second component of our approach to ML governance is \textit{accountability}. Here, we attribute model failures to the model owner and its end users, and establish the responsibility of these different principals for failures of the model. These failures may have been identified through the use of the system, but could also result from external scrutiny by entities such as regulators. We thus also discuss how to audit an ML application to identify and attribute failures that have yet to be discovered. 

To prevent failures in their ML application, and to foster trust from end users, model owners will then deploy a set of techniques to obtain \textit{assurance}. Loosely defined, these techniques establish confidence that the system meets specific requirements. The model owner here wishes to make certain claims establishing guarantees of controlled risk for their ML application. While these claims are currently often made post-hoc, by inspecting the trained model, we argue that future research should focus on the training algorithm. We discuss ways that these claims can be substantiated by, for instance, proactively collecting evidence during training  or providing documentation to end users. 

Finally, the fourth component of our approach realizes that the trade-off between ML risks and benefits will be regularly re-evaluated by the different principals involved. As such, we outline how there will be a need for mechanisms that allow one to dynamically edit models after they were released: this lifecycle management is analogous to common practices in software development like versioning. This represents challenges in how one can remove behavior already learned by a model (\ie machine unlearn) and learn new behaviors, but also retire the model altogether.

These interactions between model owners, users, and regulators are at the core of our approach to ML governance and result in a formal formulation of what it means to balance the risks of applying ML (see \S~\ref{sec:game}). Concretely, we present a Stackelberg game among the principals involved in an ML governance scenario. The approach is more general, and can capture competing interests of the principals as well as the possible trade-offs, thus delineating the Pareto frontier. 

To summarize, our contributions are the following: 
\begin{itemize}
    \item We define the problem of ML governance as balancing the risks of ML with its benefits. Specifically, ML governance supposes that society has defined norms that serve as the basis for characterizing trade-offs between risks and benefits. We formalize the interactions between ML principals: \ie model owners making claims of having managed certain risks (\eg privacy, fairness, robustness, etc.), end user who seek to trust these claims, and regulators who seek to audit such claims and verify compliance.
    \item We systematize approaches to establishing identity in ML through data and model ownership in \S~\ref{sec:ownership}. This serves as the foundation for holding model owners and other ML principals accountable for failures of ML in \S~\ref{sec:accountability}, through a combination of techniques for attribution and auditing.
    \item We systematize research on techniques for assurance, \ie proactively building confidence that an ML system meets specific security requirements.
    \item We outline the need for mechanisms that manage models throughout their lifecycle, \eg enabling model owners to version usefully. We show how current efforts on machine unlearning provide a {\em partial yet incomplete} response to this need, and that a more comprehensive approach is needed to develop the ability to patch ML systems.
\end{itemize}

We recognize that developing solutions for ML governance is not purely a technical problem because many of the trade-offs that need to be characterized involve a societal component. Given the intended readership of this paper, we put an emphasis on how computer science research can contribute  mechanisms for ML governance, but this assumes that the design of these mechanisms will be informed by societal needs.
Put another way, this SoK leads us to identify opportunities for collaboration with communities beyond computer science, \ie opportunities for interactions that inform the goals of computer science research, but also that would help increase adoption of technical concepts beyond computer science. We thus hope that our manuscript will be of interest to readers beyond the computer security and ML communities.



==> Model%20Governance%20SoK%20draft/Contents/2_background.tex <==
\section{Background}



\subsection{Machine Learning Primer}

% \todo{if there is a space shortage, we can purge here}

In this paper, we focus on the supervised learning problem in machine learning. We are given a dataset $D = \{(\mathbf{x}_i,\mathbf{y}_i)\}_{i \in [n]}$ of inputs $\mathbf{x}_i$ and labels $\mathbf{y}_i$ (encoded as one-hot vectors) and wish to learn a function $\model$ that can map the inputs $\mathbf{x}_i$ to $\mathbf{y}_i$. For a given task we associate a loss function $\mathcal{L}$ which characterizes the error of a given function $\model$ in predicting the labels of the dataset. A common choice (for classification tasks) for the loss function is cross-entropy, defined as:  
\begin{equation}
\label{eq:cross-entropy}
\centering
\mathcal{L}_{CE}=-\mathbf{y}_i\ln(\model(\mathbf{x}_i))
\end{equation}

The function $\model$, or model, is typically represented as a parameterized function whose parameters, the weights, ideally minimize the loss function $\mathcal{L}$ on dataset $D$. In practice, when a closed-form solution cannot be found, the main process of finding a low error model is done by iteratively tuning weights $\weights$ that parameter the model $\model_{\weights}$ via gradient descent. We typically add a further level of stochasticity to the optimization process by applying the update rule with respect to the loss computed on a batch of data $(\hat{\mathbf{x}},\mathbf{y})$ which is randomly sampled from the dataset $D$. To be specific the update rule is given by:
\begin{equation*}
\weights_{t+1} = \weights_t - \eta \frac{\partial \mathcal{L}}{\partial \weights}|_{\weights_t,\hat{\mathbf{x}}_t}
\end{equation*}
where $\eta$ is a hyper-parameter one tunes.

Once the model is trained, it is deployed to make predictions on points it has not seen during training. To evaluate how well a model will \textit{generalize} to these new points, one typically retains a holdout set of labeled data points to measure the performance of the model upon completing its training. 

\subsection{Operational Life-cycle}
\label{ssec:lifecycle}

% \todo{if there's a space shortage, we can purge here}

Machine learning models have a life cycle. They are trained on collected (or generated data) that is processed and optimized to perform a task which often involves recognizing a pattern in the collected data (training). The model is then used to perform the \textit{learned} task on new data, that is, to infer the said patterns in never-before-seen data. At the high level, we can distinguish 3 operational life-cycle steps which can be further subdivided into smaller steps.

\begin{description}
\item[\textbf{Data preparation 1/2: Collection.}] This is the step that gathers data: complexity and governance difficulties in this process may stem from legal, technical (which data to collect is hard to define), or business issues (there is no incentive to collect that data).
\item[\textbf{Data preparation 2/2: Cleaning.}] Here we  transform a dataset $D$ which has been collected into a dataset $D'$ which is amenable to ML methods. This includes removing data that was improperly collected or performing preliminary feature engineering.
\item[\textbf{Model development 1/2: Training.}] This step represents work done by  experts to design a model architecture, configure its training algorithm, and learn model parameters. From a governance point of view, this step is hard to investigate because it either relies on expert insight or on (deep) learning algorithms often  black-box in nature.
\item[\textbf{Model development 2/2: Testing.}] The model is evaluated with a set of metrics estimated on a holdout set of data before the model is confronted with current production data. This evaluation typically assumes that holdout from the same distribution than training data is available.
% \item[\textbf{Model deployment 1/3: Model conversion}] This is the transformation of a model from a Data scientist model (in python) to a production ready fast to infer model (in a compiled language like C++). This currently relies heavily on ad-hoc conversion formats like ONNX, torchserve etc these have not been investigated for safety/security and adversarial manipulation/accidental maleability.
\item[\textbf{Model deployment 1/2: Model Serving.}] The model is deployed at scale, often using a different software framework than the one used to train it. Much of our discussion on governance focuses on mitigating risks that manifest themselves through failures at this stage.
\item[\textbf{Model deployment 2/2: Model Retirement.}] This step carries important consequences for governance despite being often omitted. We will discuss how to maintain multiple versions of a model, and what the implications are for choosing to retire (or not) a model. 
%This step is most often forgotten but would be extremely important in a practical setting. What happens when you go from version 1.0 of a model to 1.1? Do you keep a version of the model and all of the data for auditing and revisiting purpose. From an academic perspective the question that is raised is monotonicity of models one over another. For instance, over the multiple iterations of model development the models should not say that a user is credit worthy then not and then credit worthy again. Existing models should be kept to assert this unless there is monotonicity guarantees.
\end{description}



% \begin{figure*}
%     \centering
%     \input{Contents/Figures/life_cycles.tikz}
%     \caption{Model Life Cycles 
%     % \nicolas{model and data retention for the last step?} \mohammad{Done}
%     }
%     \label{fig:life-cycles}
% \end{figure*}



% \pgfplotstableread[col sep=comma]{
% 	a,b,c
% 	1,1,[1] \emptycirc
% 	2,2,[2] \halfcirc
% 	3,3,[3] \fullcirc
% 	4,4,[4]
% 	5,5,[5]
% }\data

% \begin{figure*}
%     \centering
%     % \input{Contents/Figures/tax.tikz}
%     \input{Contents/Figures/table.tex}
%     \caption{Taxonomy}
%     \label{fig:tax}
% \end{figure*}

% \todo{For the Figure @Adelin recommends mentioning as a footnote how \cite{dowlin2016cryptonets} (homomorphic encryption) and \cite{jia2021proof} (POL) both require collaboration between parties, which isn't always the case in most of the examples seen}


==> Model%20Governance%20SoK%20draft/Contents/3_governance_def.tex <==
% \newpage
\section{Defining ML Governance}

% \url{https://medium.com/data-science-at-microsoft/machine-learning-model-governance-at-scale-26c9a2dc15b5}

% \mohammad{discussed this with Varun. ML governance is a quite well-studied operations management concept in the industry with several well-established systems (usually under the name of data mining). While this is likely not the angle we want to define our take on the problem; we have to consider at least one (generic) such system and point out that our life cycle fits within those systems reasonably well. It could be IBM's \href{https://en.wikipedia.org/wiki/Cross-industry_standard_process_for_data_mining}{standard}.}

% \nicolas{somewhere in here we should discuss assumptions about trust see p11 bishop}


%\subsection{Definition}
\subsection{Overview}

Conceptually, ML governance can be thought of as a set of solutions for balancing the benefits of applying ML with the risks it creates, often at the level of society. Governance is a prerequisite to build trust between principals involved and affected by an ML development. We describe such principals in detail in \S~\ref{sec:principals}, but for now it is useful to assume that they are three types of principals: the model owner (\ie the company or institution creating and deploying the model), the end user, and a regulator. Governance imposes constraints on how principals interact throughout the lifecycle of an ML application (as covered previously in \S~\ref{ssec:lifecycle}). 

The benefits of an ML pipeline are often application-specific. Typically, these benefits are defined by or at least motivate the model owner, \eg applying ML will generate profit for a company. 
%Every model owner would like to maximize their model performance w.r.t. a given metric, such as accuracy. 
One may think that the model's usefulness (\ie utility) is tied to a performance metric (\eg accuracy) and every other consideration can only decrease it. This is true if we view training as an optimization problem; having additional constraints limits the feasibility set. From an asymptotic\footnote{Given the training dynamics, the constraints may direct the search accurately and improve the solution found as done in LASSO~\cite{tibshirani1996regression}.} statistical learning perspective, any constrained problem can produce an objective that is at most as good as the unconstrained problem.
However, other considerations may be just as important as utility---in particular at steps of the life cycle before or after training. 
%For instance, consider labeling of images which is a well-studied supervised learning task where state-of-the-art models have long surpassed human-level accuracy\adelin{citation missing}. However,  these models often fail to \textit{generalize} when they are deployed in the real world~\cite{}. For instance, their decisions may not be robust to imperceptible changes to the input (\eg a perturbation which does not affect the semantics of the input can completely change a model's decision~\cite{}); or they may leak information about their training sets (\eg presence of a particular individual in the training set). Furthermore, 
For instance, model decisions may demonstrate significant unwanted biases (\eg misclassifying individuals from minorities) and prompt the model owner to reassess their data collection and algorithmic choices. Thus, deploying ML comes with inherent \textbf{risks} to the different principals interacting with the ML pipeline:
%Seen through the lens of risks, the utility of the model (or lack thereof) can also be seen as a risk.\adelin{That last sentence is not understandable. Do you mean that robustness should not come at the cost of baseline accuracy?} 
% Instead, the risks associated with ML are defined more widely by all actors: 
users may have concerns with models analyzing their data, regulators may seek to limit potential harm to society  (\eg limit unfair predictions). We detail these risks in \S~\ref{ssec:risks}.

These varied risks, however, do not carry equal meaning and urgency for all principals involved in creating, using, and regulating these models. Because risk definition is inherently tied to a given principal, \textit{\eg} due to their own goals and incentives, and various principal definitions may come into conflict with one another, model governance is best formalized as a \textit{game}. Each principal participating in the game is optimizing for their own set of constrained objectives at any point in time, which improves the principal's trust in the ML pipeline and its other principals. The metrics underlying these objectives may differ from accuracy, and may be worst-case in nature. Thus, many established practices for evaluating ML fall short of providing the guarantees necessary for ML governance. 


\subsection{Principals, Incentives, and Capabilities}
\label{sec:principals}

Defining governance requires understanding the various principals in the ecosystem and their capabilities and incentives. We begin enumerating them below. In certain settings these principals may not always be separate entities---a data collector could also be the model builder---in which case such a principal may assume multiple of the roles defined below. % in the meaning common to the role-based access control literature.

\begin{enumerate}
\itemsep0em
\item {\bf End User:} This principal is using a system deploying ML. It may be a customer of a company, a patient at a hospital, a citizen asking for government benefits, etc.
\item {\bf Model Owner:} This principal is one with a particular task that can be solved using ML. They communicate their requirements to the model builders, and clearly specifies how this trained model can be accessed (and by whom). 
\item {\bf Model Builder:} This principal is responsible for interpreting the model owner's requirements and designing an ML solution for them. To do so, the builder requires access to representative data from the domain (see data collector below), and an appropriate choice of training algorithm (and approach). The model builder or model owner will then be responsible for deployment.
\item {\bf Data Collector:} This principal is responsible for sourcing the data as per the model owner and builder's requirements so as to ensure that the learnt model performs well and complies with various characteristics (such as ensuring data privacy etc.). 
\item {\bf Adversaries:} The adversary is any entity that wishes to disrupt any phase of the ML life cycle. They may have varying control and access over the ML system. % including insider adversaries. \varun{i can't recall any part of the paper that uses this insider adversary model.}\mohammad{dataset inference does consider such adversaries. I don't think we go into such details in that section though}
\item {\bf Trusted Arbitrator:} This principal is required in situations where (i) auditing of services provided is required (\eg a legal agency or a mandated organization verifying if deployed models are compliant with GDPR), or (ii) there is a requirement for arbitration between two principals (in situations related to ownership resolution). We also refer to this principal as the \textit{regulator}.\footnote{For simplicity, we conflate the entity providing the regulation or standard and the enforcement entity when they in practice differ.}
\end{enumerate}


%In some situations, the data collector and model builder may both refer to the same  entity (\eg a company may collect data and train the model). Conversely, it is also possible that  responsibilities are split across subprincipals: a model builder may separate ML model development from deployment.


\input{Contents/themes}




\subsection{The Governance Games}
\label{sec:game}
\begin{figure*}
    \centering
    \includegraphics[width=0.6\textwidth]{Contents/Figures/game.pdf}
    %\input{Contents/Figures/game_flat2.pdf}
    %\input{Contents/Figures/game.tikz}
    \caption{Regulated Model Commission Game in Extensive Form---Strategy sets may be continuous (arcs) or discrete (branches). The dashed line indicates non-singleton information sets: the two decision points of model builder 1 are indistinguishable from model builder 2. The game may be repeated (dots). For brevity, we do not indicate decision spaces of most principals or their pay-offs. 
    }
    \vspace{-5mm}
    \label{fig:game}
\end{figure*}



ML governance follows from the interaction of the principals (\S~\ref{sec:principals}) who are independent decision-makers with goals that may or may not align with each other. For instance, a model owner's desire of achieving robustness may exacerbate leakage of an end user's private information~\cite{song2019membership,song2019privacy} because adversarial training encourages the model to generate predictions that are especially stable for data points that are close to ones in the training set.  We can thus see ML governance as a multi-agent system and analyze dynamics between the principals using standard tools from game theory\cite{shoham_multiagent_2009}. Solutions to this game  affect the degree of trust among principals and towards the application of ML itself. In many governance scenarios, principals act sequentially, after they perceive the effects of other principals' decisions. This naturally leads to a leader-follower, or \textit{Stackelberg} competition structure~\cite{fudenberg_game_1991}.
 
\subsubsection{Stackelberg formulation of learning problems}
\label{subsub:performative}

Work using Stackelberg competitions considers the strategic behavior of a principal (the follower) whose objective is distinct from that of the leader. This improves over the \textit{adversarial assumption} of works that use a zero-sum game formulation (\ie Yao's principle~\cite{yao_principle}) which requires that the follower's objective be exactly the opposite of the leader's. 
The most relevant application of Stackelberg competitions to our discussion is found in strategic classification~\cite{hardt_strategic_2016}. There, the subjects of algorithmic classification are strategic. After observing the decision made, these subjects can adjust their features to achieve a better classification outcome. This is also an example of classification having {\em performative qualities}~\cite{perdomo_performative_2021}: participants adjusting their features causes a distribution shift, which in turn means that the future predictions of the model may be neither fair or optimal w.r.t. the new distribution. In practice, this requires model maintainers to re-train, or employ an online learning setup to preserve their model's integrity and fairness.

%% This is directly relevant to model governance \varun{when you say "this" -- do you refer to the prior sentence or the one that follows?}\mohammad{the prior sentence should go; it's been edited to the degree of triviality}:

Using a similar Stackelberg competition, Perdomo \etal~\cite{perdomo_performative_2021} propose an equilibrium notion called {\em performative stability}. Models that are performative stable produce predictions that would remain optimal under the distribution shifts that result from their own predictions. Similarly, Br\"uckner~\etal~\cite{bruckner_stackelberg_2011} consider spam filtering and analyze an adversarial prediction game between a learner (leader) who tries to classify spam and an adversary (follower) that observes the learner's decisions with the goal of producing less detectable spam.

%Stackelberg formulations of learning have also been used in model-based reinforcement learning~\cite{rajeswaran20a} between a \textit{policy player} maximizing rewards under the learned model and a \textit{model player} that fits the real-world data collected by the policy player. An interesting application of this to governance may be to model the interactions between the data collector and model builder as policy and model players, respectively.%\todo{Mohammad I removed a sentence after here which I think is not needed} %Tsirtsis~\etal~\cite{tsirtsis2020decisions} study the joint problem of a finding a performant prediction model (or policy) and counter-factual explanations under the assumption that decision subjects are potentially strategic who would try to improve their chances of receiving a beneficial decision.
% \mohammad{Add explanation}\cite{raghunathan2018certified}

\subsubsection{Beyond two-player competitions}
As useful as Stackelberg games are, they only cover a subset of interactions that principals may have with each other as part of an ML governance scenario. 
% How should we model scenarios that involve multiple principals (an end-user that takes a model owner to arbitration over privacy violations) or those that run over a (possibly undermined) course of time (a model maintainer that has to patch his model to accommodate new reagultaions)? What would happen if a subset of principals could not observe each other actions? (Model Builders engaged in a bidding competition)
In other scenarios,  several principals may be deciding without observing their opponent actions. For example, a model owner may be unaware of possible future regulatory efforts, an end user may modify its trust assumptions about using ML services, multiple model builder contractors could enter bidding competitions to train a model, etc. This requires a strategic-form game usually captured in the form of a pay-off table~\cite{fudenberg_game_1991}.


However, such a table may be difficult to assemble because interactions can be repeating over time in several stages: principals' expected risks and pay-offs should be adjusted with the perceived effects of their decisions in the future. In such cases, an {\em extensive-form} game which can be represented as a decision tree can capture multi-stage games with observed actions; it shows {(i)} the set of principals, {(ii)} the order of their decisions, {(iii)} their choices at their respective decision points, aka \textit{strategy sets}; {(iv)} their pay-off (or cost) as a function of their own choice as well as the history of the choices made prior to it, {(v)} \textit{information sets}: the information available to each principal at any decision point, and finally {(vi)} the probability distribution over any exogenous event~\cite{fudenberg_game_1991}. 

We believe extensive-form games are a promising avenue to formalize interactions between principals and develop ML governance in a principled way. Figure~\ref{fig:game} illustrates this with a hypothetical ML governance scenario. The regulator would like to ensure fairness and privacy guarantees so it requires that a (pure) DP~\cite{dwork_algorithmic_2013} mechanism be used with a budget of $\varepsilon < 10$. For fairness, the regulator requires demographic parity~\cite{fairml} with at most $\gamma < 10\%$ disparity between sub-populations. The model owner can choose its own specifications for $\varepsilon$ and $\gamma$ and commission two model builders to produce the models. Model builders are now in a bidding competition to achieve the most performant model within specification. They may choose different architectures, source their data from various data collectors (not shown in the figure for brevity), etc. In particular, they get to choose how they allocate their \textit{privacy budget} between these different steps of the ML life cycle~\cite{mironov_renyi_2017}. We note that model builder 2 \textit{does not} observe its rival's decision (hence the non-singleton information set of builder 1 is annotated with dots). Therefore, the sub-game between the two builders is a strategic-form game played simultaneously between the two as no one goes first. Finally, the model owner accepts one model and rejects the other. Model builder pay-offs are assigned at this stage. Next, the regulator can verify achieved fairness and privacy guarantees, and issue proportional fines/incentives for the model owner if they are within specification, or even improve upon it. For instance, privacy-minded regulators could devise fines that scale with the gap between the achieved $\varepsilon$ in practice and the regulatory specified one; or a fairness regulator may propose tax breaks for model owners who have achieved a certifiably fairer prediction model. Since the game is repeated, the regulator can learn from the history of the game and update the regulation (if necessary) for the next stage of the game. 
 
%  Game theoretic formulation of learning problems are common in the ML literature~\cite{gan_goodfellow}\mohammad{@varun, others, can you put some adversarial learning papers here}, but they are mostly formulated as zero-sum games, or equivalently the general min-max ruleknown as Yao's pricniple~\cite{yao_principle}.
\subsubsection{Solution Concepts} 
%As with all games, finding the equilibria of governance games is often the focus of the analysis. This is because under an equilibrium, all principals involved in a game are choosing their optimal strategy w.r.t. each other. They are playing their \textit{best response}. %\varun{would scrap last sentence as the same info is conveyed in the sentence prior}\mohammad{`best response' is a particular notion in game theory. I would keep it to ground the discussion.}
% \noindent{\textbf{Solution concepts for extensive-form games}}
%  \begin {itemize}
%      \item existence of equilibria (equivalance between extensive and strategic form games)
%      \item multi-leader-follower works
%      \item class of correlated equilibria (recent work from deep mind)
%      \item Integrating the game formulation in the model optimizations (Fei Fangs works)
%  \end{itemize}
% Classically solving a game entails finding and analyzing its Nash equilibria. 

Calculating Nash equilibria is an NP-hard problem~\cite{nash_complexity}. As a result, most classical solution concepts for extensive-form games make simplifying assumptions which limit their applicability to governance games. These include {(i)} assuming sub-game perfect equilibria, {(ii)} amenability to backward induction, or {(iii)} agents adopting behavioral strategies~\cite{fudenberg_game_1991}. 
While computing exact strategies may be intractable in the presence of multiple principals or continuous strategy sets, or when the interaction are recurring across a time horizon~\cite{hu_multi-leader-follower_2015, pang_quasi-variational_2005};
% \varun{previous sentence does not explain why intractability is a problem?}
% \mohammad{Do we have to explain why intractability is a problem? It complicates analysis; make synthesis impossible.}
% \varun{"\eg with multiple principals, a continuous strategy set or across a time horizon---all of which are present in our example in Figure~\ref{fig:game}" $\implies$ has nothing to do with intractability, but starts with "for example:"}
% \mohammad{should be good now}
approximations such as correlated equilibria (a superset of Nash equilibria)~\cite{fudenberg_game_1991} are easier to find by iterative mechanisms, and have recently seen a flurry of research for their efficient calculation even in the presence of multiple principles and across a time horizon~\cite{meila_multiagent_2021}.

Furthermore, in many realistic scenarios principals may have incomplete information about the game (known as Bayesian games~\cite{fudenberg_game_1991}). For example, in Figure~\ref{fig:game}, model builders may not know the technologies (and therefore, the fairness/privacy guarantees) that their rival is able to achieve. 

%\varun{are extensive form games a super "class" of these other games?}\mohammad{yes, they are}
 
Recently, new solution concepts have been introduced~\cite{li_solving_2021, fiez20a_implicitlearning, li_endtoend_2020} that tackle these challenges by combining ML with established techniques such as backward induction. 

%  \subsubsection{Future directions}
\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=0.5pt,bottom=0.5pt]
\noindent{\textbf{Call to action:}} As discussed in the introduction, research on the limitations of ML often considers a single class of risk. When the interplay between risks is considered, two classes of risk are isolated to study their interplay and integrity is often one of them. For instance, the  ML community has recently started to realize the importance of considering strategic decision makers and subjects which has led to new and practical definitions of robustness\cite{perdomo_performative_2021}. The security community has also long depended on game theoretical studies of potential adversaries~\cite{gametheory_security}. We posit that it is time for the research community to discover the more complex interplay of a realistic governance scenario with {(i)} multiple principals, {(ii)} independent pay-offs and objective functions, {(iii)} allowing for possibly imperfect information. We believe such a multi-faceted approach would alleviate issues that have plagued single-objective approaches, such as choosing hyper-parameter values for parametric definitions of privacy or fairness.
\end{tcolorbox}
\vspace{-3mm}

%  \begin{itemize} 
%  \item multi-metric multi-agent consideration
%  \item What would happen in the absence of complete information \cite{roth_watch_and_learn_2016}
%  \item natural answer to the question of how to choose values for parametric metrics
% \end{itemize}
 
% \subsection{Our Approach}

% \varun{scrap fully} 

% Having defined ML, its principals, and their interactions, we now turn to our solutions for ML governance. In the rest of the paper, we describe how identity resolution through ownership (\S~\ref{sec:ownership}) enables accountability in ML through attribution and auditing (\S~\ref{sec:accountability}). We then survey techniques that foster confidence in the ML system’s ability to mitigate risk, thus obtaining assurance (\S~\ref{sec:assurance}). In the interest of space, we only cover the risks introduced earlier but we expect our discussion to be relevant to other risks. The last component of our approach to ML governance manages the life cycle of models by patching and retiring them (\S~\ref{sec:life-cycle-management}).


==> Model%20Governance%20SoK%20draft/Contents/4_ownership.tex <==
% \newpage
\section{Establishing Identity in ML Systems}
\label{sec:ownership}

% \anvith{Rough idea for a possible call to action here (maybe can tone down from cars driving into dogs, but I guess it's better than driving into babies: "When a self-driving car is found to purposefully drive into dogs on the side of the road, and it was later discovered that the training dataset was poisoned to cause such a terrible thing, who do we blame? Who owns the dataset? To answer such a question we would first need to understand exactly what principals are responsible for the model and dataset, \ie define identity and ownership (both of which have technical computer science pedigrees)."}


The notion of \textit{identity} is fundamental to computer security~\cite{bishop}. Developing the notion of identities involves first recognizing which principals are involved in a system and second how they interact with this system as it takes actions over objects. Thus, identities are a prerequisite to holding principals accountable for failures of the system (\eg who should be held responsible for the failures of an ML model deployed by a self-driving car?).

Similar to other systems, those that incorporate ML need to integrate access control mechanisms to ensure that principals are authorized to interact with the system. %the point of this was to say that access control is a prerequisite, and then we need some new stuff on top of it - Nicolas \varun{we say this (access control) but never build upon it}\nick{how about change to "...those that incorporate ML need to establish the concept of identity which can enable accountability."?} 
We identified a number of principals in \S~\ref{sec:principals}.  For instance, an end user may need to 
authenticate themselves before they are allowed to query an MLaaS API, just like authentication could be necessary to query a database. However, because ML systems introduce new, often implicit, information flows between data and models, they call for specific mechanisms.

In particular, we focus on three areas of interest: the training data, the test data, and the learned model. In the following subsections, we define {\em ownership} as the process of associating a principal with these key components of an ML system. Later, in \S~\ref{sec:accountability}, we focus on how we can hold principals accountable for model failures once identities relevant to data and models have been clearly established through the process of ownership resolution.

\subsection{Data Ownership} 
\label{subsec:data_ownership}


Data is one of the foundational pillars of a {\em functional} ML model, both at training and inference (test) time. 

\vspace{0.5mm}
\noindent{\bf Training Data:} During learning, the training data is used to compute the objective function being optimized to find the model's parameters (recall Equation~\ref{eq:cross-entropy}). Since the existence of training data is a prerequisite to obtaining a model, the entity owning the training data plays an integral role in the governance of the ML system. 

% \nicolas{add citations throughout this paragraph enumeration of questions}
% \nicolas{this paragraph feels like it is defining accountability for data owners - might be worth moving to a new subsection in the accoutnability section which follows this discussion of identity}

Specifically, understanding who collected the data can enable answering various questions regarding (i) {\em representativeness:} if the collector paid attention to ensure that the data collected is not stagnant and captures effects such as domain/concept shifts (where applicable)~\cite{gama2014survey}, (ii) {\em data cleanliness:} if the data is processed for usage, and sanitization techniques (such as the use of robust statistics) are applied~\cite{diakonikolas2019recent}, (where applicable, especially for detecting poisons~\cite{biggio2012poisoning}), (iii) {\em fairness:} if the data collected is representative of the downstream task and various subgroups (as specified by the model owner of \S~\ref{sec:principals})~\cite{holstein2019improving}, and (iv) {\em feature engineering:} if the data was pre-processed correctly for various downstream tasks (such as private/fair learning)~\cite{tramer2020differentially}.

%https://scholar.google.com/scholar?q=Datasheets+for+Datasets&hl=en&as_sdt=0&as_vis=1&oi=scholart --> look at related papers (delegated to anvith)

%\varun{how does confidentiality protect ownership? it may "enforce" ownership because the party owning the key can decrypt the data (proving that the data was theirs in the first place?)}\nick{changed "protecting" to "enforcing"}

Cryptographic primitives are essential in establishing and protecting data ownership by enforcing confidentiality. Applications of homomorphic encryption~\cite{gentry2009fully} to ML would provide the principal data confidentiality whilst still enabling training. Yet, the use of cryptography introduces computational bottlenecks and makes it difficult to leverage hardware acceleration, often requiring secure hardware~\cite{tramer2018slalom,volos2018graviton}. We discuss the application of homomorphic encryption to ML in more detail in \S~\ref{sec:assurance}. In addition, there has been a shift from centralized learning to distributed learning techniques (such as federated learning~\cite{konevcny2015federated}) to enable co-locating data and computation. Additionally, these learning techniques are {\em assumed} to provide data privacy as the data never leaves the data owner's site~\cite{melis2019exploiting}. Federated learning proposes to have individual data owners compute model updates locally on their data rather than share this data with a central server. The central server then relies on cryptographic primitives (such as secure aggregation~\cite{bonawitz2016practical}) to aggregate updates from different data owners. Other approaches involve using techniques from secure multi-party computation (MPC) to enable training~\cite{wagh2020falcon,wagh2019securenn,mohassel2017secureml,mohassel2018aby3,patra2020blaze,chaudhari2019astra,zheng2019helen,zheng2021cerebro}, but most suffer from poor scalability. 

%\varun{@anvith: please populate references as you read the scassa paper. also, what does it mean to distinguish data from facts?} \anvith{So basically facts are in the open-domain, but copyrights can apply to an original use of those facts. For example a unique selection of stories can become copyright based on the uniqueness of the selection. In general the idea is for copyright to reflect the work of the person who made it}

%\anvith{re did the following paragraph (commented out), where I followed mainly the same structure but changed the wording to explain the main points a little better}

%Beyond technical approaches,  ownership of data is also largely a legal matter. At a high level, current legislation often places an emphasis on hardware rather than information~\cite{scassa2018data}. In other words, the law defines ownership of physical hardware, \eg servers. These physical assets are owned by the data owner, or are owned by another entity which provides access to the data owner. However, ownership of information contained in such hardware, and the associated intellectual property rights like copyrights, is not as clearly defined in most cases. 
%For example, the European Union has special intellectual property rights in relation to data owned by corporations in databases~\cite{}, but Canada and the United States do not~\cite{} and have relied on the interpretation of existing laws. In North America, emphasis is put on the novelty of the data collection and analysis process to distinguish data from facts~\cite{}. If novelty of the ML pipeline being deployed is not demonstrated, intellectual property rights on the data are unclear. 

% Beyond technical approaches,  what data ownership means legally is a contentious matter~\cite{scassa2018data}. Current legislation placing emphasis on hardware rather than information~\cite{scassa2018data}; the law defines ownership of physical hardware, \eg servers. These physical assets are owned by the data owner, or are owned by another entity which provides access to the data owner.

% \st{For the following discussion of owning the information of the data, we'll specifically discuss data as datasets that are made up of individual datapoints (these datapoints can further be pieces of personal information, or facts defined in the legal sense). For ownership of the information of the dataset, the main distinction to be made is that it is likely that the individual datapoints are not copyrightable: this is the case if the datapoints are facts (measurements of the weather for example), of if it is made up of personal information~\cite{court1992mcinerney}, though provisions are in place in some countries that gives people more control on how their data can be used (\ie GDPR~\cite{mantelero2013eu}). The main distinction under which datasets may be copyrighted and thus owned (but not the individual datapoints it is made up of), as is explained by Scassa~\cite{scassa2018data}, is when the collection of datapoints constitute some original work (an example is that an original collection of well known stories could be copyrightable, in this case the collection is the dataset and the individual stories the datapoints); note that a copyright on the dataset would not prevent someone from using the individual datapoints but rather significantly copying the entire dataset. It should further be noted that copyright generally requires a human author and thus excludes completely automated processes~\cite{2010telstra,scassa2018data} with the exceptions of particularly original processess, though what constitutes sufficiently original work is subject to the court. For ML practices, what this last point entails is that if an ML pipeline being deployed is deemed not sufficiently novel, the dataset may not be applicable for copyright (and thus the information of the dataset is not owned by any specific individual). }
Defining data ownership legally is complex, if only because defining data itself is complex. Under most jurisdictions facts, that is the building blocks of the information recorded directly or indirectly as measurable data, are not protected by copyright law~\cite{scassa2018data}. Hence, the question of data ownership shifts from the protection of individual data records to their collection, arrangement, and derived works. Collections of data and derived works from data may be unprotected by copyright law depending on a number of conditions such as (i) under the merge doctrine~\cite{2007new,2013banxcorp}, if their exposition is inherently tied to the facts and data they represent, or (ii) if the arrangement is not considered original enough, as evaluated in court, \eg a phone book alphabetical order is not protected. For ML, this may entail that if a data collection pipeline being deployed is deemed not sufficiently novel, the collected dataset may not be protected by copyright law.  Observe that copyright on a dataset would not prevent someone from using individual data points but rather significantly copying the entire dataset. Depending on the jurisdiction, the status of ownership over personal information and the existence of a personal data ownership right is debated~\cite{scassa2018data}. Canada leans towards only providing access but not ownership of personal information whereas in the EU the existence of a personal data ownership right has been argued.

%An alternative mode to claim a form of ownership over data isIt should also be noted that copyright should not be mistaken for ownership in the property sense, as Scasse~\etal~\cite{scassa2018data} highlighted that case of 

% Otherwise, the intellectual property rights of data owners are currently unclear.\adelin{This is not the gist of what is said in that paper. While the point of hardware is correct, it's somewhat distracting from the main argument in that paper. The paper talks about what defines data, a complex question, and how data collections or agregates (like in big data) may or may not be protected by copyright law in Canada, Europe and the US. "Facts" are not protected by copyright law, hence the legal problem is to define what separates the data from its collection/exposition/organization. It turns out that for a collection of data (either collecting the data itself) is in North America is only protected if there is some form of originality in how the data is collected, generated and aggregated (with Canada in between EU and US). For instance, oceanographic data may be protected because of the non triviality of the engineering processes that involve deep human contributions. In Europe (for once including the UK), the question is quite different and efforts to build a system might be protected despite the system being "unoriginal". My own take: Given that this analysis states that a method that is "unoriginal" to collect and present data would not be protected, it seems that vanilla applications of DNNs models might actually not be protected by copyright law unless the model builder is capable of showing that their implementation or fine tuning of a DNN was "non trivial".}


% \nicolas{The EU has special IP rights in relation to DBs but Canada and the US don't. There are some circumstances where copyright can protect DBs but also circumstances where it does not.
% 3:08
% oops sorry — https://www.cigionline.org/static/documents/documents/Paper%20no.187_2.pdf
% 3:10
% what people can control is access to physical hardware that they own — e.g. servers and computers that hold the DB. These physical assets are indeed owned (or they are owned by the company who provides it to the DB holder and then there is some arrangement about controlling access).
% 3:12
% But the short answer (Teresa's paper gives a longer answer) is that you generally don't own information in Canada. You can own hardware and leverage this to control access. And you can have IP rights like copyright over information in some contexts.}

% \vspace{0.5mm}
\noindent{\bf Test Data:} At inference, the model is deployed to predict unseen data. Unlike training data, test data does not influence the model permanently (\ie it does not impact the values of the model parameters). That said, test data can still be responsible for model behavior that may make ML governance more difficult to achieve. For instance, test data may contain adversarial examples~\cite{goodfellow2014explaining} that affect the integrity of model predictions or sensitive data that should not be revealed to the model owner directly. Thus, like for training data, both technical and legal means are required to establish and protect test data ownership.

%\nick{why is adversarial examples related to data ownership?} --> i suspect because this a reason to ensure that test data can't be compromised (i.e. confidentiality of test data)

As discussed earlier, cryptography can address certain aspects of test data ownership as well. For instance, homomorphic encryption enables a model to perform inference without having a cleartext view of the input point~\cite{juvekar2018gazelle,mishra2020delphi,lehmkuhl2021muse}. The same can be achieved using techniques from MPC. This is helpful in scenarios where proprietary medical records can not be shared between institutions~\cite{alvarez2020secure,kaissis2021end,DBLP:journals/corr/abs-2107-10230}. Here again, moving from a central to a distributed setup for ML can help foster trust for the data owners~\cite{choquette2021capc}. % which proposes to have an ensemble of models collectively predict on a single test point without having the ability to read said test point. \varun{introduce technique used to achieve this}



%https://arxiv.org/pdf/1906.10908.pdf

\subsection{Model Ownership} 
\label{subsec:model_ownership}

Model ownership is often a broad term used to refer to the ownership of the model's {\em sensitive parameters} that were obtained after the (computationally intensive) training process. Defining ownership is necessitated by the existence of various threats that infringe the confidentiality of the model, and the need to be able to hold principals that own ML models accountable for the failures of their models. %Indeed, we rely on ownership in our upcoming discussion of accountability in \S~\ref{sec:accountability}. \nicolas{This last point is not clear in our previous data ownership section}

\vspace{0.5mm}
\noindent{\bf What is model extraction?} Attackers may target the confidentiality of ML models with a model extraction attack for three reasons: (i) data collection and labeling is time-consuming and expensive~\cite{halevy2009unreasonable}, (ii) the training process is computationally expensive (especially in many deep learning applications)~\cite{strubell2019energy}, and (iii) knowledge of the model can serve as reconnaissance to mount a follow-up attack against the model in the white-box threat model rather than black-box. Models that are proprietary could be released through insider threats~\cite{10.1145/1413140.1413158}, and models that are accessible via an interface can be reverse engineered~\cite{lowd2005adversarial}. If the latter is a query interface where principals can pose inference queries to models, then it is formalized as model extraction~\cite{tramer2016stealing}: the objective of the adversary is to succeed with {\em as few queries} as possible to avoid detection. By repeatedly posing (inference) queries to the trained model, the adversary recovers the model's {\em functionality}. But functionality is an abstract concept; Jagielski \etal~\cite{matthew2020high} provide a detailed taxonomy of what exactly an adversary can recover through this reverse engineering process, ranging from the exact model parameters to replicating output behaviors for specific input data points. 

Extraction is demonstrated in various domains, such as images~\cite{matthew2020high}, text~\cite{krishna2019thieves}, and for simple hypothesis classes~\cite{varun2020exploring}, and more complicated ones such as DNNs~\cite{carlini2020cryptanalytic, rolnick2020reverse}; assuming grey-box access~\cite{pmlr-v139-zanella-beguelin21a}, and more strict black-box regimes~\cite{milli2019model}. Some recent attacks do not pose inference queries, but assume access to hardware side-channels~\cite{batina2019csi,zhu2021hermes}; while such attacks recover the model, they are not model extraction attacks in the traditional sense. 

\vspace{0.5mm}
\noindent{\bf But how does the adversary generate queries?} Assuming that the adversary has access to the dataset used to train a model, or the distribution from which it was sampled from, is a strong assumption to make. To alleviate these concerns, Truong \etal~\cite{truong2021datafree} propose a refinement to the work of Kariyappa \etal~\cite{kariyappa2021maze}; they propose a {\em data-free} extraction method based on disagreement between the victim (\ie trained model) and model being trained by the adversary. A query synthesis active learning-based approach was used by Chandrasekaran \etal~\cite{varun2020exploring} for extracting simple hypothesis classes; this provides asymptotic bounds on the number of queries needed. The same authors also argue that pool-based active learning strategies can be used when the adversary does have access to a pool of unlabelled data, and Jagielski \etal~\cite{matthew2020high} propose using semi-supervised learning techniques such as MixMatch~\cite{berthelot2019mixmatch} to practically instantiate extraction. %at a low query complexity. 


\vspace{0.5mm}
\noindent{\bf Why is it impossible to prevent model stealing?} Various defenses have been proposed to prevent the adversary from learning enough information to enable extraction~\cite{juuti2019prada}. These range from reducing precision of the outputs~\cite{tramer2016stealing}, to more sophisticated approaches such as randomized model selection~\cite{kariyappa2020protecting,alabdulmohsin2014adding}, adding noise in responses~\cite{kariyappa2020defending}, protecting data points near decision boundaries by differential privacy~\cite{zheng2019bdpl}, or perturb outputs to mislead gradient-based optimization algorithms (\eg SGD)~\cite{tribhuvanesh2020prediction}.
% \varun{insert technique names here}
However, such approaches are rendered ineffective with an adaptive extraction strategy~\cite{varun2020exploring}, or introduce utility degradation. Chandrasekaran \etal~\cite{varun2020exploring} state the inevitability of extraction. The authors argue that any utilitarian model (\ie one that is reasonably accurate) leaks information which enables extraction. %\varun{roei's comment: new defense strategies try to "Detect" adaptive extraction -- do we have cites for this?}\nick{no, we wanted to cite lucy's work for this but it's not published yet (maybe there are works with similar idea we can cite?)}%This is very similar to the reasons why {\em knowledge distillation}~\cite{hinton2015distilling} is possible. 
%Recall that we define model ownership as the process of associating a principal with the learned model. It is clear this is challenging now since by model extraction, which is inevitable, multiple different principals may own very similar models.

\vspace{0.5mm}
\noindent{\bf How can one prove ownership?} To prove ownership, the process of {\em watermarking} was considered. Digital watermarking has been used to covertly embed a marker into digital media to later prove ownership infringements~\cite{petitcolas1999information}. In the context of watermarking ML models, the model owner encodes a specific query response pair into the training procedure (analogous to embedding a marker), and can verify if a model is indeed their own on observing such behaviours at the time of inference~\cite{adi2018turning}. This process is fundamentally similar to the concept of {\em backdooring}~\cite{gu2017badnets}, without any adversarial intent (with the additional requirement that watermarks are non-forgeable). However, recent work~\cite{jia2020entangled} demonstrates that watermarking is not resilient to model extraction; Jia \etal~\cite{jia2020entangled} propose an approach that remediates this issue, but with a nominal performance penalty. 

All forms of watermarking rely on encoding specific secret information {\em into} the training algorithm. Recent research suggests that there exists various forms of secret information \textit{already} available to the true model owner, obtained {\em during} the process of training. This includes the order in which data is sampled, intermediate checkpoints, hyperparameter values, the intermediate values of model weights, etc. One proposal to prove model ownership relies on the honest model owner logging such information during the training procedure. Since DNN training is a stochastic process, the intermediary states obtained during training are {\em hard to guess} without access to the secret information aforementioned. If a trusted third party can reproduce these states (within some acceptable tolerance threshold) with the help of the honest principal's secret information, then the honest principal's ownership of the model is validated. This is the premise of the {\em proof-of-learning} approach to enable ownership~\cite{jia2021proof}. 

% \vspace{-4mm}
\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=0.5pt,bottom=0.5pt]
% \vspace{-3mm}
\noindent{\bf Call to action:}\todo{put that in a grey box?} First, notice that claiming model ownership and differentiating between two models are two sides of the same coin. It is unclear if existing metrics (such as the distributional distance between model parameters or predictions) capture the {\em closeness}, and research is needed on this front. Second, most techniques to detect extraction rely on minor changes to the training procedure. More research is needed to understand if intrinsic properties of the ML model  can serve as its fingerprint (ergo enabling ownership resolution).
% \vspace{-3mm}
\end{tcolorbox}
% \vspace{-3mm}

%\varun{@adelin: add a brief description of how logging can help + how pol is one such logging strategy}

\subsection{Is model ownership separate from data ownership?} 

%Maini \etal~\cite{maini2021dataset} argue that knowledge contained within a trained model necessarily comes from its training set. Thus, they are able to reduce the problem of model ownership to a dataset ownership one which they tackle using a standard hypothesis testing framework. The intuition behind this reduction is that the extracted model is either trained on data labeled by the victim model, or data from the training distribution of the victim model. Therefore, the model owners only need to keep their training data, and are able to claim ownership of a stolen model if it has very high confidence on data points that are in-distribution for the victim model---in a process similar to membership inference but where signal is aggregated over multiple points. In other words, dataset inference is able to detect if two models are (even partially) trained on the same dataset. The drawback is that dataset inference cannot protect ownership of DNNs trained on public datasets. 

Maini \etal proposed dataset inference that validates whether a model was trained using a specific training set (or training-set distribution)~\cite{maini2021dataset}. This is related to model ownership because as long as only the model owner has access to the (proprietary) training data, the model owner can prove ownership. However, in other cases (such as training using public data), this technique cannot prove ownership.

%VC: Commented out to keep discussion abstract
%In particular, they observe that ML optimizers often increase the distance between a training sample representation and the incorrect-class decision boundaries of the model; but are unable to do so for a test sample. This disparity can, therefore, be interpreted as a membership signal similar to membership inference  attacks~\cite{shokri2017membership}. Since a model owner has complete access to ground truth membership information about their own training set, dataset inference~\cite{maini2021dataset} can improve on membership inference  through aggregating many such accurate membership signals. As a result, dataset inference is able to detect if two models are---even partially and/or indirectly---trained on the same dataset. The drawback, however, is that it cannot protect ownership of models trained on public datasets. 

%\anvith{added some citations and last bit}\adelin{lgtm thanks}
%such as (i) under the merge doctrine~\cite{2007new,2013banxcorp}, if their exposition is inherently tied to the facts and data they represent, or (ii) if the arrangement is not considered original enough, \eg a phone book's alphabetical order is not protected
Recall that from a legal angle, collections and derived works from data may at times be unprotected by copyright law. Because ML is known to memorize~\cite{feldman2020does}, models might not be protected by copyright law unless the model builder can show that their implementation non-trivially included significant original work. Similarly, content synthesized by generative models~\cite{zhang2020attribution}, and  language models such as GPT-3~\cite{brown2020language} could be, as derived work, respectively protected or in violation of copyright law~\cite{scassa2018data}. In Canada, but not necessarily in other jurisdictions like the European Union, copyright generally requires at least one human author---thus excluding automated art generation processes from copyright protection~\cite{scassa2018data}. 
% It should be noted, 
Given that instances of sufficiently original (and/or difficult) derived work have been allowed copyright~\cite{scassa2018data}, if a DNN satisfies such a condition that would allow for the distinction between data ownership and model.

%\adelin{This is not the gist of what is said in that paper. While the point of hardware is correct, it's somewhat distracting from the main argument in that paper. The paper talks about what defines data, a complex question, and how data collections or agregates (like in big data) may or may not be protected by copyright law in Canada, Europe and the US. "Facts" are not protected by copyright law, hence the legal problem is to define what separates the data from its collection/exposition/organization. It turns out that for a collection of data (either collecting the data itself) is in North America is only protected if there is some form of originality in how the data is collected, generated and aggregated (with Canada in between EU and US). For instance, oceanographic data may be protected because of the non triviality of the engineering processes that involve deep human contributions. In Europe (for once including the UK), the question is quite different and efforts to build a system might be protected despite the system being "unoriginal". My own take: Given that this analysis states that a method that is "unoriginal" to collect and present data would not be protected, it seems that vanilla applications of DNNs models might actually not be protected by copyright law unless the model builder is capable of showing that their implementation or fine tuning of a DNN was "non trivial".}

% Another proposal from Maini \etal~\cite{maini2021dataset} flips this approach to model ownership: they rely on the honest model owner's knowledge of the proprietary data used to train the model to prove ownership. 
% is intuited by the fact that the extracted model is either trained on data labelled by the victim model, or data from the training distribution of the victim model. Therefore, the model owners only need to keep their training data, and are able to claim ownership of a stolen model if it has very high confidence on data points that are in-distribution for the victim model. In other words, Dataset Inference is able to detect if two models are (even partially) trained on the same dataset. The drawback is that Dataset Inference cannot protect ownership of DNNs trained on public datasets. 
% \nick{@Mohammad you are the expert of this, feel free to modify/extend this paragraph}\mohammad{done}








%\nicolas{does a company own the fake paintings a GAN creates from artist paintings? same for github learning from user code. For this reason, a data owner may later seek to revoke access to their data by a model owner. This calls for machine unlearning, which we discuss later in \S~\ref{sec:}. }

\iffalse
\subsection{Open Problems}

%We will briefly discuss some open problems regarding ownership that we think are important to answer in future. 

\noindent{\bf Definition of Ownership:} The concept of ownership in the field of ML, especially model ownership, is a relatively new concept that appeared as a byproduct of research on model extraction attacks and defenses. Although we give a definition of model ownership, we believe it can be made more formal and precise in future. Thus the first open problem regarding model ownership is to introduce more formal and better definitions. 


\vspace{0.5mm}
\noindent{\bf Ownership of Predictions:} Most existing works aim to claim ownership of the model itself, but few focus on ownership of predictions (or other forms of outputs) made by the models. It would be interesting to see if one can claim ownership of predictions, or find the model/entity responsible for a prediction.

\vspace{0.5mm}
\noindent{\bf Metric to Quantify Difference:} Claiming model ownership and differentiating two models are the two sides of the same coin -- it does not make sense for two entities to claim ownership of the identical ML model. Thus a future direction is to introduce metrics that can differentiate two models owned by different entities.

\vspace{0.5mm}
\noindent{\bf Fingerprints of Models:} Techniques such as watermarking and proof of learning all require the model owners to be aware that they may want to claim ownership in future. However, such awareness is usually not the case, so future research may want to answer if it is possible to find some intrinsic properties of ML models that could be used as their fingerprint--something born with the model and can be used to tell its identity. Recently a related work tried to create fingerprints by non-transferable adversarial examples~\cite{wang2021characteristic}, but the goal was to differentiate different architectures rather than model instances.
\fi

==> Model%20Governance%20SoK%20draft/Contents/5_accountability.tex <==
% \newpage
\section{Holding ML Principals Accountable}
\label{sec:accountability}

Identities, as established in \S~\ref{sec:ownership}, serve multiple purposes~\cite{bishop}; one of them involves enabling{\em accountability}. In conjunction with traditional access control mechanisms, the notion of identity provided by data and model ownership in the context of ML allows us to establish the responsibility of principals interacting with an ML system. This is defined as accountability, and is different from the {\em process} of ascertaining accountability which we define as {\em attribution}. Indeed, accountability is essential when ML models produce {\em undesirable} behaviors (\ie failures) such as the ones discussed in \S~\ref{ssec:risks}. Some of these failure modes will be known and need to be attributed to a principal (we outline these earlier in \S~\ref{sec:principals}). This is similar to how malware analysis will seek to identify whether a malware originated from a state actor or not. Principals held responsible could be the model owner, but also end users (\eg if they are attempting to steal a model, or to have it produce an incorrect prediction with an adversarial example). Other failure modes of the model may be initially unknown but uncovered by external scrutiny of an ML pipeline, \eg by a regulator through an auditing process discussed later in this section. 


% \begin{enumerate}
% \item discussion around outlier detection
% \item concept drift detection
% \item detection of adversarial examples (adelin's work for example) \nick{currently working on this}
% \item detection of poisoning/backdooring attacks (sanghyun hong + nicolas papernot)

% \nick{the two items below is pretty much the same as "Assurance to Model Owners" in assurance.tex}
% \item detecting model extraction (lucy's work)
% \item add a sentence stating that it's hard to detect inference + reconstruction as it is passive
% \end{enumerate}

% Outlier detection for DNNs at test time was first introduced by Hendrycks \etal \cite{hendrycks2016baseline} where they showed that thresholding outputs provided a sufficient baseline as in-distribution and out-of-distribution points often yielded different outputs. Following this, c

% ~\cite{meinke2019towards,liang2017enhancing,lee2017training,lee2018simple,hein2019relu,hendrycks2018deep,ren2019likelihood,lakshminarayanan2016simple,vyas2018out},

\subsection{Attribution of Known ML Failures}
\label{subsec:attribution}

Recall that we define attribution as the process used to identify principals responsible for model failures. Here, we discuss detection of the failures discussed earlier in \S~\ref{ssec:risks}. This is a precursory requirement for attribution.

\vspace{0.5mm}
\noindent{\bf 1. Outliers:} A considerable amount of research investigates how to identify when DNNs are predicting on out-of-distribution (OOD) samples. The model's confidence for different outputs can be made more uniform on OOD samples~\cite{meinke2019towards,lee2017training,hein2019relu,hendrycks2018deep,lakshminarayanan2016simple,vyas2018out}, or the model can be trained explicitly to assign a confidence score which can be used to tell how likely the input was out of distribution~\cite{devries2018learning,vernekar2019analysis,malinin2018predictive}. Other methods have also been introduced to distinguish the outputs of DNNs on OOD and in-distribution samples~\cite{liang2017enhancing,lee2018simple,ren2019likelihood,serra2019input,hsu2020generalized}, including approaches based on inspecting the model's internal representations, training set, or performing statistical testing~\cite{raghuram2021general,sastry2019detecting,jiang2018trust,papernot2018deep,jha2019attribution}. These approaches could be applied to hold any principal querying the model on OOD samples accountable.

%All these have seen varying degrees of success, however there are yet no formal gurantees for a method to always work, with their being results showing why output based methods won't always work \cite{hein2019relu,vernekar2019analysis} (though more recently Meinke \etal \cite{meinke2019towards} analytically showed that their approach should work better than previous approaches).



%The need for outlier detection is prevalent whenever out-of-distribution inputs to a system can cause significant harm, and thus various general statistical methods have been used for the task of discerning whether a datapoint belongs to a distribution or not \cite{barnett1984outliers}. \anvith{maybe give some stats based examples} Nevertheless alternatives more tailored to the context of ML datasets (and the high dimensionality) have also been proposed: Escalante \etal \cite{escalante2005comparison} give a comparison of different approaches for outlier detection in ML datasets.\anvith{maybe give some examples not mentioned above}

\noindent{\bf 2. Concept Drift:} The model builder may attempt to detect drifts in the training data distribution to hold the data collector accountable. Lu \etal \cite{lu2018learning} summarize past research into three broad themes: (i) error rate based detection (a model's deteriorating performance serves as an indicator of shifts)~\cite{gama2004learning,gama2006learning,baena2006early,frias2014online,liu2017fuzzy,xu2017dynamic,huang2006extreme,ross2012exponentially,nishida2007detecting,bifet2007learning,bifet2009adaptive,bifet2009improving,bifet2009new,gomes2017adaptive}, (ii) data distribution based detection (which try and discern differences in the distribution of previous and new inputs)~\cite{kifer2004detecting,dasu2006information,song2007statistical,qahtan2015pca,bu2017incremental,liu2017regional}, and (iii) multiple hypothesis test drift detection (which differ from the previous two by utilizing more than one test to discern drift)~\cite{alippi2012just,wang2015concept,zhang2017three,du2015selective,maciel2015lightweight,alippi2016hierarchical,raza2015ewma}. Note that the two latter approaches could also be used by the data collector to hold potential downstream data contributors accountable.%\todo{Varun I removed a sentence below - lmk if it's a bad idea} %More recent work has looked at detecting drift in specific features~\cite{kulinski2021feature}, and improving data distribution based detection~\cite{yang2021cade}.

%Similar to outlier detection, concept drift detection is about understanding when the past dataset used to train a model is now an outlier to the current dataset the model experiences. One can take different approaches to detecting whether concept drift has occured, whether it is by looking at how the accuracy of a model changes over time or by running statistical test not too dissimilar than those for outlier detection; Lu \etal \cite{lu2018learning} describe and compare in detail different approaches relevant for ML.

% Since the goal is attribution, we only focus on detection techniques for data poisoning in this section. These
\vspace{0.5mm}
\noindent{\bf 3. Data Poisoning:} Attribution of poisoning can be done either at the data collection or model training stages. To the best of our knowledge, the only known techniques belonging to the former category utilize insight from outlier/anomaly detection~\cite{liu2017neural,Chen2017TargetedBA}. For the latter, research focuses on finding relationships between poisoned data and special behaviors in the representation space (or activations of hidden layers) ~\cite{tran2018spectral,chen2019detecting,liu2019abs}, investigate the gradients~\cite{Hong2020on}, or observe changes in the learned decision boundaries~\cite{wang2019neural,chen2019deepinspect}. 

\vspace{0.5mm}
\noindent{\bf 4. Adversarial Examples:} %Detecting adversarial examples (or evasion attacks) may serve as the basis for holding end users submitting them accountable, and is different from defending against them (\eg through adversarial training~\cite{goodfellow2014explaining}) which is a technique for assurance (see \S~\ref{sec:assurance}). \varun{we can scrap first sentence ?} 
To distinguish adversarial examples from legitimate inputs, detection techniques often first pre-process the inputs. This includes replacing the input by its internal model representations~\cite{lu2017safetynet, wong2018provable}, transforming the inputs~\cite{xu2018feature, roth2019the}, applying dimensionality reduction techniques~\cite{hendrycks2017early, bhagoji2017dimensionality}.
%, or even modeling the inputs from a steganalysis point of view~\cite{liu2019detection}. 
After pre-processing, a classifier or statistical tests distinguish distributions of adversarial and legitimate inputs~\cite{grosse2017statistical,hendrycks2017early,roth2019the,raghuram2021general}. %, and agreement of predictions on multiple inputs where some of them may be adversarial~\cite{tian2018detecting,xu2018feature,wong2018provable}. 
However, only a small fraction of the proposed detection techniques are evaluated against an adaptive attacker~\cite{tramer2020adaptive}, which may prevent robust attribution of adversarial examples and jeopardize accountability. 

%It is worth to note that most of these defenses do not require significant change in the training procedures so they are not mutually exclusive. Thus in practice, if affordable, a defender may want to use an ensemble of several detection mechanisms.

% Carlini \etal~\cite{carlini2017adversarial} has shown that some of the detecting methods can be bypassed by stronger attacks and identifying intrinsic properties that differentiate adversarial examples from natural data remains as an open problem. More recent works~\cite{lu2017safetynet,tian2018detecting,xu2018feature,liu2019detection,roth2019the,wong2018provable} are demonstrated to be robust against stronger and stronger attacks, but it is still unclear if there exists an optimal defense or this is just another army race between the defender and the adversary.

% binary classifieclear if r on inputs~\cite{hen, but it is still undrik2017on}
% N+1 class + Maximum Mean Discrepancy (MMD) test~\cite{grosse2017statistical}
% binary classifier on hidden layers~\cite{gong2017adversarial}

% safetynet: binary detector on discrete generated by quantizing activations of hidden layers~\cite{lu2017safetynet}
% binary classifier on predictions of several transformed images~\cite{tian2018detecting}

% PCA + cascade classifier~\cite{li2017adversarial}
% adversarial examples place a higher weight on the larger principal components than natural images~\cite{hendrycks2017early}
% PCA + binary classifier~\cite{bhagoji2017dimensionality}

% Feature squeezing: reduce degree of freedom at input space and check the difference between the predictions on original and reduced images~\cite{xu2018feature}

% distribution of outputs of last hidden layer~\cite{Feinman2017DetectingAS}

% detect steganography: dependency/differences between adjacent pixels modeled as a higher order Markov chain~\cite{liu2019detection}
% adding noise to adversarial examples incurs greater change in the logits~\cite{roth2019the}

% add outbound to the logit and assert the prediction doesn't change, \ie filter out any points that's too close to decision boundaries~\cite{wong2018provable}


% Data poisoning attacks~\cite{Rubinstein2009antidote,Shafahi2018poison,Jagielski2018Manipulating,liu2017neural,Chen2017TargetedBA} target the integrity of ML models. The adversary insert a small set of carefully crafted data to the training dataset, and aim to influence the model's performance. A special case of data poisoning is backdoor attacks~\cite{Shafahi2018poison,liu2017neural,Chen2017TargetedBA}, where at inference time the adversary would react abnormally to data points containing a designed trigger (the reaction is also designed by the adversary, \eg misclassify to a certain class).



%Some other works exploit more abstract behaviors of ML models. Kolouri \etal~\cite{kolouri2020universal} constructs images called Universal Litmus Patterns and trains a detector on the model's output on these images to detect poisoned model. Wang \etal~\cite{wang2019neural} and Chen \etal~\cite{chen2019deepinspect} observed the change in decision boundaries due to data poisoning and proposed detection mechanisms accordingly. 

%\nick{Despite most of the techniques for detecting poisoned models are empirically shown to be successful, they do not prevent the poisoned data to be used for training--this makes it harder to certify that the effect of backdoors are completely removed. Thus we want to ask the following question: is it possible to introduce techniques (other than anomaly detection) that can detect poisoned data before training? If not, can we introduce a more formal metric to quantify the effects of data poisong rather than sorely relying on classification accuracy?}

\vspace{0.5mm}
\noindent{\bf 5. Model Extraction:} To attribute queries contributing to a model extraction attack, Juuti \etal~\cite{juuti2019prada} compare the distribution of distances between queries. However, if an adversary leverages public data (which is in-distribution), the proposed detection method fails. It is unknown if other techniques can be devised for this in-distribution querying regime as well.
%\nick{Thus the open question here is if it is possible to defend this most powerful extraction attacks (\eg by quantifying the information leakage and stop responding to a user if certain threshold is reached, and if not, what degree of attribution should/can be required by the model owners?} 

%\nick{not sure if we should have this example--feel free to remove it if it leaks too much info about lucy's work}),  

\vspace{0.5mm}
\noindent{\bf 6. Privacy Attacks:} There currently exist no mechanisms to identify if privacy attacks (such as membership inference or data reconstruction) are occurring at inference time. This is due to the nature of the attack: adversaries query the model with (potentially) in-distribution data and observe the outputs. 

\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=1pt,bottom=1pt]
\noindent{\bf Call to action:}\todo{grey box?} Discovering approaches that can detect and attribute (adaptive)  membership inference while it is being performed remains an open problem.
\end{tcolorbox}

\vspace{0.5mm}
\noindent{\bf 7. Synthetic Content:} Generative models have revolutionized content generation~\cite{karras2019stylebased,zhang2019selfattgan,park2019semantic}; while this is useful in many scenarios (such as private data release~\cite{abay2019privacy}), it also introduces a myriad of problems. For instance, content produced by generative adversarial networks~\cite{gan_goodfellow} is being actively used in disinformation campaigns~\cite{bbc20chinastylegan}. A number of approaches were proposed in order to {\em detect} such fake content~\cite{mccloskey2018detecting,Li2020identification,zhang2019detecting,marra2018gans} (including large-scale competitions~\cite{facebook2020deepfakechallenge}). Attributing synthetic content to a particular generative model is difficult because models are often capable of producing~\cite{zhang2020attribution} and encoding~\cite{abdal2019image2style} any arbitrary content and allow for encoding of arbitrary contents. A promising approach is to study model components explicitly, \eg upsampling components which produce spectral aliasing~\cite{zhang2019detecting}. 

%\mohammad{\noindent{\bf 8. Unfairness}
% \begin{itemize}
%     \item pre-processing techniques  
%     \item in-processing techniques
%     \item post-processing techniques
%     \item metric fairness
%     \item causal definitions
% \end{itemize}
%}

% \varun{statement below is not clear from earlier discussion; some transition is missing}
% Observe that thus far, the identity responsible for training the ML model is responsible for all these failure events. It is thus in their best interest to attribute these failures to other principals like the data collector or end users through the detection approaches we have covered.

\subsection{Auditing to Identify New Model Failures}
% \subsection{ML Auditing \& Failure Detection}

Our discussion thus far has focused on techniques devised to detect failure models that are well known and understood. An alternative involves auditing mechanisms. To this end, we first define ML auditing and present how ML logging can support it. We then discuss storage, privacy, and security (open) problems that result.

%\varun{@adelin: the flow should answer the following questions: 1. how logging can help identify principals responsible for the aforementioned "bad events" --$>$ this is a more broad discussion; 2. why is logging for mL hard --$>$ this is also a broad discussion; 3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons); 5. how should it be logged (storage + computation costs); 6. compare + contrast with logging in practice}

%Similarly, accountability and attribution are the same problem viewed respectively internally and externally. 
%This apparently simple distinction provides deep insight. %This distinction is important and provides deeper insight than its apparent simple nature.
%To explicit the benefits of this model, we make a number of observation. 
%First, an internal audit is a proactive action, similar to a white-box assessment, and may rely on model \textit{logs}. On the contrary, an external audit is a policing action, similar to a black-box assessment, and may only rely on model querying. Second, 
%and internal audit results correct 

\vspace{0.5mm}
\noindent{\bf What is ML auditing?} Bishop defines an audit as a formal examination by a (third) party to determine a chain of events and actors~\cite{bishop}. In the case of ML, this definition must be extended to include the verification of the {\em claimed properties} of a model, such as its lack of bias or presence of adversarial robustness.
As noted in \S~\ref{sec:principals}, the different logical entities may, in practice, refer to the same principal. Hence, we call an audit \textit{internal (resp. external)} when the model owner and auditor are the same entity (resp. independent entities). Observe that an internal audit is a proactive action similar to a white-box assessment, and may rely on model logs \ie data records collected on the model and its inputs. On the contrary, an external audit is similar to a black-box assessment, and may only rely on model querying when the model owner cannot be trusted. Prior literature tends to conflate audit with external audit. This leads to a pessimistic view of ML audit as a non feasible task. This distinction helps us introduce alternate auditing methods including logs which are promising but completely unexplored. This apparently simple distinction provides deeper insight: (i) during internal audits, the regulators have white-box access to model internals, code, and logs; this enables easier verification of purported functionality as opposed to external audits where regulators only observe the functionality with no internal knowledge, and (ii) leveraging internal logs may alleviate technical limitations of an external audit \eg the current lack of guarantees with regards to model robustness when the auditor can only query the model. %, than to perform an external audit by querying a model in black-box fashion. 

For instance, the model deletion code (\ie internal audit) of SISA unlearning~\cite{bourtoule2019machine} can be reviewed for correctness \ie one only needs to check if a model is being trained without the data-point to be unlearned, while external verification (\ie external audit) of unlearning (through query access) remains challenging (because approaches like membership inference introduce a large number of false positives). For private learning, mechanisms like DP-SGD~\cite{abadi2016deep} come with a privacy accountant that trivially tracks expenditure, but the privacy of the models can also be audited through computationally expensive means post-hoc~\cite{jagielski2020auditing,nasr2021adversary} In the context of algorithmic fairness, model owners are being asked to conduct fairness audits~\cite{whitehouse, kim_auditing_2017}. Despite the well-intentioned tools that have arrived as a result~\cite{2018aequitas}, given poor incentives for model owners, we are now faced with the risk of fake fairness audit reports~\cite{faking_fairness}. Prominently, Aivodji~\etal demonstrates how using an interpretable proxy allows model owners to evade accurate fairness audits~\cite{aivodji2019fairwashing}.

% \varun{this faking thing is unique to fairness; can we streamline it to be similar to the other areas?}\adelin{I don't know as I didn't write this part on fairness and would not feel qualified on it anyway :-) . What I can say though is that industry folks usually have better things to do with their time and fairness issues are more likely to be out of lack of knowledge or concern altogether than fairwashing/fake fairness. I'd remove that sentence to be honest because it seems really really far fetched.}

Much like system and application logs are well-known as a fundamental tool in incident investigations in non-ML settings~\cite{bishop}, a model should never be separated from its logs. 

%\adelin{IT turns out that logging for an ML model is complex and arguably hardly ever properly defined in the literature.}
% }
%Hence, internal audit can support external audits and regulators should be flexible in mandating audit approaches. Regulators should require the most appropriate of internal or external audits depending on the technical feasibility of verification under each perspective. 

% \varun{thus far, you've not described ML logging at all and only described ML auditing; these definitions are also standard and not specific to the ML domain}\adelin{Yeah nicolas wanted both as per his comments and reply in the governance thread}
% \adelin{The external auditing perspective is common in the literature on security and privacy of ML. For instance, Jiagelski \textit{et al.}\cite{Jagielski_neurips_dpsgd} propose a poisoning attack to investigate privacy guarantees of Differentially Private Stochastic Gradient Descent.} \adelin{@anvith: here} 

%\anvith{@Adelin following is my blurb based on stuff I found: There has been significant past work on the external auditing of ML systems relevant for autonomous driving (more generally framed as verification of safety and robustness properties) \cite{xiang2018verification,pei2017towards,ivanov2019verisig}. In another case, Narodytska~\etal~\cite{narodytska2018verifying} were able to certifiably verify the robustness of a BNN (a binary neural network) to adversarial examples. More recently John~\etal~\cite{john2020verifying} proposed methods of approximately verifying the individual fairness of a model.}



%Adi, nicolas, @mohammad: privacy and fairness examples?, could also add milad's paper. }


%3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons);
%ML logs for properties or for principal actions


%Model owners may have an obligation to collect logs due to business (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pcidss_2015}) or legal requirement (financial institutions are required to report security incident and be capable of explaining the chain of event that lead to the breach or may see their practicing license revoked). 
%For instance, ML logging may be need to comply with the credit card transaction PCI-DSS standard~\cite{noauthor_pci_2020} while the EU AI regulation draft~\cite{eurlex_nodate} would fraud detection and credit scoring due to their impact on humans may require ML logging according. 

\vspace{0.5mm}
\noindent{\bf Why is logging hard for ML?} In general, knowing what and when to log is non-trivial and highly use-case dependent. Additionally, log storage space is finite, and overhead induced by logging is challenging in many other domains~\cite{bates_trustworthy_nodate}. Logging in ML differs from non-ML applications because of (i) ML pipeline control-path explosion dependent on external events, the data, and randomness which increases the content required to be logged, (ii) the different ML-specific steps, like training and testing, of the model life cycle which require logging very diverse and step specific information, and (iii) there is a need, parallel to that in system and application logs, to focus on both identifying principals responsible for a specific high-dimensional input but also, specifically for ML, tracking certain model properties (required for accountability and attribution respectively). %\varun{refer roei's comments for the 3 points that follow} \adelin{solved with roei's help} %\varun{what makes the last point a problem?}. %\stout{the probabilistic nature of ML} %Common log formats,\eg the format used in syslog~\cite{gerhards_syslog_2009}, are inappropriate for ML as they are designed to compactly log network or system events (for instance storing only an event's time, type and name). 
Consequently, the ML logged information may greatly differ from traditional event logs used in application, network, and system security. For example, the proof (or log, albeit it is not referred as such) created in the work of Jia \etal~\cite{jia2021proof} is created with the explicit goal of proving model (parameter) ownership and requires information about data used to train the model, randomness used in the training process (which is hard to precisely capture), and tracks the change in model parameters as training progresses.  
%\varun{why the next sentence?}\adelin{To illustrate a paper that does ML logging without realizing it does ML logging (it does not refer to ML logs), but needs to concentrate on a specific phase (training) and on specific challenges of data collection size. The data collected is specific to that phase and the conclusions would not hold for test time ML logs or any other part of the ML model life cycle.}

% \varun{still don't know what an ML log will look like to agree that it's gonna be different from logs in the traditional sense}\adelin{I'm not sure how you want to present that, there is a problem of circularity: you need to log a lot more and different elements than in traditional settings so the log volume is increasing faster than syslog which have efficient format}

% \varun{clearly this is paradoxical; we wanted to identify "new threats" using logging and now you're saying logging is dependent on the threat we wish to identify? while i agree with you, what is the truth? are logs specific to threats or can new threats be identified from logs?}\adelin{I agree that the section title is not good. Logs are specific to threats. Logging is usally a forensics help where you investigate a system post hoc. Nonetheless as in the surreptious paper some threats may not be detected but only found out in the forensics setting. Lastly, logging may help in identifying violations that are not possible to identify externally by just querying the model but those are not new threats.}

 %Consequently, the model owner may need to collect gradients, weights, hyperparameters, model inputs along the corresponding principals or any other information. Despite efficient formats for network or system events, \eg the format used in \texttt{syslog}~\cite{gerhards_syslog_2009}, overhead is already a major issue in non-ML audit log systems~\cite{bates_trustworthy_nodate,owasp_logging}. 
%This problem is only accentuated for ML models as models can have trillions of parameters~\cite{} and inputs may have high dimensionality. %Common log formats,\eg the format used in syslog~\cite{gerhards_syslog_2009}, are inappropriate for ML as they are designed to compactly log network or system events (for instance storing only an event's time, type and name). 

%varun: para below repeats content above; will merge the two

% \vspace{0.5mm}
% \noindent{\bf What and when to log?} Ideally, one would collect all possible information regarding the model and inputs. However in a real production system, log space is inherently finite (and log overhead is an issue in other domains~\cite{bates_trustworthy_nodate,owasp_logging}). ML model owners should first define the life cycle step and threat they want to mitigate with logging. At training time, model owners should log model parameters that track the property of interest, \eg, privacy expenditure ($\varepsilon$) through noise addition. During deployment, model owners may further have an obligation to collect logs due for business reasons (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pci_2020}), or legal reasons (the EU AI regulation draft may require ML logging of fraud detection and credit scoring due to their impact on humans~\cite{eurlex_nodate}). Hence, standard ML logging guidance and a dedicated yet efficient ML log format must be designed from ground up. \varun{provide some suggestions on how this may look like}\adelin{Don't want to provide too much as nicolas wants a paper on that}\adelin{For instance, the difference in weights at different steps could be saved instead of the weights themselves. The format could also specify common properties of interest and how their structure can be used for format-specific compression.}

\vspace{0.5mm}
\noindent{\bf Maintaining log confidentiality.} Lastly, when designing an ML auditing system based on logs, the privacy and security of that system itself should be taken into account. 
%While standard logging and backup protection guidelines~\cite{owasp_logging,noauthor_pci_2020} should be employed where relevant, we delve further into two 
Here again, ML introduces specific issues. First, since logs may be accessed by auditors, they represent a risk and must be sanitized~\cite{bishop}. As illustrated in other sections, this sanitization is not trivial and in the case of logging is further complicated by its stream nature. This (important) requirement makes ML logging hard in practice. Second, adversaries may try to simultaneously pose threats to the ML model and log analysis system (if it is ML-based). For example, Travers \etal~\cite{travers2021exploitability} propose evasion attacks for audio-based ML models whilst ensuring that intermediary steps (which can be considered as logs) are within acceptable levels.

% \vspace{0.5mm}
\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=1pt,bottom=1pt]
\noindent{\bf Call to action:}\todo{grey bubble?} Despite the upstart of a number of industry ML logging tools and practices (both for the model and underlying system performance)~\cite{noauthor_whylogs_2021}, only little academic work has delved into the challenges of ML logging. 
\end{tcolorbox}
%google_monitoring, mlflow_log, fiddler_monitoring_nodate,amazon_log,


% We discuss two works, which despite not explicitly referring to logs, can be thought to provide a form of training time logs. The Proof-of-Learning framework from Jia \etal~\cite{jia2021proof} saves a model weights to enable internal audit against model extraction attacks\adelin{@mohammad please verify this} \varun{enables external audit too}. Hong \etal~\cite{Hong2020on} leverage gradient information at training time to identify and mitigate model poisoning \varun{based on the discussion of hong's paper, it seems like any technique that relies on some model specific information to make a decision about a failure event is considered an internal audit; if this is the case- there are dozens more}\adelin{Can we discuss this directly and do you have a list of papers you want to add.}. For deployment time, Chen \etal~\cite{DBLP:journals/corr/abs-1907-05587} utilize input correlation to identify model queries made in preparation of an adversarial example based attack. In the audio biometrics domain, Travers \etal~\cite{travers2021exploitability} show how compliance-driven ML input logs can be leveraged for malicious authentication investigation (similar to Transition-Based Auditing which targets known attempts to breach security~\cite{bishop}).

%Ideally, one would collect all possible information for each single input to the model, however in a real production system, log space is inherently finite. Overhead is already a major issue in non-ml audit log systems~\cite{bates_trustworthy_nodate,owasp_logging} for which each individual record is small; the problem is only accentuated for audit logs of ML models and systems (SOTA models can have trillions of parameters~\cite{}).  %These formats are extremely compact (\eg an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). 
%Hence, a dedicated yet efficient log format must be designed from ground up for ML logging.



%These formats are extremely compact (\eg an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). 

%A wide range of existing frameworks in traditional security (eg \url{https://cheatsheetseries.owasp.org/cheatsheets/Logging_Cheat_Sheet.html}). They are not readily applicable in ML due to the probabilistic nature of the domain (like how SISA is the only method to perform perfect unlearning so far). In the same way we can't readily use normal logging procedures for audit log generation. However, we could use proof of learning algos for audit logs. 

%Since SOTA models can be extremely large, a huge body of works focuses on model compression but models can still be in tens or hundreds of MBs making checkpoints prohibitive as a log solution.
%\varun{motivate why checkpoints can be used for logging a bit better; the next para does that well}

%"Logging is the collection of information; auditing is its analysis."
%A bit reducing the audit process but acceptable
%"Last comes auditing. Commercial systems emphasize recovery and accountability. Auditing is the process of analyzing systems to determine what actions took place and who performed them. Hence, commercial systems must allow extensive auditing and thus have extensive logging (the basis for most auditing). Logging and auditing are especially important when programs move from the development system to the production system, since the integrity mechanisms typically do not constrain the certifier. Auditing is, in many senses, external to the model." bishop
%Basically external is when the enforcement arm of the auditor is mandated by someone other than the model owner and internal is when the model owner and regulator enforcement are conflated
%attribution is external under that view while accountability is internal.
%in acountability the model owner proactively makes the model identifiable in case of a problem.
%In attribution the model owner is trying to evade being linked to a specific model
%often, a lot of the research is written under the assumption that the model is productized or whatever and external entities find issues that require resolution. auditing + logging seems to be the only internal concept that’s interesting, that i can think of. anything i am missing?
%I think there is: internal can help exernal. See it as internal ~= whitebox, external ~= blackbox. (edited) 
%Then proof of learning is internal whereas radioactive data is somewhat external
%internal can help external -> that also makes sense. and this concept holds across, right?
%Yep. In financial audit a regulator requires both external and internal audit
%Audit logs may be useful to detect an attack while it is happening, perform post hoc correlation analysis over multiple records (a stronger paradigm then current ML model defenses/cite lucy's work), or enable the reconstruction of event following an attack to identify the \textit{modus operandi} of the attacker and prevent the same attack from reoccurring. 





%"The first goal is to detect any violations of a stated policy; the second is to detect
%actions that are known to be part of an attempt to breach security." bishop

%\vspace{0.5mm}\noindent{\bf Existing work}
%6. compare + contrast with logging in practice
%The external auditing perspective is common in the literature on security and privacy of ML and is covered in a number of related SoKs\cite{}\adelin{Adi, nicolas, @mohammad: privacy and fairness examples?, could also add milad's paper}. 




%\vspace{0.5mm}\noindent{\bf Security and privacy of ML logs}
% 2. why is logging for mL hard --$>$ this is also a broad discussion;
%   5. how should it be logged (storage + computation costs); 
 %
%We identify 2 major open issues with ML logging, respectively log sanitization and storage overhead.

%As outlined in \S~\ref{sec:model_extraction} the case of ML, such risks include model inversion and membership inference techniques. \varun{don't quite understand how these issues are exacerbated when the logs are provided, especially if the auditor is "trusted"}\adelin{because even a trusted auditor is not allowed to see certain information. For instance, a pentester is trusted but should not get access to your SSN when they pwn the client's db. Trusted does not mean can disregard all privacy and confidentiality laws}

 

%instantiate the surreptitious adversarial example class with a joint optimization attack. Similarly, Chen \etal~\cite{DBLP:journals/corr/abs-1907-05587} introduce query blinding to attack their stateful detection system.



% \subsection{Accountability}

% \varun{make blanket statement about accountability here (\ie it is model owner's problem if any of these issues occur) + discuss (a) baiwu’s work here, and (b) @Nick Jia did some research from the policy/legal side (recall our discussion of smart cars + who is responsible if it crashes) — we can add this too. we can phrase this as a broader open question that the community should address}

==> Model%20Governance%20SoK%20draft/Contents/6_assurance.tex <==
% \newpage
\section{Assurance in ML}
\label{sec:assurance}

In addition to being transparent about failures resulting from the ML system's use, which they can be held responsible for as shown previously in \S~\ref{sec:accountability}, ML principals will need to establish trust in their application of ML techniques. Bishop distinguishes trust, which is the often ill-defined belief that a system is secure, from \textit{assurance} which is a set of techniques by which one builds confidence from evidence that a system meets its security requirements~\cite{bishop}. Here, by security we refer to the broader mitigation of risks identified in \S~\ref{ssec:risks}. One well-known example of such techniques is formal methods for verification, which have started to emerge for ML systems~\cite{raghunathan2018certified,cohen2019certified,sommer2020towards,singh2019abstract,singh2018fast}. We discuss these techniques and others, following the operational life-cycle described in \S~\ref{ssec:lifecycle}



\subsection{Assurance during Data Preparation}
\label{subsec:assurance_data}

Assurance in the context of data preparation ensures that models learnt satisfy specific properties (\eg privacy, robustness, fairness, etc.). Assurance can be provided through data sanitization (\eg removal of data poisons)~\cite{gudivada2017data,cortes1995limits} and checks for concept drift~\cite{lu2018learning}, bias alleviation~\cite{wang2020revise,zhang2018mitigating}, and subgroup representation~\cite{buolamwini2017gender,selwood2002politics}. To the best of our knowledge, there has been no work that provides formal guarantees about a dataset providing the aforementioned properties. It is also unclear how such guarantees would be provided. An alternative approach to providing assurance involves providing documentation showing the processes used during data collection met certain criteria that are designed to provide assurance; Gebru~\etal~\cite{gebru2018datasheets} proposed datasheets for datasets, a generic documentation scheme meant to be used to verify the data collector employed practices sufficient to alleviate known failures, and other work have further expanded on (or proposed similar measures)~\cite{holland2018dataset,miceli2021documenting,costa2020mt,hanley2020ethical}.


\subsection{Assurance for Training}

As in the case of prior components of the life cycle, assurance can either be obtained {\em post-hoc} (\ie after training completes), or be obtained during training. Recall that assurance is required among various axes, which we describe next.

\vspace{1mm}
\noindent{\bf Integrity:} In the context of evasion attacks, robustness is {\em provably} provided using two main strategies. The first is adversarial training~\cite{madry2017towards} and its variants~\cite{shafahi2019adversarial,xie2019intriguing,xie2020smooth,tramer2019adversarial,andriushchenko2020understanding,shafahi2020universal,wang2019convergence,wong2020fast}. Such strategies are formalized such that assurance is encoded into the training algorithm and an auditor would have to inspect the algorithm itself to understand what properties were provided. An alternative approach involves providing a certificate of robustness~\cite{cohen2019certified, salman2019provably} which provides a certificate indicating that the trained model is robust to perturbations within a pre-defined $p-$norm radius. To the best of our knowledge, Steinhardt \etal~\cite{Steinhardt2017certified} proposed the first certified data poisoning defense by proving an upper bound on the model's loss in the presence of an adversary. However, as they pointed out, their methods have to run on clean data, which is often impractical. Ma \etal~\cite{Ma2019DataPA} propose DP as a solution against poisoning and provide theoretical bounds on the number of poisons tolerable by such models. Weber \etal~\cite{Weber2020RABPR} and Levine \etal~\cite{Levine2021deep} both propose newer certified defenses against data poisoning; the former uses techniques similar to randomized smoothing~\cite{cohen2019certified} and the latter uses collective knowledge from an ensemble of models to prove robustness. Finally, integrity of the computation and model parameter values can also be verified by a mechanism that provides a proof associated with the particular run of gradient descent which produced the model parameters, as suggested by Jia \etal~\cite{jia2021proof}. 

\vspace{1mm}
\noindent{\bf Privacy:} Several approaches can be taken to preserve data privacy. The de-facto approach is to utilize {\em DP learning}. Proposed initially by Chaudhuri \etal~\cite{chaudhuri2011differentially}, DP learning has evolved from the objective perturbation approach proposed by the authors to more sophisticated techniques which involve adding noise during optimization~\cite{abadi2016deep}, or during aggregating votes from disjoint learners~\cite{papernot2018scalable}. These newer approaches have tighter forms (and analyses) of privacy accounting (\ie calculating $\varepsilon$). In the decentralized setting, approaches such as CaPC~\cite{choquette2021capc} provide assurances about data confidentiality and privacy. Recent research~\cite{jagielski2020auditing, nasr2021adversary} demonstrates that the privacy accounting during training is not tight (in practical scenarios), and could benefit from external audits.
% \varun{check if milad's work also suggests that it's not tight; matthew's work suggest that the gap sometimes is 10-100x}\anvith{I can confirm Milad's work shows it's tight (they instatiate a really strong adversary under which the lower bound on DP becomes almost the upper bound)}\anvith{I recommend saying not tight for most common adversaries}

% \varun{commenting below as it is added to patching}
%Complementary to ensuring that a model does not learn sensitive information, the process of ensuring that the ML model forgets a piece of data and remains comparably performant is formalized as {\em machine unlearning}. More details are provided about techniques in \S~\ref{}. The assurance that unlearning is correctly performed stems from the technique deployed (for example, re-training a model after removing the data-point {\em provably} unlearns that data-point). It would be ideal for a governing body if there was a black-box procedure that could take a model and a datapoint and conclude if the model had "unlearned" that datapoint or not, and in fact in some sense POL \cite{jia2021proof} can do just that; if "unlearning" simply means plausible deniability, then in fact submitting a POL that didn't use that point would count as unlearning as it shows the model \textit{can} come from training without that datapoint.

\noindent{\bf Randomness:} Unsurprisingly, providing assurance that sources of randomness in the process of learning are cryptographically secure is essential. Research demonstrates that, if manipulated, the order of the batches served to a model during training can itself result in a lack of generalization guarantees from the training algorithm, resulting in a lack of integrity for the model parameters output by this training algorithm~\cite{shumailov2021manipulating}. Furthermore, randomness in data sampling is fundamental to amplification results demonstrated for DP learning~\cite{abadi2016deep,erlingsson2020encode,kairouz2021practical}. Providing assurances on this matter is an open problem.

%the decision making process \varun{process?}\mohammad{decision making process} --> swapped with example

\noindent{\bf Fairness:} For individual fairness, \cite{ruoss_learning_2020} produces a formal certification by ensuring the representations of similar points are kept close in the latent space. For subgroup fairness definitions, however, 
% despite the outsized importance of data collection in ensuring fairness~\cite{selwood2002politics}, 
the primary focus
% of algorithmic fairness 
has been in designing unfairness mitigation techniques despite data bias issues.
Considering a core ML task (often classification) as an example, these techniques can be categorized into {(i)} pre-processing, where algorithms re-weight, obfuscate, transform, and/or remove samples to satisfy a notion of fairness~\cite{wang2020revise,feldman2015certifying,calmon2017optimized,kamiran2012data,zemel2013learning}; {(ii)} in-processing, where additional constraints are added to the optimization procedure to result in fairer models~\cite{zhang2018mitigating,kamishima2012fairness,celis2019classification,ruoss2020learning}; or {(iii)} post-processing, where the output is changed to match a desired distribution~\cite{hardt2016equality,pleiss2017fairness,kamiran2012decision}. Other methods have been developed to empirically assure the fairness of a model by thoroughly documenting its performance on different sub-populations~\cite{mitchell2019model,yang2018nutritional}.

Despite improving fairness, an important limitation of these techniques is that they do not strictly provide formal fairness guarantees. To obtain assurance of fairness during the training of a model, algorithms that provably result in fair models must be implemented. Again, initial work in this vein provides guarantees through
pre-pocessing~\cite{feldman2015certifying} and  in-processing~\cite{celis2019classification,zemel2013learning,ruoss2020learning}. The most well-known formal guarantees for prediction fairness is provided under a metric-based notion of individual fairness~\cite{individual_fairness}: Rothblum~\etal introduce a PAC-like relaxation of the said notion to prove asymptotic fairness guarantees for the individual~\cite{pacf}.

\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=1pt,bottom=1pt]
\noindent{\bf Call to action:}
The algorithmic fairness community has recently recognized the importance of considering the broader ``algorithmic system''~\cite{studying_up}, to consider social actors and decision making context. While we agree with the message, we posit that we need to go beyond studying fairness---or any single class of risk on its own---and consider the complex but realistic interplay of the principals in the broader context of ML governance. Given the importance of data in all such systems, a concrete step is to research fairer, more accurate, and non-privacy-invasive data collection practices. 
\end{tcolorbox}
\vspace{-2mm}


\subsection{Assurance at Deployment}
\label{subsec:assurance_deployment}
% \adelin{conflates model builder and deployer which might no be the same} 

When a model is deployed as a service, there are mainly two entities possibly interacting with the model: the service provider who publishes the model, and the end users querying the model. In this section, we discuss assurance provided by the service providers to the end user.

% \subsubsection{Assurance to End Users}
To build end user confidence, service providers may aim to show two features of their service: (i) integrity, that is the computation is performed correctly and the prediction is indeed made by the model being advertised (rather than for instance a simpler but cheaper model), and (ii) maintain confidentiality of the query made by the users which can contain sensitive information. For example, hospitals may query online healthcare ML models to diagnose patients' diseases, where 
the queries could contain the patients' (private/confidential) health condition. %\varun{the previous sentence talks about training, not inference..}\nick{I rewrote it}

\vspace{1mm}
\noindent{\bf Integrity:} End users would require assurance regarding the correctness of the prediction generated by the model. The field of verified computations~\cite{walfish2015verifying} is designed to allow a principal to verify the correctness of outsourced computation. The main issue with using {\em off-the-shelf} techniques from verified computations literature on DNN inference is the large overhead incurred. To solve this issue, building on Thaler \etal's~\cite{thaler2013time} work towards efficient verified computing, Ghodsi \etal~\cite{ghodsi2017safety} introduce SafetyNets which applies verified computing techniques to inference operations efficiently. 
% scales verified computing techniques to verify the integrity of inference made by MLaaS
Note that verifying the integrity of computation is fundamentally different from approaches that assure confidence of (or trust in) the prediction~\cite{jiang2018trust} %\varun{last sentence is confusing?}. \nick{I don't remember writing this sentence and not sure what is supposed to mean. maybe someone else can help}

%In high level, SafetyNets represent DNNs as arithmetic circuits and uses Thaler \etal's~\cite{thaler2013time} method to verify the matrix multiplication and quadratic activation at each layer of the DNNs. It is worth to note that there is some restrictions on the architecture of the DNNs for them to be represented as arithmetic circuits (\eg MaxPooling layer and ReLu activation function cannot be used). Besides, SafetyNets assume the user also has access to the model's weight parameters, which is usually unrealistic in the setting of MLaaS. Thus, future work is needed for verifiable inference that is (i) more efficient, (ii) applicable with more commonly used DNN architectures, and (iii) requires less information known by end users.

\vspace{1mm}
% \varun{privacy is not confidentiality}
% \nick{changed all "privacy" to "confidentiality" in this paragraph}
\noindent{\bf Confidentiality:} Another concern of using MLaaS is regarding the confidentiality of the data used to query the ML models. To this end, several approaches rely on homomorphic encryption~\cite{dowlin2016cryptonets,liu2017oblivious,juvekar2018gazelle,mishra2020delphi,reagen2021cheetah}, or use MPC techniques for inference~\cite{wagh2020falcon,choquette2021capc}. Both these approaches rely on cryptographic techniques which are provably correct. 
% \varun{@nick: add references to mpc for inference.} 


%proposes CryptoNets to encrypt the users' data by homomorphic encryption (HE) so that most operations needed during inference such as multiplication and addition can be applied to the encrypted data. Then the user receives the model's output and decrypts it locally. However, the use of HE causes the inference time to be significant slower than on plaintext. Following researches try to solve this by combining HE with other cryptographic techniques such as secret sharing and garbled circuits (MiniONN)Besides how to improve performance, another question we may want to ask in this field is how could the certificate of confidentiality be providing to some end users who do not have any knowledge on cryptography (\eg a normal person bought a smart door lock). \varun{missing papers from raluca ada popa} \nick{added}

% \varun{missing discussion about explainability; cc @mohammad @anvith}\nick{working on this}

% \noindent{\bf Explainability:} \nick{The explainability of predictions made by ML models is directly related to if end users can trust the predictions, since ML models are black-box functions that output predictions without any visualizable reasoning--making them hard to be trusted.}

%  \nick{In high level, there are two streams of works here: (i) feature-level, and (ii) concept-level attributions. The former attributes every pixel to a prediction by locally trained model (LIME~\cite{ribeiro2016lime}), or gradient-based methods with different noise reducing techniques~\cite{kindermans2018learning, Kapishnikov2021guided}. The outputs of these methods are usually binary or 0-1 masks indicating the contribution of each pixel to the model outputs, which can be considered as a certificate. On the other hand, concept-level attribution can be achieved by concept classifiers (TCAV~\cite{kim2018tcav}), decomposing activations to pretrained concept vectors~\cite{zhou2018interpretable}, or even in the unsupervised setting, clustering super-pixels to create concepts~\cite{ghorbani2019towards}. The advantage is that the concepts can be more easily understood by humans. However, it becomes harder to certify the explainability since we do not know what portion of information in the predictions is explained by the concepts. Thus Yeh \etal~\cite{yeh2020completeness} proposes a completeness metric to quantify explainability achieved by given concepts.}

% LIME: interpretable model locally around the prediction~\cite{ribeiro2016lime}

% trust score: ratio between the distance from the testing sample to the nearest class different from the predicted
% class and the distance to the predicted class~\cite{jiang2018trust}

% gradient based attribution with different noise reducing methods~\cite{kindermans2018learning, Kapishnikov2021guided}

% concept-based attribution: concept classifier~\cite{kim2018tcav}, decompose activation to pretrained concept vectors~\cite{zhou2018interpretable}, clustering of super-pixel~\cite{ghorbani2019towards}

% measure completeness of concepts~\cite{yeh2020completeness}




% \subsubsection{Assurance to Model Owners}
% As mentioned in \S~\ref{sec:ownership}, ML models are valuable intellectual properties. Thus when they are deployed as services, the service providers need to give assurance to the model owners that their models are not damaged or stolen (by the users). Recent researches has shown that with only the same power as a normal end user, an adversary could implement attacks that steal the ML models (model extraction~\cite{}), or infringe the privacy of data used for training (membership inference~\cite{} and model inversion~\cite{}). If online learning~\cite{} is applied to the MLaaS, in particular when the end users can submit data to train the model, there could be even more threats. For example, an adversary can craft data points to force the model to learn unwanted behavior (data poisoning~\cite{}), and/or increase the power consumption and latency for training the model (sponge examples~\cite{}). Similarly to before, we will also discuss the assurance to model owners from the perspectives of integrity and confidentiality.

% \noindent{\bf Integrity:} Integrity of a ML model might be targeted by the adversary if he/she gets access to manipulate the parameters of the model (\eg by submitting training data ), which is the case in online learning~\cite{}. Data poisoning and sponge examples are attacks that can happen in this situation. Since the threats come from the training data, the service providers can use the same methods to achieve assurance at \S~\ref{subsec: assurance_data}.

% \noindent{\bf Confidentiality:} The main threat factors for confidentiality of the model (model extraction attack) and its training data (membership inference/model inversion attack), which are both valuable intellectual properties of the service providers, happen at the inference time. We have discussed in \S~\ref{subsec:model_ownership} and \S~\ref{} what are these two attacks and how they can be applied with only black-box access to the model respectively. Here we are interested in what can the service providers do to assure the users are not applying these attacks while querying the MLaaS. However, although there exists works on detecting/defending these attacks as described in \S~\ref{subsec:attribution}, most of them assume the service provider is the same as the model owner, so they do not consider the problem of assurance and only empirically demonstrate their methods to be successful. 
% None of them comes with a certification mechanism or provides a formal proof that the system is secure, which is important for achieving assurance. We hope that our work will help bring people's attention onto this problem and perhaps help others to construct techniques to provide assurance to model owners.

==> Model%20Governance%20SoK%20draft/Contents/7_patching.tex <==
\section{Life Cycle Management of ML Systems}
\label{sec:life-cycle-management}

% \nicolas{but also how one can efficiently store the different versions of a model}

The techniques presented thus far do not preclude ML models from needing modifications: training from scratch to remove certain pathological behaviors learned by the model may be expensive~\cite{bourtoule2019machine} and leveraging backups will not solve issues which are embedded in the backup model's weights. The process of patching an ML system, a form of maintenance, is thus the last component of our approach to governance. In the following, we outline what these different processes would look like for ML systems.

%Eventually, one may also wish to retire the ML system.

% \nicolas{see the concept of recovery p10 bishop}


\subsection{Patching ML Systems}

%Research suggests that modification to a model's behavior which was learned from data may be done in a two-step approach. First, remove the effect of a subset of the training points. Then, learn a new behavior. 

% We can expect during the lifecycle of the model, which encompasses the events that occur after deploying the model, that various modifications must be made post deployment. These 

%realize that the training data was poisoned and now presents a security risk to end-users who interact with the model. It could also be that under various conditions, such as the EU's GDPR~\cite{gdpr}, the model owner's access to some portion of the data that was used to train the model is revoked, in which case they are no longer allowed to deploy a model which had used said data. The specific case where for various reasons a deployed model must now be modified/patched to "forget" some portion of its original training dataset (\ie the poisoned data or the data the model owner no longer has access to) is what is referred to as machine unlearning \cite{cao2015towards}.
% \vspace{1mm}
\noindent{\bf 1. Unlearning:} After deployment, the model owner may lose access to part of the data used to train the model. This may be due to detecting data poisons, or outliers, or for legal reasons. For example, this may be the case when the data collector raises privacy concerns and invokes the right-to-be-forgotten~\cite{bertram2019five,mantelero2013eu}. The process of obtaining a model without the influence of said data-point(s) is referred to as machine unlearning~\cite{cao2015towards}. 

% (up to some maximum number of data-points to forget) \varun{content in brackets vague}\anvith{@Varun actually can I change the above bit for DP to the certified-forgetting citation (as it's probably the better citation on this, it's the bigger paper)?, it would then be: "Alternatively, the approach of Guo~\etal~\cite{guo2019certified} states that if one makes the feature extraction of a model DP-private and then applies a unlearning rule on the final linear layer, one can have certificates of indistguishability of the final model from one that was properly unlearned"}

Various forms of unlearning have been proposed which offer different guarantees. For example, retraining a model from scratch would give a concrete guarantee to the end-user the unlearned model is now independent of the data the user revoked access to. However, this comes with large (training) costs. One could modify the model's architecture and training pipeline to reduce the retraining cost~\cite{bourtoule2019machine}, but to some the cost may still be too high. Alternatively, the approach of Sekhari \etal~\cite{sekhari2021remember} states that a model with strong privacy guarantees (\ie DP-privacy) does not need to be modified to forget a user as it does not leak user-specific information in the training dataset, and thus unlearning requires no additional computational resources. However, private models are often not utilitarian~\cite{tramer2020differentially,bagdasaryan2019differential}. To find a middle ground between computational costs and performance, an alternative approach is to define an unlearning rule (for example adding a hessian-vector product) that modifies a model such that the resultant model would be similar to a model that had not trained on the users' data~\cite{guo2019certified,graves2020amnesiac,golatkar2020eternal,baumhauer2020machine}.

%one might modify the weights by some amount (that is not too expensive to compute relative to retaining, for example a single gradient or Hessian-vector product) \varun{content in brackets again vague}\anvith{how so? added a "single .." to be more specific} to be more similar to those that would have come from a model that had not trained on the users' data~\cite{guo2019certified,graves2020amnesiac,golatkar2020eternal}. In other cases, only the last layer of the model's weights are modified~\cite{baumhauer2020machine}. \varun{what's the advantage/disadvantage of modifying last layer?}

Unlearning highlights the importance of modeling interactions between ML principals and the interplay between different risks raised (\S~\ref{sec:game}). For example, a user's decision to revoke access to their information can itself leak information about them having been in the training dataset if it is made adaptively~\cite{zanella2020analyzing,gupta2021adaptive,chen2020machine}. %This can possibly create tensions with the fairness of the ML pipeline~\cite{bourtoule2019machine}. \varun{why only fairness? not robustness?}\anvith{I don't think I've read work investigating that}

%(if normally they had a $50\%$ chance of being sampled into the training set, but because of model memorization they consistently revoke access, then we'd see a gap between the expected model distribution and that which we observe and could infer membership), which presents another consideration for what unlearning must achieve, and this was further investigated by Gupta~\etal~\cite{gupta2021adaptive}.%There have also been various other approaches for unlearning models that are not DNNs \cite{}. \anvith{I think this last sentence is kind of forced, we might just want to drop it}

% \vspace{-1mm}
\begin{tcolorbox}[boxsep=0.5pt,left=0.8pt,right=0.8pt,top=0.8pt,bottom=0.8pt]
\noindent{\bf Call to action:} Regulators will play an important role in deciding what should be forgotten (and to what degree) for the various scenarios when parts of the training dataset must be removed. It could be that any unlearning method that mitigates privacy leakage would suffice for dealing with users revoking access to their data. In contrast, it might be that for data poisoning (where there could be grave security risks) the model owner would need to completely retrain or give some guarantee of changing the weights sufficiently to remove the threat. Determining this is subject to future research. 
\end{tcolorbox}

% \vspace{1mm}
\noindent{\bf 2. Fine-tuning:} One may also want to additionally learn new model behaviors. This can be achieved by fine-tuning models. Fine-tuning is needed in two scenarios: in (i) online learning~\cite{fontenla2013online}, \ie more and more data becomes available after the model is trained so it is preferable to fine-tune the model on more data to improve its performance, and (ii) transfer learning~\cite{tan2018survey}, where one wants to fine-tune a trained model to help a different but related task, \eg classifying traffic signs used in another country.
% \nicolas{Someone should fill in using below}
% \begin{enumerate}
% \item online learning
% \item transfer learning
% \end{enumerate}
If the model's capacity remains fixed or training data previously used is not repeatedly used to train the model, one must take care in avoiding catastrophic forgetting: by learning a new behavior, the model may inadvertently perform poorly on data points it has previously analyzed~\cite{French1999Catastrophic}.
% \todo{add citations}

% \fi



\subsection{Retiring ML Systems}

Following our discussion of unlearning, it is easy to see that one may consider retiring an ML model altogether when a large portion of the training data is requested to be unlearned (and the remaining data is insufficient to obtain a performant model). Apart from unlearning, there may be other reasons for a model owner to choose to retire an ML pipeline. This includes ethical concerns where retiring the data itself may help prevent further ethical concerns, \eg as discussed by Peng \etal~\cite{peng2021mitigating}. Regulators will here again play a crucial role, and may decide to develop frameworks that encourage ML principals to retire their data and models when appropriate. 

%\nicolas{note from tired Nicolas to Varun: in case we run out of space, do not remove this retiring ML idea because we mentioned it several times in abstract + intro, feels novel and important!}

% \nicolas{discuss implications of retirement for privacy (e.g., right to be forgotten)}

% \varun{also discuss arvind narayanan's new paper on dataset retirement}


==> Model%20Governance%20SoK%20draft/Contents/8_discussion.tex <==
\section{Discussion}

Our systematization led us to develop a framework for ML governance. Through the concepts of ownership, accountability, assurance, and life cycle management, we foster trust between principals involved in an ML application. Our game formulation proposes to explicitly search for equilibria that balance the benefits of ML with its risks. Space constraints prevented us from discussing certain aspects that remain relevant to achieving governance. For instance, deploying ML involves computer systems that support ML but are not captured in our analysis; such computer systems are implicitly assume to form the trusted computing base. Hence, our solutions for governance largely rely on the security of these systems themselves. Beyond this aspect, we now outline avenues for future work to strengthen our understanding of governance.

\vspace{1mm}
\noindent{\bf Risk Interplay:} Through this work, we have delved into understanding various facets of risk associated with ML. The game formulation explains the interaction between various principals and how this leads to a constant recalibration of risk. Yet, we pointed out how there remains a limited understanding of the interplay between the various risks themselves. %For example, it is well known that private learning results in utility degradation~\cite{tramer2020differentially}, but we have a limited understanding of why \varun{not a good example? adding noise results poor utility is well understood?}. In a similar vein, 
Limited research has been conducted to analyze the interplay of the various facets of risk in unison; research however has been conducted to understand this interaction in a pair-wise manner (\ie relationship between utility and robustness~\cite{dohmatob2019generalized}, or privacy and fairness~\cite{chang2020privacy}), but this paints an incomplete picture as discussed in \S~\ref{sec:game}.

\vspace{1mm}
\noindent{\bf Inter-principal Trust:} An important goal of governance is to improve trust between ML principals. Hence, documenting clearly the limitations of ML systems is of paramount importance to communicate clearly when a satisfactory approach to governance cannot be found. For this reason, we believe that approaches analogous to the one taken by dataset cards~\cite{gebru2018datasheets} will complement well our work on governance. This also relates to research on explainability which seeks to enable end users to understand the logic behind learning algorithms. There are two lines of work here: (i) feature-level, and (ii) concept-level attribution. The former attributes every feature (\eg pixels in an image) to a prediction~\cite{ribeiro2016lime,kindermans2018learning, Kapishnikov2021guided}. The latter attributes higher-level concepts to a prediction~\cite{kim2018tcav,zhou2018interpretable,yeh2020completeness}.

\vspace{1mm}
\noindent{\bf Interpretability:} The techniques discussed in \S~\ref{sec:accountability} arm principals in identifying various issues. However, they may not understand {\em why} these issues occur and consequently may have a difficult time resolving them. Ensuring that the learning and prediction process of many ML algorithms is interpretable (particularly to non-experts) is paramount to enable more widespread and trustworthy usage. 

\vspace{1mm}
\noindent{\bf Parameterization:} Furthermore, the assurance provided is often parameterized. For example, the assurance provided by DP learning is the expenditure of privacy ($\varepsilon$). However, interpreting these parameters is non-trivial for the average user. It is also cumbersome for the user to specify their requirements (for example, privacy requirements) to model builders for the same reason. Parameterized definitions are not easily accessible, and this further impedes governance. Additionally, recent research~\cite{kaptchuk2021need} suggests that user expectations for privacy do not match what is provided. Thus, this difference between mental models and reality can also impede governance. While similar to the earlier discussion on interpretability, we wish to highlight that parameterization is more focused on providing principals knowledge to bootstrap the training process, while interpretability provides tools to better understand its outcomes.

\vspace{1mm}
\noindent{\bf Trust in Regulators:} We implicitly assumed that the regulator principal is trustworthy and seeks to preserve the society from ML risks. This may not always be the case, for instance in settings where ML is used by authoritarian regimes. Additionally, trusted regulators may not be privy to sensitive information in reality, as such forms of data transfer are strictly governed by laws~\cite{2016re}. 

\vspace{1mm}
\noindent{\bf Legal Challenges:} While we have taken care to highlight certain legal challenges raised by ML governance, there currently lacks interdisciplinary work on law and ML. Studying the technical problem in isolation is unsatisfactory because without a match between law and techniques, techniques will not see adoption. For instance, the technical community focuses on DP but legal frameworks focus on anonymization~\cite{gdpr}. This gap results in a lack of adoption of advances made to privately learn from data. Sometimes the inverse problem holds: while laws against disparate impact have long been in effect; it has been fairly recently that we have seen their adoption by the ML community~\cite{feldman2015certifying}.

% \anvith{@mohammad here, also can cite \cite{feldman2015certifying} if you want}

%Sometimes, the inverse is also true: laws that are framed (such as equality) are seldom part of algorithmic frameworks by default~\cite{}.\todo{}

% Nicolas: I am commenting this out because it is a bit fuzzy. If we want to keep some of this, I would recommend merging with "Parameterization" instead.
% \vspace{1mm}
% \noindent{\bf Techniques Re-use:} We have mentioned some techniques that may contribute to governance. However, most of them were not designed for the goal of governance initially, so some adjustments may need to be made for them to be used in practice. For example, many techniques mentioned when discussing assurance are only demonstrated to be successful empirically but lack of formal certification mechanisms. Besides, there is few standardized and quantifiable metrics for techniques performing similar tasks in model governance, so another step towards practical model governance is to fulfill this shortage. We hope that our work will help bring people's attention onto these problems and lead to techniques more practical to model governance.

% \nick{we may also want to mention the following}
% \begin{itemize}
%     \item \nick{the gap existed for most works from being used in practice in model governance, i.e., many works only give empirical results but not any proved/certified robustness}
%     \item \nick{another step towards practical model governance is standard + quantifiable metrics for assurance/attribution/etc.}
% \end{itemize}



% communication 

% \todo{should probably move cards somewhere in the actual body of the paper - but I'm affraid I'll forget it later}

% \adelin{This section conflates ML system and ML model. I would use ML model to be consistent with the rest of the paper and to avoid opening the can of worms of system patching} \adelin{Otherwise we will have to go into technical solutions for parallel model deployment in ML systems/MLOps like TF Serve, AWS Multimodels and TFX. I can write a paragraph on that if we want the systems approach. I can write a definition of ML systems if we want to go down that route too }

% \subsection{Stack}

% ML security relies on systems security 
% \adelin{Excellent to see that here! Happy to take a stab at this as well. @nicolas please let me know}




% \subsection{Legal}

% Studying the technical problem in isolation is also unsatisfactory because without a match between law and techniques, techniques will not be adopted by companies. For instance technical community focuses on differential privacy but legal frameworks focus on anonymization. This gap results in a lack of adoption of advances made to privately learn from data. \adelin{Very good points. I think we want to go beyond legal for compliance/say somewhere that by legal we understand a broader meaning like industry frameworks one has to respect under the threat of losing operating licenses}

% \nicolas{laws bishop p18}

% \subsection{Rogue governments}
% \adelin{If we talk about human rights, the elephant in the room is rogue governments. Here the regulator is implicitly assumed trustworthy. What if this is not the case?}

==> Model%20Governance%20SoK%20draft/Contents/Figures/table.tex <==
\begin{tabular}{llllll}
\toprule
Principals/Life Cycle & Data Collection & Data Pre-processing & Model Training & Model Inference & Model Retention \\
\midrule
Data Collector     & \citefull{liu2017neural} \citefull{gebru2018datasheets}   &    &       &       &   \\
Model Builder     &    &      & \citefull{tran2018spectral} \citefull{lakshminarayanan2016simple} \citefull{malinin2018predictive} \citefull{jia2020entangled} \citefull{jia2021proof} \citefull{lu2018learning} \citefull{madry2017towards} \citefull{cohen2019certified} \citefull{Steinhardt2017certified} \citefull{abadi2016deep} \citefull{dowlin2016cryptonets}  &       &   \\
Model Maintainer     &    &      &       &  \citefull{malinin2018predictive} \citefull{lu2018learning} \citefull{juuti2019prada}  & \citefull{bourtoule2019machine}  \\
%Test Data Owner     &    &      &       &       &   \\
Adversary     & \citefull{munoz2017towards}   &      &   \citefull{shumailov2021manipulating}    &    \citefull{szegedy2013intriguing} \citefull{shokri2017membership} \citefull{jia2018attriguard} \citefull{fredrikson2015model}   &   \\
End User     &    &    &    & \citefull{perdomo_performative_2021} \citefull{dowlin2016cryptonets} &   \\
Trusted Arbitrator    &    &      &       &    \citefull{ghodsi2017safety}  & \citefull{jia2021proof}  \\
\bottomrule
\end{tabular}

==> Model%20Governance%20SoK%20draft/Contents/Unused/Structure.tex <==
\anvith{below is very rough, will fill in when I wake up}

\vspace{1mm}
\noindent{\bf Section:}{What is Governance}
\anvith{this is basically the blurb I was thinking of}
\paragraph{Define Governance formally} Have model owner(s), user, third part arbitrator, and the possibility of a model owner or user being adversarial. Goal of governance is to define/instruct how a third party arbitrator resolves conflicts between and among the other two players. Main interactions of interests are between model owners and other model owners (possibly adversarial), users (possibly adversarial), and users interacting with adversarial model owners.

Model owner vs adversarial model owner is what we define broadly as model stealing (i.e., ownership disputes), and specific examples are \anvith{add specific examples}

Model owner vs adversarial user is what people have generally been calling adversarial machin learning, and specific examples are adversarial examples, data poisoning, sponge examples, etc.

Adversarial Model Owner vs user is what we typically characterize as fairness \anvith{I think}

Model governance isn't interested in the specific ways these parties interact, but rather resolving the claim by one party that the other is adversarial (i.e., a model owner claiming another model owner is adversarial, or user is adversarial etc). The claims fall under the following main categories

\begin{enumerate}
    \item Ownership disputes: Model owner makes the claim another model owner is adversarial
    \item Adversarial Detection\anvith{better name?}: Model owner makes the claim a user is adversarial
    \item Auditing disputes: User claims the model owner is adversarial
\end{enumerate}

Model governance deals with the above, but also the subsequent process after such a claim is found to be true. In certain cases these would be legal actions (a legal suit against the adversarial model owner or user), in other cases it's a form of patching (model owner modifies model to satisfy auditing). As we're not legal experts, we focus on just this last problem (amongst the subsequent processes), the question of patching to satisfy auditing (in particular what this satisfying means).




\anvith{so we now have the following sections}

\vspace{1mm}
\noindent{\bf Section:}{Ownership}

\vspace{1mm}
\noindent{\bf Subsection:}{Prevention}

\begin{enumerate}
    \item "Proof of Learning:Definitions and Practice" \cite{jia2021proof} \anvith{we all know what this is about}
    \item "Perturbing Inputs to Prevent Model Stealing" \cite{grana2020perturbing} \anvith{to read}
    \item "Defending against model stealing attacks with adaptive misinformation" \cite{kariyappa2020defending} \anvith{to read}
\end{enumerate}

\vspace{1mm}
\noindent{\bf Subsection:}{Identification}

\begin{enumerate}
    \item "Proof of Learning:Definitions and Practice" \cite{jia2021proof} \anvith{we all know what this is about}
    \item \anvith{add watermarking citations}
\end{enumerate}

\vspace{1mm}
\noindent{\bf Subsection:}{Patching}
\anvith{not sure what patching model stealing means}

\vspace{1mm}
\noindent{\bf Section:}{Adversarial Users}

\vspace{1mm}
\noindent{\bf Subsection:}{Prevention}

\begin{enumerate}
    \item "On the (statistical) detection of adversarial examples" \cite{grosse2017statistical} \anvith{to read}
    \item "Detecting adversarial examples using data manifolds" \cite{jha2018detecting} \anvith{to read}
    \item "Sample Complexity of Adversarially Robust Linear Classification on Separated Data" \cite{bhattacharjee2020sample} \anvith{to read}
    \item \anvith{find more citations for robust training of machine learning}
    \item \anvith{add citation for prevention of data poisoning}
\end{enumerate}


\vspace{1mm}
\noindent{\bf Subsection:}{Identification}


\begin{enumerate}
    \item first two references for prevention also fall into this
    \item "Detection of adversarial training examples in poisoning attacks through anomaly detection" \cite{paudice2018detection} \anvith{to read}
    \item "Detecting Poisoning Attacks on Machine Learning in IoT Environment" \cite{baracaldo2018detecting} \anvith{to read}
\end{enumerate}

\vspace{1mm}
\noindent{\bf Subsection:}{Patching}

\begin{enumerate}
    \item \anvith{not sure what paching an adversarial examples means}
    \item for data poisoning, all unlearning papers (could cite mine for an overview of approximate approaches, and SISA for exact)

\end{enumerate}





\vspace{1mm}
\noindent{\bf Section:}{Auditing}

\vspace{1mm}
\noindent{\bf Subsection:}{Prevention}

\vspace{1mm}
\noindent{\bf Subsection:}{Identification}

\vspace{1mm}
\noindent{\bf Subsection:}{Patching}



==> Model%20Governance%20SoK%20draft/Contents/Unused/accountability.tex <==
\section{RM3: ML Accountability through Model Ownership}

\paragraph{Change in Threat Model for Accountability}(Nick) When we are considering accountability instead of ownership, it may be possible that the model owner/trainer is uncooperative. For example, if we find a model that is not trustworthy and we suspect a person/organization A trained it -- then if we don't have a record of A's PoL, we won't be able to claim A is the trainer since A could totally only provide part of the PoL.

Adelin: In the worst case the model owner would not even release a partial PoL. Do you suggest PoL should become legally required (in which case the partial PoL makes sense)? I don't see a legal requirement to release a PoL as it would become a huge risk to model developers and would stiff innovation in the field beyond repair. It's interesting how this ties back to the european legal framework however.

Adelin: The above problem relates nicely to the logging problem. It's a common issue in audit. People usually resort to a confidence based approach: the more trustworthy you seem (by proactively providing proofs), the more leeway you get down the line. I think we can do the same with an "adaptive" PoL model that is not all or nothing but rather there is a confidence parameter that the auditor/verifier has.

Nicolas: "yeah we will need some commitment for a model"; 
Nicolas' comment on the example: "I think in this case we should assume that the party will want to prove that it is their model and it complies with fairness/privacy requirements".

Another interesting part would be if we (as the government) find a model that is not trustworthy and have a database of many models/PoL released by many people/organizations, how could we efficiently find the suspicious trainer of the not trustworthy model

Adelin: It's a good idea but it requires a number of extra infrastructure. You need proper process to add the models to that list. How do you ensure that the list is not leaked, proper chain of custody of the list, registration? 

% Nick: 

\paragraph{Formalize Terminology}(Nick) I think we need to clarify the difference between signature of training a model, and signature of a trained model. The former is more related to ownership, while the latter is more
related to accountability.

Adelin: One question I have with this is how resilient these definitions would be to a system perspective. It might be early for this reflection but I believe 2 trained models could have vastly different outcomes depending on the pre and post-processing (see the audio and finance papers). Hence can we really limit the definition to the model itself? In the proof of unlearning paper there is a distinction between the unlearning over the weights and over the outcomes. I think this is important here as well.

There are a few things could be used as (part of) signatures, e.g. knowledge of a model, exact parameters of a model, or even prediction vectors made by a model. I think it's worth to discuss their difference, and how they are related to ownership and accountability.

Adelin: What would be useful as well is a discussion of why cryptographic signatures can't be used out of the box for this purpose. We would also need to distinguish a signature that cannot be spoofed from a "fingerprint" that correlates 2 models but can be spoofed. 

Anvith: k so just cuz I'm terrible at reading and need lots of bold letters I put what Nick and I discussed during our meeting in the subsection below. Basically we tried to make some formalism of the trying to reason with accountability.

\subsection{($\epsilon, \delta$) Accountability for Machine Learning}

The idea was to abstract our way to what we truly mean by accountability and then providing some mathematical definition we could then work with. The setup is as follows.

In general we have a proof of learning $P$ and knowledge of some process $F$ that takes as input a proof of learning (so could simply be a function of the final weights as that's part of a proof of learning) and returns some arbitrary function/model; note this process could be slightly random. We now wish to know, given some set of states $\mathbf{X}$ in the output space of $F$, can we say that this set was derived from a proof of learning $P$, i.e., can we hold $P$ accountable for them?

This leads to the following definition, where we now denote $m$ as some measure on the space of proofs $M$ (so some real vector space if we're mainly just interested in the final weights aspect of a proof $P$):

\begin{definition}[($\epsilon, \delta$) Accountability]
We say $P$ is ($\epsilon, \delta$) accountable for the set $\mathbf{X}$ if $\mathbb{P}(F(P) \in \mathbf{X}) > \epsilon$ and $m(A) < \delta$ where $A = \{a \in M~s.t~\mathbb{P}(F(a) \in \mathbf{X}) > \epsilon,~a \neq P\}$
\end{definition}

where essentially the definition captures the likelihood of $\mathbf{X}$ coming from $P$ (the $\epsilon)$ and nothing else (the $\delta$); the goal is to push $\epsilon$ close to 1 while bring $\delta$ as small as possible. Note $A$ and $m$ here have been left ambiguous as to what space they are, i.e., what is the topology of proofs? The main choices I think of interest are

\begin{enumerate}
    \item If we're simply interested in the space of final weights resulting from a proof (or in general the sequence of weights), then $A$ is some subset of an real vector space which defines $M$, and $m$ can be chosen to simply be the Lebesgue outer measure.
    \item If our space of proofs $M$ is in fact some countable (finite) set of proofs (say for example a ledger we've kept of all the proofs we're interested in), then $A$ is some countable set and $m$ is the canonical counting measure
\end{enumerate}

So $A$ can be constructed, it's just a question of what the specific scenario we're interested in (note that lebesque measure does carry some undesirable consequence such as having non-empty sets with measure 0, namely any countable set). You can also expect $F$ output space to be in one of these two scenarios (i.e., a real vector space of discrete set).

Adelin: There are classic proofs in Statistical Learning Theory to deal with the issue that the function space is infinite and that we could adapt to this case. We don't necessarily need finite ledgers (countable is a nice property already) in fact.

Just to make explicit, the concrete accountability scenario is

\begin{definition}[Absolute Accountability]
We say $P$ is absolutely accountable for the set $\mathbf{X}$ if $\mathbb{P}(F(P) \in \mathbf{X}) > 0$ and $A = \emptyset$ where $A = \{a \in M~s.t~\mathbb{P}(F(a) \in \mathbf{X}) > \epsilon~\forall \epsilon \in (0,1],~a \neq P\}$
\end{definition}

which allows to conclude that $X$ must have come from $P$ (if $M$ is an exhaustive set of all the proofs). Nevertheless this has been rather abstract, but let's just proceed abstractly for a moment to consider some $F$, and at the end I'll try and set up how these definitions lead to concrete renditions/procedures.

Adelin: I think we should avoid "absolute" if we are dependent on a measure unless we can come up with an equivalency result for arbitrary measures (in which case the above is correct). 


Adelin: This definition of A is non-constructive in practice which is really problematic. Do you take a closed-world assumption? The definition of accountability is also dependent on the chosen measure when it should be independent of it in the general case. you could define different strength levels of accountability depending on the assumptions made. Moreover you make a somewhat naive assumption that a PoL will be released for a given model. I'm saying that this is naive because at best you could hope for plausible deniability that the model did not come from you (as in baiwu's paper) but at worse an adversary would just not release a PoL tying them to a model

Anvith: So yeah in the second scenario for A and m I just added above (which I think is the one we're really interested in) it's akin to a closed-world assumption where we basically only are interested in the proofs we know to exist (those we have a ledger on). I also added two examples of what scenarios for A and m we'll probably be interested, and so we can basically just say out right that if it's a real vector space we're focused on lebesque outer measure, and if it's a countable set we're just using a counting measure. For the different strength levels I was actually thinking about what absolute accountability in our sort of closed-world assumption would be, and added it above. And yeah I do make the naive assumption that PoL will be released for the model we're trying to deduce accountability on, and that we have a set of all PoL we're interested in.


Adelin: Is the set X finite or even countable? I fear it might be hard to prove things in the general case.

Anvith: I'm thinking it depends on what F really does; if it maps to a countable set of models (so it performs some countable function like setting some countable number of weights to 0) then X is some countable set. If instead F manipulates the weights in some continuous way (say by adding noise to them) then X would need to be some subset of a real vector space. I guess another naive assumption is that we know the process F an adversary might employ. 

%where essentially the definition captures the likelihood of $\mathbf{X}$ coming from $P$ (the $\epsilon)$ and nothing else (the $\delta$); the goal is to push $\epsilon$ close to 1 while bring $\delta$ as small as possible.

\subsection{A Classification of Interesting F}

So after having sort of come to a definition, we basically came up with two interesting $F$ to study (there definitely could be more)

\begin{enumerate}
    \item $F$ takes as input the final weight from $P$ and trains $n$ steps on some arbitrary dataset/distribution $D$ to obtain some new final weights $w_n$
    \item $F$ modifies the final model from $P$ but retains its functionality; that is the model returned by $F(P)$ returns the same (or tries to return the same) outputs as the final model in $P$. In other words we did something but haven't changed the \textit{function}
\end{enumerate}

\subsection{Making this Concrete}

\subsubsection{The real vector space Case} Let us consider the following pseudo-example. For the time being let's say the aspect of proof of learning we're interested in is the final weights, and so the space of proofs is a real vector space which is the weight space. Let's also say that $F$ is a process that takes the final weights $w \in R^n$ and maps them to $w' = w+u+g \in R^n$ where $g$ is some noise and $u$ is a constant vector; let us say we know $g$. We denote $\mathfrak{P_w}$ as the probability density function of the random variable $w'$ starting at $w$

Let's say now $X \in R^n$ is some subset of weights and we suspect $w$ is accountable for them. We proceed then as follows to find the $\epsion,\delta$ accountability

First to find epsilon we compute $\epsilon = \int_{X} \mathfrak{P_w}(w') dw'$, and then to find delta we find $A$ by finding all $a$ s.t $\epsilon =< \int_{X} \mathfrak{P_a}(w') dw'$; if $g$ is explicit (say Gaussian noise) this shouldn't be impossible as the right hand side is an integral we can get an explicit formula for, and if it's too difficult we can always just find some larger subset containing $A$ and use that for our bounds (by the monotonicity of measures).

Lastly we then find the Lebesgue outer measure of $A$ to get $\delta$, or if we're lazy we can just bound it (using a larger subset that contains it), to get our $\delta$.

Now say that $X$ isn't a set but just a single point, in which case the above procedure is meaningless as $\epsilon = 0$. Nevertheless we can artificially create a small ball around $X$, $B_r(X)$, and define this as our new set $X'$ of interest. I think we can then focus on the $r$ that minimizes $\delta$ for a given $\epsilon$ s.t $\epsilon \leq \int_{B_r(X)} \mathfrak{P_w}(w') dw'$, and this provably gives some sense of the accountability for $X$, but I'm not sure why.

Anyways with either $X$ or using $B_r(X)$ we can add another layer to this setup, where now we add that in fact we're interested in some countable set of the real vector space of proofs (say a countable set $A'$). In which case we're now interested in the counting measure of $A' \cap A$ where $A$ was obtained as above; this could possibly lead to something remotely like absolute accountability where now if the intersection is empty, with $\epsilon \neq 0$, then we deduce $w$ must have led to $X$ as there were no other choices. 

\subsubsection{A practical protocol}

Basically the question is what do we do when we don't have such a precise definition/understanding of $F$ like in 3.3.1; say in the case 1 from 3.2 where F is just training.

Well I think the idea is to find thresholds like POL which allow us to deduce with confidence that some set of weights $X$ came from a certain initial weights (so high epsilon) but nothing else (low delta).

\paragraph{Experimental Setup for Finetuning}

My idea is the following

\begin{enumerate}
    \item We start from some pretrained weights $w_0$ and finetune on some dataset to obtain finetuned weights $w_f$
    \item we repeat this many many times to construct a distribution for the weights coming from $w_0$ (we can do this by artificially making the space discrete and doing probability buckets over the space)
    \item Now we repeat for many different pretrained model $w_1,w_2 \cdots$ to construct corresponding distributions $\mathbb{P}_{w_0},\mathbb{P}_{w_1}, \cdots$
    \item we now test our ability to distinguish whether a finetuned model came from some weights by uniformaly drawing some model from $w_0,w_1, \cdots$ and finding the according epsilon and delta accountability for the various pretrained models; we can try various schemes but for now I think picking the one with the largest epsilon will do
\end{enumerate}

UPDATED: we can actually use kalman filtering given in https://arxiv.org/abs/1912.11316 to compute distributions, then it's just a matter of solving the real vector space case tightly


\subsection{Some general theoretical observations}

\begin{lemma}[Order reversing of epsilon and delta]
For a given $P$, $F$, $X$ and space of proofs $M$ and measure $m$, if we have one pair of epsilon delta accountability $(\epsilon_0,\delta_0)$, then for all  $\epsilon \geq \epsilon_0$ s.t $\mathbb{P}(F(P) \in \mathbf{X}) > \epsilon$,  exists a corresponding epsilon delta accountability of $(\epsilon, \delta_0)$ and more generally $(\epsilon, \delta)$ where $\delta \leq \delta_0$.
\end{lemma}

\paragraph{proof} let $A_{\epsilon_0} = \{a \in M~s.t~\mathbb{P}(F(a) \in \mathbf{X}) > \epsilon_0,~a \neq P\}$ and $A_{\epsilon} =  \{a \in M~s.t~\mathbb{P}(F(a) \in \mathbf{X}) > \epsilon,~a \neq P\}$. Note $A_{\epsilon} \subseteq  A_{\epsilon_0}$ and thus by monotonicity of measures, we have $m(A_{\epsilon}) \leq m( A_{\epsilon_0}) \leq \delta_0$

\anvith{I sort of feel like these are all just lemmas, but then again I've seen some pretty short theorems in my life} 

\begin{theorem}[First theorem on passing epsilon deltas in chain]
Consider a given $P$, $F_1$, $X_1$ and space of proofs $M$ and measure $m$ that has $(\epsilon_1,\delta_1)$ accountability, and a $F_2$,$X_2$ with $\epsilon_2 \leq \mathbb{P}(F_2(x) \in X_2) \forall x \in X_1$. Then if $\delta \geq m(A_{\epsilon_1\epsilon_2})$ where $A_{\epsilon_1\epsilon_2}$ is with respect to $P$, then an epsilon delta accountability of $P$, $F_2 \circ F_1$, $X_2$ is $(\epsilon_1\epsilon_2, \delta)$
\end{theorem}

\paragraph{Proof} 
\begin{multline}
    \mathbb{P}(F_2 \circ F_1(P) \in X_2) \\ \geq \mathbb{P}(F_2 \circ F_1(P) \in X_2 | F_1(P) \in X_1)\mathbb{P}(F_1(P) \in X_1) \\ \geq \epsilon_1 \mathbb{P}(F_2 \circ F_1(P) \in X_2 | F_1(P) \in X_1) \\ = \epsilon_1 \int_{X_1} \mathbb{P}(F_2(x) \in X_2)\mathfrak{P}(F_1(P) = y|F_1(P) \in X_1) dx \\ \geq \epsilon_1\epsilon_2 \int_{X_1} \mathfrak{P}(F_1(P) = y|F_1(P) \in X_1) dx = \epsilon_1\epsilon_2
\end{multline}

and thus we have $\mathbb{P}(F_2 \circ F_1(P) \in X_2) \geq \epsilon_1\epsilon_2$ and thus if $\delta \geq m(A_{\epsilon_1*\epsilon_2})$ where $A_{\epsilon_1*\epsilon_2}$ is with respect to $P$, we have epsilon delta accountability of $(\epsilon_1\epsilon_2, \delta)$.

\begin{theorem}[Deducing epsilon delta from chain]
For a given $P$, $F_1$, and space of proofs $M$ and measure $m$, let $\{X_i\}_{i=1}^n$ be a finite partition of the output space of $F_1$, and $X_a$ be such that $\mathbb{P}(F_1(P) \in X_a) \geq \mathbb{P}(F_1(P) \in X_i) \forall i$. Then if $(\epsilon_0,\delta_0)$ is an epsilon delta accountability of $P$ for $X_2$ given $F_2 \circ F_1$, then letting $\delta \geq m(A_{\epsilon_0/n})$ where $A_{\epsilon_0/n}$ is with respect to $P$, we have $(\epsilon_0/n,\delta)$ is an accountability of $P$ for $X_a$ given $F_1$.

\end{theorem}

\paragraph{Proof}

\begin{multline}
    \mathbb{P}(F_2 \circ F_1(P) \in X_2) = \sum_{i=1}^n \mathbb{P}(F_2 \circ F_1(P) \in X_2|F_1(P) \in X_i) \mathbb{P}(F_1(P) \in X_i) \\ \leq \mathbb{P}(F_1(P) \in X_a) \sum_{i=1}^n \mathbb{P}(F_2 \circ F_1(P) \in X_2|F_1(P) \in X_i) \\ \leq n\mathbb{P}(F_1(P) \in X_a)
\end{multline}

so we have $\epsilon_0 \leq \mathbb{P}(F_2 \circ F_1(P) \in X_2) \leq n\mathbb{P}(F_1(P) \in X_a)$ and thus $\epsilon_0/n \leq \mathbb{P}(F_1(P) \in X_a)$ and so if $\delta \geq m(A_{\epsilon_0/n})$ where $A_{\epsilon_0/n}$ is with respect to $P$, we have an epsilon delta accountability of $P$ for $X_a$ which is $(\epsilon_0/n,\delta)$.

\begin{theorem}[Second Theorem on passing of epsilon delta in chain]
For a given $P$, $F_1$, and space of proofs $M$ and measure $m$, let $\{X_i\}_{i=1}^n$ be a finite partition of the output space of $F_1$, and $X_a$ be such that $\mathbb{P}(F_1(P) \in X_a) \leq \mathbb{P}(F_1(P) \in X_i) \forall i$. Furthermore let $\mathbb{P}(F_2 \circ F_1(P) \in X_2|F_1(P) \in X_i) > \alpha~\forall i$. Then if $(\epsilon_0,\delta_0)$ is an epsilon delta accountability of $P$ for $X_a$ given $F_1$, then letting $\delta \geq m(A_{n\epsilon_0\alpha})$ where $A_{n\epsilon_0\alpha}$ is with respect to $P$ and $F_2 \circ F_1$, we have $(n\epsilon_0\alpha,\delta)$ is an accountability of $P$ for $X_2$ given $F_2 \circ F_1$.
\end{theorem}

\paragraph{proof}

\begin{multline}
    \mathbb{P}(F_2 \circ F_1(P) \in X_2) = \sum_{i=1}^n \mathbb{P}(F_2 \circ F_1(P) \in X_2|F_1(P) \in X_i) \mathbb{P}(F_1(P) \in X_i) \\ \geq \mathbb{P}(F_1(P) \in X_a) \sum_{i=1}^n \mathbb{P}(F_2 \circ F_1(P) \in X_2|F_1(P) \in X_i) \\ \qeq n\mathbb{P}(F_1(P) \in X_a)\alpha
\end{multline}

Thus $\mathbb{P}(F_2 \circ F_1(P) \in X_2) \geq n\mathbb{P}(F_1(P) \in X_a)\alpha \geq n\epsilon_0\alpha$ and if $\delta \geq m(A_{n\epsilon_0\alpha})$ where $A_{n\epsilon_0\alpha}$ is with respect to $P$ and $F_2 \circ F_1$, then we have $(n\epsilon_0\alpha,\delta)$ is an accountability of $P$ for $X_2$ given $F_2 \circ F_1$

\begin{corollary}
\anvith{@for me: I think we can also pass the delta in the above is n=2}
\end{corollary}


==> Model%20Governance%20SoK%20draft/Contents/Unused/auditing.tex <==
\section{RM2: Auditing for ML}

\paragraph{Fairness without Awareness/Demographics}(Nick) The question I had was if we can train a fair model, or test if a model is fair for a group of people when we don't know/have the corresponding fairness attribute in our dataset. e.g. is it possible to train a model for people of all different colors even if we only have data on people of a subset of these colors? Moreover, is it possible to train a model fair for one aspect (e.g. skin color) even if we don't have this particular aspect in our mind (instead we just want to train a fair model in general)?

According to Natalie, there has been some works on “fairness without awareness”. In terms of “fairness without demographics”, Natalie recommended the following paper: \url{https://proceedings.neurips.cc//paper/2020/file/07fc15c9d169ee48573edd749d25945d-Paper.pdf}, "but there’s often a few assumptions you have to make about the data (here they make the assumption that the demographic subgroups are “computationally identifiable”)".

\paragraph{Auditing and logging}(Adelin) Audit logs may be useful to detect an attack while it is happening, perform post hoc correlation analysis over multiple records (a stronger model then current ML model defenses/cite lucy's work), or enable the reconstruction of event following an attack to identify the \textit{modus operandi} of the attacker and prevent the same attack from reoccurring. Businesses may have an obligation to collect logs due to business (for instance for credit card transaction as per PCIDSS standard) or legal requirement (financial institutions are required to report security incident and be capable of explaining the chain of event that lead to the breach or may see their practicing license revvoked). For instance, systems where ML logging is likely to be legally required are fraud detection and credit scoring due to their impact on humans [verify EU regulation draft]. 

There are a wide range of existing audit frameworks in traditional security (eg \url{https://cheatsheetseries.owasp.org/cheatsheets/Logging_Cheat_Sheet.html}). They are not readily applicable in ML due to the probabilistic nature of the domain (like how SISA is the only method to perform perfect unlearning so far). In the same way we can't readily use normal logging procedures for audit log generation. However, we could use proof of learning algos for audit logs. 

\textbf{Log overhead and format:} For ML, the information to be collected greatly differs from traditional event-driven logs used in network security. One may need to collect gradients, weights (which can be in the trillions) etc. Ideally, one would collect all possible information for each single input to the model, however in a real production system, log space is inherently finite. Overhead is already a major issue in non-ml audit log systems [Bates, OWASP] for which each individual record is small; the problem is only accentuated for audit logs of ML models and systems. Since SOTA models can be extremely large, a huge body of works focuses on model compression but models can still be in tens or hundreds of MBs making checkpoints prohibitive as a log solution. This also makes the log protocols like Common Event Format (CEF, used in syslog) and Common Log File System (CLFS, used in Windows event logs) inappropriate. These formats are extremely compact (\textit{e.g.} an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). Hence, a dedicated yet efficient log format must be designed from ground up for ML logging. One way to reformulate this is to state the logging problem as an optimization problem over a set of metrics that act as proxies, or correlate, to some task (debugging, security etc). In audio \textit{Travers et al.} suggest a security use case for ML logs for correlation analysis and hw an adversary could try to attack the logging system.%Observe that we cannot know in advance where the target error or attack will occur.


\textbf{What to log for each ML phase? (Adelin):} We need to distinguish the logging problem in the training/learning and in the testing phase for offline systems. In the training case, the relationship of a batch to the model weights change after the batch is of interest. In the testing case, the interest is in the relationship between the input and the model output prediction. For online training, there is a superposition of the two offline settings. For the rest of this definition we consider offline only.

\textbf{Formalizing the detection problem:} Logs are useful if they determine: which inputs (and time) a particular event $e$ in a set of interest $\mathcal{E}$ in has happened (\textbf{R1}) ---in contrast with unlearning methods like slicing which assume that the checkpoint to unlearn is known from a lookup table---, if possible the magnitude of this event (\textbf{R2}) and with the minimal amount of overhead computation/storage (\textbf{R3}). Lastly, we need to characterise the event $E$ either deterministically or from a set of heuristics correlated to the target event $\mathcal{H}_E$ of size $M=|\mathcal{H}|$ (\textbf{R4}). Storing each log entry or record $r$ has a given cost $c_r$ linked to its storage overhead. We thus want to find the optimal set of entries $\mathcal{R}$ and corresponding log frequency $k$ and $n$ attributes taken from $\forall e\in \mathcal{E} \mathcal{H}_\mathcal{E}$ given a budget constrain $\mathcal{B}$ and a target event reconstruction precision (defined for training poisoning below). 

Observe that these 4 requirements are close but slightly different from the OWASP recommendations for logs: what (type, severity, ), when (date/time), who (user id/ip etc) and where (script id, service name etc). We do not explore the private information retained in the logs as it is likely that it is the same as for ML models in genral and an open research problem. In this case PoL can't be used out of the box because a PoL does not tie back a computation proof to properties of the model and only considers steps that are likely to be spoofed by a \textit{forger}, that unduly claims to have done the computation. Nonetheless, the PoL framework identifies characteristics of the model (weights etc) and when these should be collected (every $k$ steps) with potential adjustments.  


\textbf{Practical application: towards training logs for model poisoning} Training time is a good security setting for a first analysis of optimal ML log generation because the attack surface is much more reduced than at test time and is mostly limited to poisoning[cite] and data reordering attacks[Ilia]. Due to the involved randomness at each step and its concern with the test time results, DP is not a good setting for training time logging.  On the contrary, poisoning is a good training logging problem because poisoning gradients can easily be identified from benign ones (as in the \textit{gradient shaping} paper), and hence there is a guideline to develop audit logs. In the training poisoning setting, the set of events $\mathcal{E}$ are posioning events. Thus, \textbf{R1} corresponds to logs that should enable to provide bounds on the batch and epoch numbers that were poisoned (and possibly the corresponding time) so that repair actions (a la Cao et al.) be taken. \textbf{R2} correspond to bounding magnitude of the corresponding weight update. In this case we can formally define the logging problem. \textbf{R3} is straightforward to formalize thanks to PoL and \textbf{R4} cannot be obtained deterministically but as per the gradient shaping paper, there are good heuristics one can use. 

\begin{definition}[ML Poisoning optimal audit logs]
Let $i\in \llbracket 1, I\rrbracket$ be the indices of all training batches. The logging problem is: find the minimal information and largest interval $k$ that should be recorded in a PoL such that all poisoning update batches indices $i_{\text{poison}}$ can be identified with a heuristic $h\in\mathcal{H}$ with a precision of at most $m$ steps ($\text{min}(k_j+m,k_{j+1})\geq i_{\text{poison}}\text{max}(k_j,k_{j+1}-m)$). In this case, there is a simple heuristic $h$: the norm of the weight gradient $\nabla \theta$ is larger then a threshold $T_{\text{poison}}$, $\norm{\nabla \theta}_2\geq T_{\text{poison}}$ .
\end{definition}

%\textbf{Remark:} The Log problem is an optimization problem over a finite set of controls.

\textbf{Implementation:} Ideally the logger would be implemented directly as an instrumentation in the ML compiler for instance with dedicated ops to limit performance impact which is critical in ML. It could also be implemented in python directly.

Anvith: this is pretty damn cool


==> Model%20Governance%20SoK%20draft/Contents/Unused/notes.tex <==
- Fair washing is auditing. Auditing is explanation done by a third party.



==> Model%20Governance%20SoK%20draft/Contents/Unused/ownership_large.tex <==
\newpage
\section{Establishing Identity in ML Systems}
\label{sec:ownership}

The notion of \textit{identity} is fundamental to computer security~\cite{bishop}. Identities identify principals involved in the system as actions are taken over the objects being manipulated by said system. Thus, identities are a prerequisite to holding principals accountable for failures of the system. 

\adelin{There is a mix up of different concepts Identity and ownership. While they are related trying to sell ownership research as IAM just doesn't really work. It reads like a tangential justification/fluff. I think that identity doesn't bring much to the table here as the identity property is not ML specific/already well established. Only ownership is ML specific/difficult to achieve in ML. }

Having described the principals typically involved in a ML system in \S~\ref{sec:principals}, we here outline how the concept of identities are relevant to machine learning. In particular, we focus on three objects of interest: the training and test data, and the learned model. In the following, we define {\em ownership} as the process of associating a principal with these two key components of a ML system. 
Later, in \S~\ref{sec:accountability}, we will then focus on how we can hold principals accountable for model failures once  identities relevant to data and models have been clearly established through the process of ownership.\adelin{This reads like a confusion identity/ownership. data/model are not identities imo. I would drop the identity argument altogether here.}

\nicolas{need to discuss role of authentication + access control} \adelin{I agree these are important but what is ML specific with those?}

\subsection{Data Ownership} 
\label{subsec:data_ownership}
\varun{data ownership is largely a legal discussion and can be written later.} \adelin{Why is it legal discussion? Do you mean under the privacy angle or under the private property angle?}


\paragraph{Training data} Data ownership is of paramount importance as data is one of the foundational pillars of a {\em functional} ML model. Understanding who collected the data can enable answering various questions regarding: (i) {\em representative:} if the collector paid attention to ensure that the data is truly representative\adelin{representative is representative is a tautology --- define the concept formally} of domain/concept shifts, (ii) {\em sanitization:} if the data is sanitized \adelin{same as for representative}of outliers, particularly poisons~\cite{} (which induce spurious performance in trained models)\adelin{problem here. Data cleaning is a common practice in practical ML use cases but real data is never really clean. This also disregards finance like domains where real data can shift extremely fast without being adversarial. Should we just ditch 2008 crisis data?Most likely not}, (iii) {\em fairness:} if the data collected is representative for the underlying task and various subgroups\adelin{elephant in the room: how are these subgroups defined, by whom? that is not very clear and very important}, and (iv) {\em feature engineering:} if the data was pre-processed correctly for various downstream tasks (such as private/fair learning).\adelin{feature engineering is great but is this work ML or DNN focused? rest of what I read is mostly DNN focused so this seems strange here}

\nicolas{The EU has special IP rights in relation to DBs but Canada and the US don't. There are some circumstances where copyright can protect DBs but also circumstances where it does not.
3:08
oops sorry — https://www.cigionline.org/static/documents/documents/Paper%20no.187_2.pdf
3:10
what people can control is access to physical hardware that they own — e.g. servers and computers that hold the DB. These physical assets are indeed owned (or they are owned by the company who provides it to the DB holder and then there is some arrangement about controlling access).
3:12
But the short answer (Teresa's paper gives a longer answer) is that you generally don't own information in Canada. You can own hardware and leverage this to control access. And you can have IP rights like copyright over information in some contexts.}

\nicolas{does a company own the fake paintings a GAN creates from artist paintings?} 

\paragraph{Test data} \nicolas{This is interesting because it will lead to confidentiality issues as in CaPC}

%https://arxiv.org/pdf/1906.10908.pdf

\subsection{Model Ownership} 
\label{subsec:model_ownership}

Model ownership is the process where, as defined, an actor claims ownership over the model. This is similar to what can be achieved with certificates for websites.\nicolas{add a reference and make this sentence a bit more precise}\adelin{I don't think any current model ownership technique give a guarantee on par with crypto certificates. When we write websites certificates do we mean X509?} As we explain in more details later, this often refers to ownership of the model's {\em sensitive parameters} that were obtained after the computationally expensive training process (especially in many deep learning applications). Defining ownership is necessitated by the existence of various threats that infringe it, such as insider exploits~\cite{} or reverse engineering efforts~\cite{}\adelin{reverse engineering makes sense, insider threat not at all. Or maybe you mean theft by an insider as protected by Data Loss Prevention systems (DLP). If it's the latter it should be reformulated because it currently appear like mixing concepts that don't have much in common. Avoid using the term exploit which refers very specifically to code that leverages a vulnerability}. The latter, formalized as model extraction~\cite{tramer2016stealing}, is the process where an adversary interacts with the model through a query interface to steal its sensitive/confidential parameters. 

\subsubsection{Model extraction}

By repeatedly posing queries to the trained model, the adversary is able to recover the model's functionality (a more nuanced discussion on what this means is presented later). 
Extraction is shown to be possible in various domains, such as images~\cite{matthew2020high}, text~\cite{krishna2019thieves}, audio~\cite{} \varun{lucas' work} and for simple hypothesis classes~\cite{varun2020exploring}, and more complicated ones such as DNNs~\cite{carlini2020cryptanalytic, rolnick2020reverse}; assuming white-box access~\cite{}, grey-box access~\cite{pmlr-v139-zanella-beguelin21a}, and more strict black-box regimes~\cite{milli2019model}. These threat models define what the adversary has access to:

\paragraph{Query-only} Truong et al. introduced a GAN-like method named Data Free Model Extraction (DFME)~\cite{truong2021datafree}, which uses a generative model to generate data that the victim and extracted models have the largest disagreement on. In other words, DFME maximize information extracted from the victim model that are not learned by the extracted model yet.

\paragraph{Unlabelled In-distribution Data}
In addition to the query access, some threat models also assume am unlabelled dataset from a similar distribution to the victim model's training dataset. This assumption is valid since online ML services usually state what tasks they could be used for (e.g. classifying digits). Then it is relatively easy for the adversary to collect some publicly available data related to the tasks (e.g. searching images of digits by Google). The goal of using such unlabelled data is also for query efficiency: the adversary wants to (a) select the data points that trains the extracted model faster by techniques such as Active Learning, as discussed by Chandrasekaran et al.~\cite{varun2020exploring}, and (b) leverage the rest of unlabelled data to help training by semi-supervised learning techniques such as MixMatch~\cite{berthelot2019mixmatch, matthew2020high}.

\paragraph{Other Information}
Batina et al. proposes a method named CSI-NN to extract DNNs under a very different threat model~\cite{batina2019csi}. The adversary takes advantage of side-channel information such as  timing and electromagnetic emanation and is shown to be capable of extracting the architecture and weight parameters of fully-connected DNNs or Convolutional Neural Networks.  

\nicolas{why not move this to the earlier portion where we said a more nuanced discussion will be presented later?}
Recall that earlier, we stated that the adversary recovers the model's {\em functionality}; Jagielski \etal~\cite{matthew2020high} provide a detailed taxonomy of what exactly an adversary can recover through this reverse engineering process, ranging from the exact model parameters to replicating functionality for specific data-points. The latter attacks are generally designed to achieve high \textit{accuracy}. This is usually the case when the adversary want to use ML models for their utility, but is unwilling/unable to collect training data and/or spend computational cost on training the models. The former class of attacks focus on high \textit{fidelity} (i.e., performing functionally similarly to the victim model). Such attacks can serve as a reconnaissance step to other attacks. For example, the adversary can create adversarial examples by the stolen copy to attack the victim model. These adversarial examples can be more easily transferred to the victim model since the two models are functionally similar. 

\subsubsection{Why is it impossible to prevent model stealing?}

Various defenses have been proposed over the years to prevent the adversary from learning enough information to build an extracted model~\cite{juuti2019prada} \varun{look at some of mario fritz' work}, but they are often rendered ineffective with an adaptive extraction strategy~\cite{}, or introduce utility degradation~\cite{}. 
Thus, Chandrasekaran \etal~\cite{varun2020exploring} state the inevitability of extraction, claiming that any utilitarian model can be reversed engineered through the interactive process that model extraction perform which relies on some form of {\em knowledge distillation}~\cite{}.

As mentioned in Section~\ref{sec:model_extraction}, the adversary's goal is to extract the model with as less queries as possible. Thus the defender could aim the opposite: restrict the information leaked by each query so the adversary has to make more queries. This could be done by having less significant digits in the outputs, or even adding noise to the outputs of the models~\cite{tramer2016stealing}. However, this does not make model extraction impossible unless the outputs are completely random, in which case the model's utility is seriously harmed. \adelin{if the output is completely random why even have a model and inputs??? that last sentence would benefit from a rewrite}

Instead of perturbing the outputs, other works first detect if a query may contribute to model extraction, and then either reject the query or even ban the user who submitted this query~\cite{}\adelin{how is the ban performed? some form of single account ban like fail2ban? If so it should be possible to register multiple API keys(one for your dog, one for you etc) to simply bypass these anti-extraction methods}. This is intuited by the use of synthetic dataset in many attacks, which are likely to be from a different distribution than the training dataset. However, by construction, such defenses are vulnerable against attacks using unlabelled in-distribution data~\cite{}.\adelin{and abusive user registration to disperse clues}

\subsubsection{What is model ownership?}

We now turn to techniques that assume that model stealing will be impossible to prevent, and instead allow model owners to create claims of ownership that are robust against such infringement. But in order to claim ownership of a model, one must first define what constitutes a model.

\paragraph{Functionality} As intellectual properties, the value of ML models comes from their functionalities (e.g., the ability to classify hand-written digits)\adelin{Sentence somewhat reads off because the value of a model comes more from the difficulty of creating it (what's rare is expensive) than from the fact that it is IP (which is anecdotal since IP can refer to trivial to create things).}.\adelin{Sentence is very much GAFAM focused. Most corps don't use DNN like models that are computationally expensive but rather SVM where feature engineering is the important step. Afaik Florian's work steals the parameters of random forest/svm but not the feature used right?} This is also usually the target of ML model thieves\adelin{Do these exist in real life? sentence reads off as creating your own problem just to provide ways to solve it}. However, functionality is a very abstract concept. The model owner cannot frame the functionality of his/her model in a way that can be compared with others and used as a claim.\adelin{vague. I think i see what is meant here but would benefit from refinement}

\paragraph{Parameters} When people implement ML models, they usually use the word "model" to refer to the function composed of operations (i.e., architecture of the model) and parameters (e.g., weights and bias).\adelin{By oposition to? previous sentence reads like a tautology. Maybe refer to the FAIL paper/proof of learning for proper definition of what a model is?} With these pieces of information, one can obtain the model and use it for inference. The issue with this is that despite one set of parameters map to certain functionality, the reverse is not true: mapping from functionality to sets of parameters is 1-to-N (i.e., models with different parameters can have the same functionality). This leads to a line of attacks on model ownership: model extraction attacks~\cite{tramer2016stealing} which tries to steal the functionality of ML models but not the exact parameters (so it is harder to be caught). It will be discussed with more details in Section~\ref{sec:model_extractio}. 

% Nicolas: I think this is a technique not a definition of a model
% \paragraph{Training-time Information} This is intuited by the fact that all ML models are trained, and only the trainer of the model has done the computation on training. Since there exists some information during training that are not included in the final model for inference (e.g. intermediate checkpoints, training data, etc.), ownership claims can be made once we show an unforgeable connection between these information and the trained ML model. One representative example is the Proof-of-Learning~\cite{jia2021proof} which can be used as a claim robust against model extraction attacks. 
However, here it is assumed the trainer of the model is the owner of the model, so there might be some improvements needed when this is not the case (e.g., the trainer sells the model to another party).\adelin{vague. I think that the paper would benefit form identifying the roles rather then identities so that these mappings are clearer} \adelin{the Point is great though! in al,ost all ownership lit trainer is conflated with modek owner. If that's not the case then contractual agreements (along with passing some secret info) might be the only way to deal with things as in cloud settings.}


\subsubsection{How to claim model ownership?}

Ownership is generally claimed by demonstrating that one has knowledge about training which the adversary cannot have if they have not trained the model. This knowledge can result from an explicit modification of the training procedure (as we will see first with watermarks) or be inherent to the training procedure itself (as covered in our discussion below of proof-of-learning and dataset inference). The goal of the model owner is in essence to prove that they trained the model before the adversary gained access to it. 

To prove ownership, the process of {\em watermarking} was considered a promising solution. Here, the model owner encodes a specific query response pair into the training procedure, and can verify if a model is indeed their own on observing such behaviours at the time of inference~\cite{adi2018turning}. This process is fundamentally similar to the concept of {\em backdooring}~\cite{}, without any adversarial intent. However, recent work demonstrates that watermarking is not resilient to model extraction efforts~\cite{jia2020entangled} due to large model capacity (in the case of DNNs), potentially resulting in sub-networks being learnt for (a) the legitimate task, and (b) the watermarking task. Jia \etal~\cite{jia2020entangled} propose an alternative approach which entangles internal representations for both tasks, resulting in a watermarking technique resilient to extraction, but with a nominal performance penalty. 

Previous detection proposals rely on encoding specific types of {\em secret information} into the training algorithm. New research suggests that there exists various forms of secret information available to the true model owner, obtained during the process of training. This includes the order in which data is sampled, intermediate checkpoints, hyperparameter values, the intermediate values of model weights, etc. One proposal to prove model ownership relies on the honest model owner logging such information during the training procedure. Since DNN training is a stochastic process, the intermediary states obtained during training are {\em hard to guess} without access to the secret information aforementioned. If a trusted third party can reproduce these states (within some acceptable tolerance threshold) with the help of the honest party's secret information, then the honest party's ownership of the model is validated. This is the premise of the {\em proof-of-learning} approach to enable ownership~\cite{jia2021proof}. 
Instead, an adversary is unable to guess a valid sequence of intermediate model weights because the cumulative noise introduced by the training algorithm and high dimensionality of the parameter space make it impossible to get the same model twice without access to the honest party's intermediate training information. Despite having a large computational and storage footprint, proof-of-learning innovates by providing not only an ownership claim but also a token of identity for the model owner.

\subsection{Is model ownership separate from data ownership?} 
Another proposal from Maini \etal~\cite{maini2021dataset} flips this approach to model ownership: they rely on the honest model owner's knowledge of the proprietary data used to train the model to prove ownership. \nicolas{Mohammad should write something here, explaining that in fact model ownership is not separate from data ownership since in dataset inference we use data ownership to assess model ownership. this will be a nice conclusion to the section}
is intuited by the fact that the extracted model is either trained on data labelled by the victim model, or data from the training distribution of the victim model. Therefore, the model owners only need to keep their training data, and are able to claim ownership of a stolen model if it has very high confidence on data points that are in-distribution for the victim model. In other words, Dataset Inference is able to detect if two models are trained on the same dataset. Therefore, the drawback is that Dataset Inference cannot protect ownership of DNNs trained on public datasets. 
\nick{@Mohammad you are the expert of this, feel free to modify/extend this paragraph}



==> Model%20Governance%20SoK%20draft/Contents/themes.tex <==
\subsection{Risks}
\label{ssec:risks}

We highlight three classes of risks relevant to ML governance that have been studied extensively in the literature. We also outline different failure modes inducing these risks (that can occur at different stages of the ML pipeline). Awareness of the risks present provides design goals and considerations that impact the creation, deployment, and retention of the model, and these failure modes will later shape our discussion on accountability and assurance in \S~\ref{sec:accountability} and~\ref{sec:assurance}. Though we do not exhaustively cover all risks due to space constraints, the governance aspects which constitute this paper are generic and can be expected to generalize to other risks. %\todo{adelin again this is not a real risk as in a model could be unfair and not lead to any resulting harm due to a bunch of factors (gabe an I have such discussion for finance and AEs). I think you need to map real examples to accepted definitions of risks. Happy to help refine these definitions and claims too nicolas I think as a response to Adelin's comment here we should lift the discussion of risk in this subsection here to the entire ML application/pipeline rather than just the model
%  yeah I think that would work. @mohammad: please ping me for that}



%\label{subsubsec:integrity}

\vspace{1mm}
\noindent{\bf 1. Integrity:} Losing integrity (\ie correctness of the system outputs) is the immediate risk that a model owner tries to minimize, for example, via training the most accurate and robust model. The integrity of a model needs to take into account the overall system this model is deployed within. Integrity risk quantifies the lack of alignment between the output of the ML system and what was expected from it. 

The {\em accidental failures} that cause integrity risks stem from the reliance of ML models on data; data used to train models need to possess specific properties and must be (pre-)processed in specific ways to enable effective training (\S~\ref{subsec:data_ownership}). This  ensures that models are resilient to {\em outliers} (data points that are outside the range of those expected)~\cite{gudivada2017data,cortes1995limits}. Another failure mode for integrity is that of {\em concept drifts} (where the distribution of data changes over time)~\cite{lu2018learning,koh2021wilds}. Collectively, both these issues result in the model failing to generalize. 

% \anvith{@Varun cited the big survey paper on concept drift above, perhaps below comments are less relevant now? I commented them out for the time being}

%\varun{loads of relevant papers:
%\url{https://cs.stanford.edu/~pliang/papers/}; also check out ludwig schmidt's work}. Collectively, both these issues result in the model being unable to generalize. \varun{@anvith: can you use google doc to add papers from percy + ludwig which are relevant to this topic?} \anvith{added a couple papers on concept drift, I only found two relevant papers from percy liang which I added to the google sheet (but I could be slighlty blind), and from that I think only one really fits with the discussion and even then not really}


%\anvith{following is new and feels very forced, in particular the last citation, I think it was before without it (we talk about this stuff anyways later)} Different approaches have been proposed for dealing with learning under such situations: Lu \etal \cite{lu2018learning} reviewed past approaches, and new approaches have worked on understanding how better to adapt \cite{kumar2020understanding}. 


{\em Adversary-induced failures} follow. At training time, adversaries incorporate \textit{data poisons} (which are specifically perturbed data points) which result in poor generalization (\ie indiscriminate poisoning attacks~\cite{munoz2017towards}), or targeted misclassification (\ie targeted poisoning attacks~\cite{munoz2017towards}). Poisoning adversaries can assume that the data collector uses the labels provided with the poisons, or can also specify their own labels~\cite{shafahi2018poison,zhu2019transferable}. The former is known to be ineffective for large parameterized models~\cite{suciu2018does}, while the latter is effective across the spectrum. Poisoning is effective across a range of learning paradigms~\cite{carlini2021poisoning,ma2019policy}, and across different threat models~\cite{fang2020local}. Backdoor attacks use a different strategy; a specific {\em trigger} pattern induces a misclassification, and can be added to {\em any input} whilst generic poisoning ensures misclassification of inputs belonging to a particular class~\cite{liu2017trojaning}.

During inference, adversaries can strategically modify inputs  called \textit{adversarial examples} (whilst ensuring that they are indistinguishable from their benign counterparts). This induces a misclassification~\cite{szegedy2013intriguing,biggio2013evasion}. These evasion attacks are known to be effective across a wide range of hypothesis classes~\cite{szegedy2013intriguing,goodfellow2014explaining,vernekar2019analysis,shafahi2018adversarial,papernot2016limitations},
% \todo{broken cite}
and learning frameworks~\cite{lin2017tactics,behzadan2017vulnerability,kos2018adversarial}. Initially introduced in vision~\cite{szegedy2013intriguing,biggio2013evasion}, evasion has now been demonstrated for a wide variety of domains including audio~\cite{carlini2018audio,yakura2018robust,qin2019imperceptible} and text~\cite{ebrahimi2017hotflip,alzantot2018generating,garg2020bae,zhao2017generating}. Attacks can also be physically realized~\cite{kurakin2016adversarial,yakura2018robust,Lovisotto2021slap} and constrained such that samples generated for evasion preserve input semantics~\cite{qin2019imperceptible,alzantot2018generating,dreossi2018semantic,jain2019analyzing,qiu2020semanticadv,sheatsley2021robustness}.

\vspace{1mm}
\noindent{\bf 2. Privacy:} Data is fundamental to training. Research has demonstrated how models trained without privacy considerations can leak sensitive information~\cite{shokri2017membership,carlini2019secret}. This has raised concerns about the use of data containing sensitive information and its consequences for individuals and groups alike. Thus, privacy is increasingly becoming a societal norm~\cite{boyd2010privacy}. This is perhaps best illustrated by  legislative work seeking to adapt protective regulations such as the GDPR to the context of ML applications~\cite{gdpr}. Thus, setting aside the value of upholding privacy as a human norm, growing regulation of data usage means that it is in the interest of model owners to respect privacy-preserving practices. Indeed, not mitigating privacy risks in their ML applications could result in a poor reputation for the model owner and compliance complications. 

Additionally, memorization of training data is essential for generalization of ML models~\cite{feldman2020does,Feldman2020what}, and recent work shows encouraging the model to memorize may help its performance and convergence rate~\cite{Katherine2021Deduplicating}. However, memorization could also lead to {\em accidental failures}: a model can memorize sensitive data, such as credit card numbers, inadvertently~\cite{carlini2019secret}. Such secret information may then be leaked at inference time, \eg when the model tries to auto-complete a sentence talking about credit cards. As shown by the authors, the only effective method among those evaluated is differentially private training~\cite{abadi2016deep}, often at the expense of model performance.

There are also known {\em adversary-induced failures}. In a {\em membership inference attack}, an adversary wishes to determine if a given data point was used to train the model. Adversaries  initially assumed  access to confidential information from the black-box model~\cite{shokri2017membership} which was shown sufficient to determine membership. Following this,  research has further improved (and simplified) black-box attacks~\cite{salem2018ml,song2019privacy,jayaraman2020revisiting,truex2019demystifying,yeom2018privacy}, for instance by performing label-only attacks~\cite{li2020label,choquette2021label}. Instead, white-box attacks further leverage information held in model parameters~\cite{sablayrolles2019white,leino2020stolen,song2017machine,nasr2019comprehensive}, or gradient updates~\cite{melis2019exploiting}. 

%Yeom \etal~\cite{yeom2018privacy} draw the connection between the efficacy of membership inference and overfitting. Based on this insight, various defences have been proposed~\cite{shokri2017membership,jia2019memguard,nasr2018machine}. However, they fail to provide meaningful guarantees of privacy as demonstrated  by Song \etal \cite{song2021systematic} with the introduction of the privacy risk score which still strongly correlates with membership despite these various defences being employed. However, Yeom \etal~\cite{yeom2018privacy} note that training the model to obtain differential privacy  does reduce a membership inference's efficacy; drawing  theoretical connections between the efficacy of the attack and the privacy budget ($\varepsilon$) (in particular bounding the efficacy of such an attack) along with others~\cite{erlingsson2019we,jayaraman2020revisiting,sablayrolles2019white}.
% Thus, as of now, the one promising defence against an membership inferenceis to train with differential privacy. 

Beyond membership inference, other attacks attempt to reconstruct data. In  attribute inference attacks, the adversary attempts to impute missing values in a partially populated record using access to an ML model~\cite{jia2018attriguard}. Model inversion attacks aim to reconstruct data points that are {\em likely} from the training dataset. In the classification setting, Fredrikson \etal~\cite{fredrikson2015model} exploit confidence information from the prediction vectors (based on the same overfitting assumption made earlier). With a similar intuition, Yang \etal~\cite{yang2019neural} use an autoencoder to reconstruct the input from the confidence vectors, while Zhang \etal~\cite{zhang2020the} use GANs to aid reconstruction.  
%Note that the aforementioned attacks are possible when the model is fully trained.\todo{missing word in prev sentence}
More recent attacks (applicable in distributed training regimes, such as federated learning~\cite{konevcny2015federated}\footnote{Federated learning is a paradigm where multiple clients jointly learn a model by training a local model on their private datasets and sharing gradients which are aggregated at a central entity.}) enable successful reconstruction from gradients~\cite{geiping2020inverting,nasr2019comprehensive,melis2019exploiting, hitaj2017deep,wang2019beyond, song2020analyzing}. %Again here, training with differential privacy is proposed as a technique to defend against data reconstruction. In the federated learning setting, this has been studied and deemed effective~\cite{geiping2020inverting}.\todo{}\anvith{added one} 




%\paragraph{Fairness} The third overarching risk class is \textbf{fairness}.
\vspace{1mm}
\noindent{\bf 3. Fairness:} ML models rely on extracting patterns in data, and 
%there is no question that 
unwanted biases are reflected within historically-collected data~\cite{lum_predict_2016, mattu_machine_nodate}. 
% \adelin{cite to substantiate claim}\mohammad{done}
Unmitigated, these biases transfer into algorithmic decisions that are fed back into the decision making process, thus aggravating the situation. Furthermore, algorithmic decisions themselves can also encode new biases that were not initially present in historical data~\cite{bagdasaryan2019differential}; this may be due to poor quality~\cite{suresh_framework_2021}, and even the careless use of fairness constraints.~\cite{cost_of_fairness}
% \todo{}\mohammad{done}

Like integrity and privacy, the challenges of algorithmic fairness can be considered through the lens of attacks and defenses. One can consider, for example, a prejudiced adversary that attempts to sabotage a model performance against a particular sub-group; but this also risks the integrity of the model. But does guaranteeing integrity mean that we have ensured fairness? The answer is no.



% \anvith{@Mohammad, @Varun, @Someone, missing attacks for this}
Unlike integrity and privacy, fairness risks largely stem from data collection and processing steps. In an ideal world, (i) we would have balanced datasets to train our models on, and (ii) the predictions of models would apply equally to different members of the population which would, in turn, ensure future balancedness of our datasets because model contributions\footnote{Indeed, it is common for model predictions to be incorporated as training data in the future, as can be the case for instance with online learning.} to historical data would be balanced.  But in most areas of critical concern in algorithmic fairness, neither is the case because there is a \textit{de-facto} sampling process often (implicitly) encoded in the processes that produce the data collected~\cite{mitchell_algorithmic_2021}; an essential factor that should thus be considered under data collection. For example, in pre-trials where a judge has to assess the risk of accepting or rejecting bail, the defendants are only being subject to algorithmic predictions because they have been arrested in the first place. Mitchell~\etal~\cite{mitchell_algorithmic_2021} provide a broad overview on various fairness risks associated with three broad categories: (i) {\em data bias:} both statistical--which evolves from lack of representation (\ie selective labels~\cite{selective_labels}), and societal--which indicates a normative mismatch~\cite{suresh_framework_2021}; (ii) {\em model bias:} influence of choice of hypothesis~\cite{chouldechova2017fairer} and even interpretability, and (iii) {\em evaluation:} how today's predictions can alter decision subjects' behaviors, thus requiring new predictions in the future. We will discuss such performative qualities of models in \S~\ref{subsub:performative}.


We quickly note that alleviating fairness risks in the ``ideal'' way above, would inherently be incompatible with controlling privacy and integrity risks, since our samples sizes are limited by the size of the smallest sub-population, which potentially limits the generalization of our models which not only threatens integrity but can also have adverse effects on privacy~\cite{shokri2017membership}.

==> Model%20Governance%20SoK%20draft/Contents/users/adelin.tex <==
\subsection{Auditing to Identify New Model Failures}

\nicolas{we need to read the auditing chapter in bishop p689 and see how logs need to be incorporated in this whole thing. typically auditing is logging + analysis. here we mean more that a regulator is querying a model to figure out what its limitations are (more or less what its attack surface is). so we might need to rethink this subsection}

We first define ML auditing and present how ML logging can support it. %examine the types of auditing that can be conducted in the context of machine learning models. 
We then overview adequate ML logging procedures as well as storage, privacy and security open problems in ML logging.

%\varun{@adelin: the flow should answer the following questions: 1. how logging can help identify principals responsible for the aforementioned "bad events" --$>$ this is a more broad discussion; 2. why is logging for mL hard --$>$ this is also a broad discussion; 3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons); 5. how should it be logged (storage + computation costs); 6. compare + contrast with logging in practice}


\vspace{0.5mm}\noindent{\bf How can ML logging support ML auditing?}
For systems, Bishop~\cite{bishop} defines an audit as a formal examination by a (third) party to determine a chain of events and actors. In the case of ML models, this definition must be extended to include the verification of claimed properties of a model.
As noted in section \ref{sec:principals}, the different logical entities may in practice refer to the same principal. Hence, we call an audit \textit{internal (resp. external)} when the model owner and auditor are the same entity (resp. independent entities). Observe that an internal audit is a proactive action, similar to a white-box assessment, and may rely on model \textit{logs}. On the contrary, an external audit is a policing action, similar to a black-box assessment, and may only rely on model querying. Similarly, accountability and attribution are the same problem viewed respectively internally and externally. 
%This apparently simple distinction provides deep insight. %This distinction is important and provides deeper insight than its apparent simple nature.
%To explicit the benefits of this model, we make a number of observation. 
%First, an internal audit is a proactive action, similar to a white-box assessment, and may rely on model \textit{logs}. On the contrary, an external audit is a policing action, similar to a black-box assessment, and may only rely on model querying. Second, 
%and internal audit results correct 
This apparently simple distinction provides deeper insight as (i) verifying that internal techniques are properly implemented may be straightforward for a regulator and (ii) leveraging internal logs may alleviate technical limitations of an external audit. %, than to perform an external audit by querying a model in black-box fashion. 
For instance, the model deletion code of SISA unlearning of Bourtoule \textit{et al.}~\cite{bourtoule2019machine} can be reviewed for correctness (as in (i)) while model unlearning external verification remains a largely open problem (as in (ii)). Hence, internal audit can support external audits and regulators should be flexible in mandating audit approaches. Regulators should require the most appropriate of internal or external audits depending on the technical feasibility of verifications under each perspective. 

%The external auditing perspective is common in the literature on security and privacy of ML and is covered in a number of related SoKs\cite{}\adelin{Adi, nicolas, @mohammad: privacy and fairness examples?, could also add milad's paper}. 


%3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons);
%ML logs for properties or for principal actions




%Model owners may have an obligation to collect logs due to business (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pcidss_2015}) or legal requirement (financial institutions are required to report security incident and be capable of explaining the chain of event that lead to the breach or may see their practicing license revoked). 
%For instance, ML logging may be need to comply with the credit card transaction PCI-DSS standard~\cite{noauthor_pci_2020} while the EU AI regulation draft~\cite{eurlex_nodate} would fraud detection and credit scoring due to their impact on humans may require ML logging according. 

\vspace{0.5mm}\noindent{\bf Why is logging hard for ML?}
Knowing what and when to log is non trivial and highly use-case dependent. In response, logging guidance have been established in non-ML applications~\cite{owasp_logging,noauthor_pci_2020}. These guidelines are not readily applicable in ML due to the (i) probabilistic nature of ML, (ii) ML-specific steps, like training, of the life cycle and (iii) the need to focus not only on identify principals responsible for a specific input but also on tracking certain model properties. %Common log formats,\textit{ e.g.} the format used in syslog~\cite{gerhards_syslog_2009}, are inappropriate for ML as they are designed to compactly log network or system events (for instance storing only an event's time, type and name). 
Consequently, the ML logged information may greatly differ from traditional event-driven logs used in application, network and system security. 

\vspace{0.5mm}\noindent{\bf What and when to log?}
Ideally, one would collect all possible information regarding the model and inputs, however in a real production system, log space is inherently finite. ML model owners should first define the life cycle step and threat they want to mitigate with logging. At train time, model owners should log model parameters that track the property of interest. During the deployment phase, model owners may further have an obligation to collect logs due to business (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pci_2020}) or legal requirement (the EU AI regulation draft~\cite{eurlex_nodate} may require ML logging of fraud detection and credit scoring due to their impact on humans). Consequently, the model owner may need to collect gradients, weights, hyperparameters, model inputs along the corresponding principals or any other information.  Despite efficient formats for network or system events, \textit{ e.g.} the format used in syslog~\cite{gerhards_syslog_2009}, overhead is already a major issue in non-ml audit log systems~\cite{bates_trustworthy_nodate,owasp_logging}. This problem is only accentuated for ML models as models can have trillions of parameters~\cite{} and inputs may have high dimensionality. %Common log formats,\textit{ e.g.} the format used in syslog~\cite{gerhards_syslog_2009}, are inappropriate for ML as they are designed to compactly log network or system events (for instance storing only an event's time, type and name). 
Hence, standard ML logging guidance and a dedicated yet efficient ML log format must be designed from ground up. 

Despite the upstart of a number of industry ML logging tools and practices (both for the model and underlying system performance)~\cite{google_monitoring, mlflow_log, fiddler_monitoring_nodate,amazon_log,noauthor_whylogs_2021}, only little academic work has delved into ML logging.\adelin{I have not checked bias and fairness lit} We highly two works which, despite not explicitly referring to logs, can be thought to provide a form of training time logs. The Proof of Learning framework from Jia\textit{et al.}~\cite{jia2021proof} saves a model weights to enable internal audit against model extraction attacks\adelin{@mohammad please verify this}. Hong \textit{et al.}~\cite{DBLP:journals/corr/abs-2002-11497} leverage gradient information at training time to identify and mitigate model poisoning. For deployment time, Chen \textit{et al.}~\cite{DBLP:journals/corr/abs-1907-05587} utilize input correlation to identify model queries made in preparation of an adversarial example based attack. In the audio biometrics domain, Travers \textit{et al.}~\cite{travers2021exploitability} show how compliance-driven ML input logs can be leveraged for malicious authentication investigation (similar to Transition-Based Auditing which targets known attempts to breach security~\cite{bishop}).

%Ideally, one would collect all possible information for each single input to the model, however in a real production system, log space is inherently finite. Overhead is already a major issue in non-ml audit log systems~\cite{bates_trustworthy_nodate,owasp_logging} for which each individual record is small; the problem is only accentuated for audit logs of ML models and systems (SOTA models can have trillions of parameters~\cite{}).  %These formats are extremely compact (\textit{e.g.} an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). 
%Hence, a dedicated yet efficient log format must be designed from ground up for ML logging.



%These formats are extremely compact (\textit{e.g.} an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). 

%A wide range of existing frameworks in traditional security (eg \url{https://cheatsheetseries.owasp.org/cheatsheets/Logging_Cheat_Sheet.html}). They are not readily applicable in ML due to the probabilistic nature of the domain (like how SISA is the only method to perform perfect unlearning so far). In the same way we can't readily use normal logging procedures for audit log generation. However, we could use proof of learning algos for audit logs. 

%Since SOTA models can be extremely large, a huge body of works focuses on model compression but models can still be in tens or hundreds of MBs making checkpoints prohibitive as a log solution.
%\varun{motivate why checkpoints can be used for logging a bit better; the next para does that well}

%"Logging is the collection of information; auditing is its analysis."
%A bit reducing the audit process but acceptable
%"Last comes auditing. Commercial systems emphasize recovery and accountability. Auditing is the process of analyzing systems to determine what actions took place and who performed them. Hence, commercial systems must allow extensive auditing and thus have extensive logging (the basis for most auditing). Logging and auditing are especially important when programs move from the development system to the production system, since the integrity mechanisms typically do not constrain the certifier. Auditing is, in many senses, external to the model." bishop
%Basically external is when the enforcement arm of the auditor is mandated by someone other than the model owner and internal is when the model owner and regulator enforcement are conflated
%attribution is external under that view while accountability is internal.
%in acountability the model owner proactively makes the model identifiable in case of a problem.
%In attribution the model owner is trying to evade being linked to a specific model
%often, a lot of the research is written under the assumption that the model is productized or whatever and external entities find issues that require resolution. auditing + logging seems to be the only internal concept that’s interesting, that i can think of. anything i am missing?
%I think there is: internal can help exernal. See it as internal ~= whitebox, external ~= blackbox. (edited) 
%Then proof of learning is internal whereas radioactive data is somewhat external
%internal can help external -> that also makes sense. and this concept holds across, right?
%Yep. In financial audit a regulator requires both external and internal audit
%Audit logs may be useful to detect an attack while it is happening, perform post hoc correlation analysis over multiple records (a stronger paradigm then current ML model defenses/cite lucy's work), or enable the reconstruction of event following an attack to identify the \textit{modus operandi} of the attacker and prevent the same attack from reoccurring. 





%"The first goal is to detect any violations of a stated policy; the second is to detect
%actions that are known to be part of an attempt to breach security." bishop

%\vspace{0.5mm}\noindent{\bf Existing work}
%6. compare + contrast with logging in practice
%The external auditing perspective is common in the literature on security and privacy of ML and is covered in a number of related SoKs\cite{}\adelin{Adi, nicolas, @mohammad: privacy and fairness examples?, could also add milad's paper}. 




%\vspace{0.5mm}\noindent{\bf Security and privacy of ML logs}
% 2. why is logging for mL hard --$>$ this is also a broad discussion;
%   5. how should it be logged (storage + computation costs); 
 %
%We identify 2 major open issues with ML logging, respectively log sanitization and storage overhead.
\vspace{0.5mm}\noindent{\bf What else should be considered in ML logs?}
Lastly, when designing an ML auditing system based on logs, the privacy and security of that system itself should be taken into account. While standard logging and backup protection guidelines~\cite{owasp_logging,noauthor_pci_2020} should be employed where relevant, we delve further into two ML specific issues. First, since logs may be accessed by auditors, they represent a risk and must be sanitized~\cite{bishop}. As outlined in section \ref{sec:model_extraction} the case of ML, such risks include model inversion and membership inference techniques. This is problematic since techniques such as differential privacy target the training phase rather than already existing sets of weights\cite{}\adelin{Would appreciate help in finding the correct citation}. Second, adversaries may try to evading simultaneously the ML model and supplementary log analysis system as performed by the new class of \textit{surreptitious adversarial examples} introduced in Travers \textit{et al.}~\cite{travers2021exploitability}. This type of attack may be facilitated if both the target system and log analysis module are ML based, indeed Travers  \textit{et al.}~\cite{travers2021exploitability} instantiate the surreptitious adversarial example class with a joint optimization attack. Similarly, Chen \textit{et al.}~\cite{DBLP:journals/corr/abs-1907-05587} introduce query blinding to attack their stateful detection system.

%\textit{Travers et al.}~\cite{travers2021exploitability} introduce \textit{surreptitious adversarial examples}, a new class of attack evading simultaneously the ML model and supplementary log analysis system. They instantiate this class with a joint optimization attack. %Whereogging systems should be resilient to these attacks.

%complex as Proof of Learning Logs are essentially a snapshot of a model while spectrogram logs could be inverted 




%One way to reformulate this is to state the logging problem as an optimization problem over a set of metrics that act as proxies, or correlate, to some task (debugging, security etc). 

% \adelin{It seems that you are confusing 2 concepts. Log based auditing/monitoring (internal) and external auditing. They are related but not the same.  Internal information helps speed up external audit but is not required in the same way whitebox is great for security analysis but adversaries may operate in a blackbox paradigm. Happy to help formalize/write this now that I have time.}

% \adelin{The paper would benefit throughout from an internal vs external audit perspective as explained in slack: 
% Basically external is when the enforcement arm of the auditor is mandated by someone other than the model owner and internal is when the model owner and regulator enforcement are conflated
% Adelin:shell:  5 hours ago
% attribution is external under that view while accountability is internal.
% in acountability the model owner proactively makes the model identifiable in case of a problem.
% In attribution the model owner is trying to evade being linked to a specific model
% Varun  5 hours ago
% that makes sense, but i don’t think there’s anything interesting/unique to talk about when we are discussing “internal” related concepts right? often, a lot of the research is written under the assumption that the model is productized or whatever and external entities find issues that require resolution. auditing + logging seems to be the only internal concept that’s interesting, that i can think of. anything i am missing?
% Adelin:shell:  5 hours ago
% I think there is: internal can help exernal. See it as internal ~= whitebox, external ~= blackbox. (edited) 
% Then proof of learning is internal whereas radioactive data is somewhat external
% Varun  4 hours ago
% internal can help external -> that also makes sense. and this concept holds across, right?
% Adelin:shell:  4 hours ago
% Yep. In financial audit a regulator requires both external and internal audit
% It could help with the compliance thing: a lot of techniques which are hard externally may be easy internally. Hence we could argue that a regulator doesn't legally enforce external audit but legally requires internal techniques. It;s easier to check that internal techniques are properly implemented (hence the results are correct) than to actually do the external check in a few cases}



==> Model%20Governance%20SoK%20draft/Contents/users/adelin_governance.tex <==
% \newpage
\section{Defining ML Governance}

% \url{https://medium.com/data-science-at-microsoft/machine-learning-model-governance-at-scale-26c9a2dc15b5}

% \mohammad{discussed this with Varun. ML governance is a quite well-studied operations management concept in the industry with several well-established systems (usually under the name of data mining). While this is likely not the angle we want to define our take on the problem; we have to consider at least one (generic) such system and point out that our life cycle fits within those systems reasonably well. It could be IBM's \href{https://en.wikipedia.org/wiki/Cross-industry_standard_process_for_data_mining}{standard}.}

% \nicolas{somewhere in here we should discuss assumptions about trust see p11 bishop}


\subsection{Definition}

Conceptually, ML governance can be thought of as a set of solutions for balancing the benefits of applying ML with the risks it creates, often at the level of society. Put another way, governance is a prerequiste to build trust between principals involved and affected by a ML development. We describe such principals in detail in \S~\ref{sec:principals}, but for now it is useful to assume that they are three types of principals: the model owner (\ie the company or institution creating and deploying the model), the end user, and a regulator. Governance imposes constraints on how principals interact throughout the lifecycle of a ML application (as covered previously in \S~\ref{ssec:lifecycle}). 

The benefits of a ML pipeline are often application specific. Typically, these benefits are defined by or at least motivate the model owner, \eg applying ML will generate profit for a company. 
%Every model owner would like to maximize their model performance w.r.t. a given metric, such as accuracy. 
One may think that the model's usefulness (i.e. utility) is tied to a performance metric (\eg accuracy) and every other consideration can only decrease it. This is true if we view training as an optimization problem: a constrained problem can only produce solutions at most as good as its unconstrained counterpart. However, other considerations may be just as important than utility---in particular at steps of the life cycle before or after training. 
%For instance, consider labeling of images which is a well-studied supervised learning task where state-of-the-art models have long surpassed human-level accuracy\adelin{citation missing}. However,  these models often fail to \textit{generalize} when they are deployed in the real world~\cite{}. For instance, their decisions may not be robust to imperceptible changes to the input (e.g. a perturbation which does not affect the semantics of the input can completely change a model's decision~\cite{}); or they may leak information about their training sets (e.g. presence of a particular individual in the training set). Furthermore, 
For instance, model decisions may demonstrate significant unwanted biases (e.g. misclassifying individuals from minorities) and prompt the model owner to reassess their data collection and algorithmic choices. Thus, deploying ML comes with inherent \textbf{risks} to the different principals interacting with the ML pipeline:
%Seen through the lens of risks, the utility of the model (or lack thereof) can also be seen as a risk.\adelin{That last sentence is not understandable. Do you mean that robustness should not come at the cost of baseline accuracy?} 
% Instead, the risks associated with ML are defined more widely by all actors: 
users may have concerns with models analyzing their data, regulators may seek to limit potential harm to society  (\eg limit unfair predictions). We detail these risks in \S~\ref{ssec:risks}.

These varied risks, however, do not carry equal meaning and urgency for all principals involved in creating, using and regulating these models. Because risk definition is inherently tied to a given principal, \textit{e.g.} due to their own goals and incentives, and various principal definitions may come into conflict with one another, model governance is best formalized as a \textit{game}. Each principal participating in the game is optimizing for a set of constrained objectives at any point in time, which impacts the principal's trust in the ML pipeline and its other principals. The metrics underlying these objectives may differ from accuracy, and may be worst-case in nature\adelin{missing context. I think the point we want to make is that SOTA accuracy is not the only thing that should be considered in evaluating a model}. Thus, many established practices for evaluating ML fall short of providing the guarantees necessary for ML governance.\adelin{Same thing applies to how AML work is evaluated} 


\subsection{Principals, Incentives, and Capabilities}
\label{sec:principals}

Defining governance requires understanding the various principals in the ecosystem and their capabilities and incentives. We begin enumerating them below. In certain settings these principals may not always be separate entities---a data collector could also be the model builder---in which case such a principal can be thought of as playing multiple roles in the meaning common to the role-based access control literature.

\begin{enumerate}
\itemsep0em
\item {\bf End User:} This principal is using a system deploying ML. It may be a customer of a company, a patient at a hospital, a citizen asking for government benefits, etc.
\item {\bf Model owner:} This principal is one with a particular task that can be solved using ML. They communicate their requirements to the model builders, and clearly specifies how this trained model can be accessed (and by whom). 
\item {\bf Model Builder:} This principal is responsible for interpreting the model owner's requirements and designing a ML solution for them. To do so, the builder requires access to representative data from the domain (see data collector below), and an appropriate choice of training algorithm (and approach). 
\item {\bf Data Collector:} This principal is responsible for sourcing the data as per the model owner and builder's requirements so as to ensure that the learnt model performs well and complies with various characteristics (such as ensuring data privacy etc.). 
\item {\bf Adversaries:} The adversary is any entity that wishes to disrupt any phase of the ML life cycle. We consider adversaries with varying control and access over the ML system, including insider adversaries.
\item {\bf Trusted Arbitrator:} This principal is required in situations where (a) auditing of services provided is required (such as a legal agency or a mandated organization verifying if deployed models are compliant with GDPR), or (b) there is a requirement for arbitration between two principals (in situations related to ownership resolution). We also refer to this principal as the \textit{regulator}.\footnote{For simplicity, we conflate the entity providing the entity drafting the regulation or standard and the enforcement entity when they in practice differ.}
\end{enumerate}


In some situations, the data collector and model builder may both refer to the same  entity (\eg a company may collect data and train the model). Conversely, it is also possible that  responsibilities are split across subprincipals: a model builder may separate data science from deployment.


%\input{Contents/themes}


\subsection{Risks}
\label{ssec:risks}

We highlight three classes of risks relevant to ML governance that have been studied extensively in the literature. We also outline different failure modes inducing these risks (that can occur at different stages of the ML pipeline). Awareness of the risks present provide design goals and considerations that impact the creation, deployment and retention of the model, and these failure modes will later shape our discussion on accountability and assurance in \S~\ref{sec:accountability} and~\ref{sec:assurance}. Though we do not exhaustively cover all risks for clarity of exposition, the governance aspects which constitute this paper are generic and can be expected to generalize to other risks. 
\adelin{Could fix with a sentence to the effect of: To be precise, integrity is not a risk in and of itself as loss of model integrity may not necessarily translate at the system level to actual harm to model owner, such as reputation or financial loss, or end users, such as loss of life in autonomous driving. Nonetheless, to simplify our taxonomy, by integrity risk we entail any harm that may results from a loss of integrity of the model.} 
%\todo{adelin again this is not a real risk as in a model could be unfair and not lead to any resulting harm due to a bunch of factors (gabe an I have such discussion for finance and AEs). I think you need to map real examples to accepted definitions of risks. Happy to help refine these definitions and claims too nicolas I think as a response to Adelin's comment here we should lift the discussion of risk in this subsection here to the entire ML application/pipeline rather than just the model
%  yeah I think that would work. @mohammad: please ping me for that}
%\adelin{This has still not been lifted to the pipeline/system level. Integrity is not a risk, it is a failure mode. Lack of fairness and privacy is the same. Risk is: loss of life, reputation damage, financial loss etc. A model may fail locally without risk arising at the system level}


\vspace{1mm}
\noindent{\bf 1. Integrity:}
\label{subsubsec:integrity}
The most prevalent risk class is \textbf{integrity}. This is the immediate risk\adelin{Not a risk => failure mode. I as a business owner do not care if my finance model predicts x or y so long as I am not losing money}\adelin{Could fix with a sentence to the effect of: To be precise, integrity is not a risk in and of itself as loss of model integrity may not necessarily translate at the system level to actual harm to model owner, such as reputation or financial loss, or end users, such as loss of life in autonomous driving. Nonetheless, to simplify our taxonomy, by integrity risk we entail any harm that may results from a loss of integrity of the model.} that a model owner tries to minimize, for example, via training the most accurate and robust model. The integrity of a model needs to take into account the overall system this model is deployed within. Integrity risk quantifies the lack of alignment between the output of the ML system and what was expected from it.\adelin{Last 2 sentences are very good} 

There are in fact \textbf{accidental failures} that cause integrity risks\adelin{here it seems like risk==lack of assurance (ie risk is anything that cannot be proven correct). This is an inaccurate shortcut: risk is "The possibility of suffering harm or loss; danger." in the dictionary} stemming from how ML models are known to be brittle with regard to their data; data used to train models need to possess specific properties and must be processed in specific ways to enable effective training (\S~\ref{subsec:data_ownership}). This is done to ensure that models are resilient to {\em outliers} (data-points that are outside the range of those expected); since outliers are not representative of the underlying data distribution\adelin{This is factually incorrect in many sectors especially finance! Lookup any paper on "heavy tailed distributions" which have outliers naturally. It's a very common mistake to make.}, any model learnt using this data will not learn representations useful to model the test data of interest~\cite{gudivada2017data,cortes1995limits}. Another failure mode for integrity is that of {\em concept drifts} (where the distribution of data changes over time) \cite{lu2018learning}. Collectively, both these issues result in the model being unable to generalize. 

% \anvith{@Varun cited the big survey paper on concept drift above, perhaps below comments are less relevant now? I commented them out for the time being}

%\varun{loads of relevant papers:
%\url{https://cs.stanford.edu/~pliang/papers/}; also check out ludwig schmidt's work}. Collectively, both these issues result in the model being unable to generalize. \varun{@anvith: can you use google doc to add papers from percy + ludwig which are relevant to this topic?} \anvith{added a couple papers on concept drift, I only found two relevant papers from percy liang which I added to the google sheet (but I could be slighlty blind), and from that I think only one really fits with the discussion and even then not really}


%\anvith{following is new and feels very forced, in particular the last citation, I think it was before without it (we talk about this stuff anyways later)} Different approaches have been proposed for dealing with learning under such situations: Lu \etal \cite{lu2018learning} reviewed past approaches, and new approaches have worked on understanding how better to adapt \cite{kumar2020understanding}. 

Furthermore there are also known \textbf{adversary-induced failures} that cause integrity risks\adelin{again not integrity is not a risk in and of itself failure}.

At training time, adversaries incorporate \textit{data poisons} (which are specifically perturbed data-points) which result in poor generalization (\ie indiscriminate poisoning attacks~\cite{munoz2017towards}), or targeted misclassification (\ie targeted poisoning attacks~\cite{munoz2017towards}). \anvith{@Varun not sure what the following citations are referring to}Poisoning adversaries can assume that the data collector uses the labels provided with the poisons~\cite{}, or can also specify their own labels~\cite{}.\todo{citations missing} The former is known to be ineffective for heavily parameterized models~\cite{}, while the latter is effective across the spectrum. Poisoning is effective across a range of learning paradigms~\cite{carlini2021poisoning} (\varun{include latest carlini ssl work}), and across different threat models~\cite{}. Backdoor attacks proceed with a fundamentally different strategy; a specific {\em trigger} pattern induces a misclassification, and can be added to {\em any input} whilst generic poisoning ensures misclassification of inputs belonging to a particular class.

At inference time, adversaries can strategically modify inputs (whilst ensuring that they are indistinguishable from their benign counterparts) called \textit{adversarial examples}. This induces a misclassification~\cite{szegedy2013intriguing,biggio2013evasion}. These evasion attacks are known to be effective across a wide range of hypothesis classes~\cite{szegedy2013intriguing,goodfellow2014explaining,vernekar2019analysis,shafahi2018adversarial,papernot2016limitations},
% \todo{broken cite}
and learning paradigms~\cite{lin2017tactics,behzadan2017vulnerability,kos2018adversarial} \anvith{not too clear what you mean by learning paradigms, like unsupervised learning?}\varun{or re-inforcement learning, online learning etc.}\anvith{added}. While it was initially demonstrated for vision~\cite{szegedy2013intriguing,biggio2013evasion}, evasion has been demonstrated for a wide variety of domains including audio~\cite{carlini2018audio,yakura2018robust,qin2019imperceptible} and text~\cite{ebrahimi2017hotflip,alzantot2018generating,garg2020bae,zhao2017generating}. Research has demonstrated that such attacks can be physically realized~\cite{kurakin2016adversarial,yakura2018robust,Lovisotto2021slap}\varun{add slap attack from usenix 2021}\nick{added}. Additionally, research has also demonstrated that samples generated for evasion preserve input semantics~\cite{qin2019imperceptible,alzantot2018generating,dreossi2018semantic,jain2019analyzing,qiu2020semanticadv} \varun{add papers with sanjit seshia + chandrasekaran and seshia + dreossi + jha; also bo li has a bunch of papers to generate "semantic adversarial examples"}\nick{added}.

\vspace{1mm}
\noindent{\bf 2. Privacy:} Data is fundamental to training. Research has demonstrated how models trained without privacy considerations can leak information~\cite{shokri2017membership,carlini2019secret}. This has raised concerns about use of data containing sensitive information and its consequences for the individuals and groups alike. Thus, privacy is increasingly becoming a societal norm. This is perhaps best illustrated by recent legislative work seeking to adapt protective regulations such as the GDPR to the context of ML applications~\cite{}. Therefore, setting aside the value of upholding privacy as a human norm, growing regulatory limitations on non-private data usage means that it is in the interest of model owners to respect privacy-preserving practices. Indeed, not mitigating privacy risks\adelin{privacy loss is a risk. "Privacy risk" does not mean anything. Loss of privacy brings harm. Could be fixed with a sentence that says: By privacy risk we entail any harm that may results from a loss of privacy.} in their ML applications could result in a poor reputation for the model owner and compliance complications. 

Additionally, memorization of training data is essential for generalization of ML models~\cite{feldman2020does,Feldman2020what}, and recent work shows encouraging the model to memorize may help its performance and convergence rate~\cite{Katherine2021Deduplicating}. However, memorization could also lead to {\em accidental failures}: a model can memorizes sensitive data, such as credit card numbers, inadvertently~\cite{carlini2019secret}. Such secret information may then be leaked at inference time, \egwhen the model tries to auto-complete a sentence talking about credit card. As showed by the authors, the only effective method to prevent this happening is differentially private training, often at the expense of model performance.

There are also known \textbf{adversary-induced failures}.

In a membership inference attack (MIA), an adversary wishes to determine if a given data-point was used to train the model. Adversaries  initially assumed  access to confidence information from the black-box model~\cite{shokri2017membership} which was shown sufficient to determine membership. Following this,  research has further improved (and simplified) black-box attacks~\cite{salem2018ml,song2019privacy,jayaraman2020revisiting,truex2019demystifying}, for instance by performing label-only attacks~\cite{li2020label,choquette2021label}. Instead, white-box attacks further leverage information held in model parameters~\cite{sablayrolles2019white,leino2020stolen,song2017machine,nasr2019comprehensive}, or gradient updates~\cite{melis2019exploiting}. Yeom \etal~\cite{yeom2018privacy} draw the connection between the efficacy of MIA and overfitting. Based on this insight, various defences have been proposed~\cite{shokri2017membership,jia2019memguard,nasr2018machine}. However, they fail to provide meaningful guarantees of privacy as demonstrated  by Song \etal \cite{song2021systematic} with the introduction of the privacy risk score which still strongly correlates with membership despite these various defences being employed. However, Yeom \etal~\cite{yeom2018privacy} note that training the model to obtain differential privacy  does reduce a MIA's efficacy; drawing  theoretical connections between the efficacy of the attack and the privacy budget ($\varepsilon$) (in particular bounding the efficacy of such an attack) along with others~\cite{erlingsson2019we,jayaraman2020revisiting,sablayrolles2019white}.% Thus, as of now, the one promising defence against an MIA is to train with differential privacy. 

Beyond membership inference, other attacks attempt to reconstruct data---albeit with mitigated success. In  attribute inference attacks, the adversary attempts to impute missing values in a partially populated record using access to a ML model~\cite{jia2018attriguard}. Model inversion attacks aim to reconstruct data-points that are {\em likely} from the training dataset. In the classification setting, Fredrikson \etal~\cite{fredrikson2015model} exploit confidence information from the prediction vectors (based on the same overfitting assumption made in MIA). However, reconstructed  points are not exact training points but rather average representations of points from a class in the training set. With a similar intuition, Yang \etal~\cite{yang2019neural} use an auto-encoder to reconstruct the input from the confidence vectors, while Zhang \etal~\cite{zhang2020the} use GANs to aid reconstruction.  
%Note that the aforementioned attacks are possible when the model is fully trained.\todo{missing word in prev sentence}
More recent attacks (applicable in distributed training regimes, such as federated learning~\cite{konevcny2015federated}\footnote{Federated learning is a paradigm where multiple clients jointly learn a model by training a local model on their private datasets and sharing gradients which are aggregated at a central entity.}) enable successful reconstruction from gradients~\cite{geiping2020inverting,nasr2019comprehensive,melis2019exploiting, hitaj2017deep,wang2019beyond, song2020analyzing}. Again here,  training with differential privacy is proposed as a technique to defend against data reconstruction. In the federated learning setting, this has been studied and deemed effective~\cite{geiping2020inverting}.\todo{}\anvith{added one} 




%\paragraph{Fairness} The third overarching risk class is \textbf{fairness}.
\vspace{1mm}
\noindent{\bf 3. Fairness:} The challenges of algorithmic fairness are often not considered in terms of attacks and defenses. One can consider, for example, a prejudiced adversary that attempts to sabotage a model performance against a particular subgroup; but this also risks\adelin{change this verb because it overlaps with risk as used in the rest of the section} the integrity of the model. But does guaranteeing integrity mean that we have ensured fairness?\adelin{Once again have a sentence to the effect of: as before for simplicity we conflate lack of fairness and the actual (reputation, or end-user) risks or harm that result and designate them as "fairness risk"}

The answer is no; because ML models rely on extracting patterns in data, and 
%there is no question that 
unwanted biases are reflected within historically-collected data~\cite{lum_predict_2016, mattu_machine_nodate}. 
% \adelin{cite to substantiate claim}\mohammad{done}
Unmitigated, these biases transfer into algorithmic decisions that are fed back into the decision making process, thus aggravating the situation. Furthermore, algorithmic decisions themselves can also encode new biases that were not initially present in historical data; this may be due to poor quality, or non-representative data~\cite{suresh_framework_2021}, and even the careless use of fairness constraints.~\cite{cost_of_fairness}
% \todo{}\mohammad{done}

% \anvith{@Mohammad, @Varun, @Someone, missing attacks for this}
Unlike privacy and integrity, fairness risks, in large part, stem from data collection and processing steps. In an ideal world, (a) we would have had balanced datasets to train our models on, and (b) our models would apply equally to the population which would, in turn, ensure future balancedness of our datasets \varun{can you elaborate?}. But in most areas of critical concern in algorithmic fairness, neither is the case because there is a \textit{de-facto} sampling process~\cite{mitchell_algorithmic_2021} which precedes model building; an essential factor that should be considered under data collection. For example, in pre-trials where a judge has to assess the risk of accepting or rejecting bail, the defendants are only being subject to algorithmic predictions because they have been arrested in the first place. Mitchell~\etal~\cite{mitchell_algorithmic_2021} provide a broad overview on various fairness risks in three broad categories of (a) Data bias: both statistical--which evolves from lack of representation (\ie selective labels~\cite{selective_labels}), and societal--which indicates a normative mismatch~\cite{suresh_framework_2021}; (b) Model bias: influence of choice of \varun{hypothesis or} architecture~\cite{} and even interpretability, and (c) Evaluation: how the predictions would affect model predictions in the future. We will discuss such performative qualities of models in \S~\ref{subsub:performative}.

We quickly note that alleviating fairness risks in the ``ideal'' way above, would inherently be incompatible with controlling privacy and integrity risks, since our samples sizes are limited by the size of the smallest sub-population, which potentially limits the generalization of our models which not only threatens integrity but can also have adverse effects on privacy~\cite{shokri2017membership} .





\subsection{The Governance Games}
\label{sec:game}
\begin{figure*}
    \centering
    \input{Contents/Figures/game.tikz}
    \caption{Model Governance Extensive-Form Game Example---Strategy sets may be continuous (arcs) or discrete (branches). Dotted line indicates a non-singleton information set: the two decision points of Model Builder 1 are indistinguishable to Model Builder 2. The game is repeated (dots).}
    \label{fig:game}
\end{figure*}



 ML governance follows from the interaction of the principals (\S~\ref{sec:principals}) who are independent decision-makers with goals that may or may not align with each other. For instance, a model owner's desire of achieving robustness may exacerbate leakage of an end user's private information~\cite{song2019membership,song2019privacy}  because adversarial training encourages the model to output consistent outputs around its training data. 
 We can thus see ML governance as a multi-agent system and analyze dynamics between the principals using standard tools from game theory\cite{shoham_multiagent_2009}.
 Solutions to this game  affect the degree of trust among principals and towards the application of ML itself. 
 In many governance scenarios, principals act sequentially, after they perceive the effects of other principals' decisions. This naturally leads to a leader-follower, or \textit{Stackelberg} competition structure.~\cite{fudenberg_game_1991} 
 
 \subsubsection{Stackelberg formulation of learning problems}
 \label{subsub:performative}
Stackelberg competitions are found in strategic classification~\cite{hardt_strategic_2016} where subject of algorithmic classification---often in regards to welfare-related decisions such as employment, credit-lending, housing, etc---are strategic: after observing the decision made, they can adjust their features to achieve a better classification outcome. This is also an example of classification having performative~\cite{perdomo_performative_2021} qualities: participants adjusting their features causes a distribution shift, which in turn means that the future predictions of the model are not optimal w.r.t. to the new distribution. In practice, this requires model maintainers to re-train, or employ an online learning setup. Using a similar Stackelberg competition, \cite{perdomo_performative_2021} proposes an equilibrium notion called performative stability. Models that are performative stable produce predictions that would remain optimal under the distribution shifts that result from their own predictions. Br\"uckner~\etal~\cite{bruckner_stackelberg_2011} consider a similar problem in spam filtering and analyze an adversarial prediction game between a learner (leader) who tries to classify spam emails and an adversary (follower) that observes the learner decisions with the goal of producing less detectable spam emails.
  
% \paragraph{\bf Additional examples of Stackelberg games used in ML context}}
Stackelberg formulation of learning problems have been used in model-based reinforcement learning~\cite{rajeswaran20a} between a \textit{policy player} maximizing rewards under the learned model and a \textit{model player} that fit the real-world data collected by the policy player. An interesting application of this game in model governance may be to model the interactions between the Data Collector and Model Builder as policy and model players, respectively.%\todo{Mohammad I removed a sentence after here which I think is not needed} %Tsirtsis~\etal~\cite{tsirtsis2020decisions} study the joint problem of a finding a performant prediction model (or policy) and counter-factual explanations under the assumption that decision subjects are potentially strategic who would try to improve their chances of receiving a beneficial decision.
% \mohammad{Add explanation}\cite{steinhardt_certified_2017}

\subsubsection{Beyond two-player Stackelberg competitions: Extensive-Form games}
Most of the aforementioned art considers the strategic behavior of one other principal (the follower) whose objective is distinctly different from that of the leader. This improves over the \textit{adversarial assumption} of works that use a zero-sum game formulation (\ie Yao's principle~\cite{yao_principle}) which requires that the follower's objective be exactly the opposite of the leader's. As useful as that is, it only covers a subset of interactions that principals may have with each other. 

% How should we model scenarios that involve multiple principals (an end-user that takes a model owner to arbitration over privacy violations) or those that run over a (possibly undermined) course of time (a model maintainer that has to patch his model to accommodate new reagultaions)? What would happen if a subset of principals could not observe each other actions? (Model Builders engaged in a bidding competition)

In other scenarios (\eg contractor bidding competitions, or auctions) several principals may be deciding without observing their opponent actions. This requires a strategic-form game usually captured in the form of a pay-off table. Finally, such interactions can be repeating over time in several stages: principals' expected risks and payoffs should be adjusted with the perceived effects of their decisions in the future. An extensive-form represented as a decision tree can capture these multi-stage games with observed actions; it shows {\bf (i)} the set of principals, {\bf (ii)} the order of their decisions, {\bf (iii)} their choices at their respective decision points, {\bf (iv)} their payoff (or cost) as a function of their own choice as well as the history of the choices made prior to it, {\bf (v)} the information available to each principal at any decision point, and finally {\bf (vi)} the probability distribution over any exogenous event~\cite{fudenberg_game_1991}.

Figure~\ref{fig:game} which shows a hypothetical ML governance scenario. The regulator would like to ensure fairness and privacy guarantees so it requires that a (pure) deferentially private mechanism be used with a budget of $\epsilon < 10$. For fairness, the regulator requires demographic parity~\cite{fairml} with at most $\gamma < 10\%$ disparity between subpopulations. The model owner can choose its own specifications for $\epsilon$ and $\gamma$ and commission two model builders to produce the models. Model owners are now in a bidding competition to achieve the most performant\adelin{performant reads oddily} model within specification. They may choose different architectures, source their data from various data collectors (not shown in the figure for brevity), etc. In particular, they get to choose their privacy budget allotment between these intermediate steps~\cite{mironov_renyi_2017}. We note that model builder 2 \textit{does not} observe its rival's decision (hence the non-singleton information set of builder 1 annotated with dots). Therefore, the sub-game between the two builders is a strategic-form game played simultaneously between the two as no one goes first. Finally, the model owner accepts one model and rejects the other. Model builder payoffs are assigned at this stage. Next the regulator can check weather regulations have been respected, and issue proportional fines/incentives for the model owner. Also, since the game is repeated, the history of the game can be used to update the regulation (if necessary) for the next stage of the game. 
 
%  Game theoretic formulation of learning problems are common in the ML literature~\cite{gan_goodfellow}\mohammad{@varun, others, can you put some adversarial learning papers here}, but they are mostly formulated as zero-sum games, or equivalently the general min-max ruleknown as Yao's pricniple~\cite{yao_principle}.
\subsubsection{Solution Concepts} 
As with all games, finding the equilibria of governance games is often the focus of the analysis. This is because under an equilibrium, all principals involved in a game are choosing their optimal strategy w.r.t. each other. 
% \noindent{\textbf{Solution concepts for extensive-form games}}
%  \begin {itemize}
%      \item existence of equilibria (equivalance between extensive and strategic form games)
%      \item multi-leader-follower works
%      \item class of correlated equilibria (recent work from deep mind)
%      \item Integrating the game formulation in the model optimizations (Fei Fangs works)
%  \end{itemize}
% Classically solving a game entails finding and analyzing its Nash equilibria. 
 However, while such optimal solutions exists (for instance, for multiple-leader-follower Stackelberg games~\cite{hu_multi-leader-follower_2015, pang_quasi-variational_2005}); computing such optimal strategies is intractable in most cases of interest in ML governance: e.g. with multiple principals, a continuous (thus infinite) strategy set or across a time horizon~\cite{}\todo{}---all of which are present in our example in Figure~\ref{fig:game}.

\cite{fiez20a_implicitlearning}
\cite{li_endtoend_2020}

 \subsubsection{Future directions}
 \begin{itemize} 
 \item multi-metric multi-agent consideration
 \item What would happen in the absence of complete information \cite{roth_watch_and_learn_2016}
 \item natural answer to the question of how to choose values for parametric metrics
 \end{itemize}
 
\subsection{Our Approach}

\paragraph{Identity in ML systems} ownership
\paragraph{Accountability} attribution + auditing
\paragraph{Assurance} monitoring models + predictions (proactively ensuring integrity, privacy, fairnes etc)
\paragraph{Lifecycle} versioning, patching (unlearning and beyond), documentation (dataset cards)


==> Model%20Governance%20SoK%20draft/Contents/users/adelin_old.tex <==
\subsection{Auditing to Identify New Model Failures}

\nicolas{we need to read the auditing chapter in bishop p689 and see how logs need to be incorporated in this whole thing. typically auditing is logging + analysis. here we mean more that a regulator is querying a model to figure out what its limitations are (more or less what its attack surface is). so we might need to rethink this subsection}

We first examine the types of auditing that can be conducted in the context of machine learning models. We then overview how adequate ML logging procedures can support the auditing process and finally outline open problems in ML logging.

\varun{@adelin: the flow should answer the following questions: 1. how logging can help identify principals responsible for the aforementioned "bad events" --$>$ this is a more broad discussion; 2. why is logging for mL hard --$>$ this is also a broad discussion; 3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons); 5. how should it be logged (storage + computation costs); 6. compare + contrast with logging in practice}




\subsubsection{Flavors of ML auditing}

1. how logging can help identify principals responsible for the aforementioned "bad events" --$>$ this is a more broad discussion.

Similarly to Bishop~\cite{bishop} for systems, we define a audit as a formal examination by a third party to determine a chain of events and actors. In the case of ML models, this definition must further be extended to include the formal verification of claimed properties of a model.
As noted in our section on principals, the different parties may actually refer to the same logical entity. Hence, we introduce the notion of \textit{internal and external} audits respectively when the model owner and auditor are the same or independent entities. This distinction is important and provides deeper insight than its apparent simple nature.

To explicit the benefits of this model, we make a number of observation. First, an internal audit is a proactive action similar to a white-box assessment and may rely on model \textit{logs}. On the contrary, an external audit is a policing action by nature similar to a black-box assessment. Second, techniques which are hard externally may be easy internally\adelin{examples below}.  Third, it may be easier for a regulator to verify that internal techniques are properly implemented, proving internal audit results correct, than to perform an external audit by querying a model in black-box fashion. For instance, the implementation code of SISA unlearning of Bourtoule \textit{et al.}~\cite{bourtoule2019machine} can be easily reviewed for correctness while model unlearning verification is still largely open problem\adelin{make claim softer}. 

This distinction thus allows us to realize that (i) internal audit can help enhance external audits and (ii) regulators should be flexible in mandating audit approaches. Regulators should require the most appropriate of internal or external perspective depending on technical feasibility of verifications under each perspective. Observe that accountability and attribution are then the same problem viewed respectively internally and externally. 

\subsubsection{Log collection for ML: What to log?}
3. what should be logged? (only finitely many things can be logged -- what are the pros and cons of each)?; 4. when should it be logged? (pros + cons);


Model owners may have an obligation to collect logs due to business (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pci_2020}) or legal requirement (the EU AI regulation draft~\cite{eurlex_nodate} would fraud detection and credit scoring due to their impact on humans may require ML logging according). 
%Model owners may have an obligation to collect logs due to business (for instance for credit card transaction as per PCI-DSS standard~\cite{noauthor_pcidss_2015}) or legal requirement (financial institutions are required to report security incident and be capable of explaining the chain of event that lead to the breach or may see their practicing license revoked). 
%For instance, ML logging may be need to comply with the credit card transaction PCI-DSS standard~\cite{noauthor_pci_2020} while the EU AI regulation draft~\cite{eurlex_nodate} would fraud detection and credit scoring due to their impact on humans may require ML logging according. 

Well established logging guidance exist in non-ML settings~\cite{owasp_logging,noauthor_pci_2020} but are not readily applicable due to the (i) probabilistic nature of ML and (ii) ML-specific steps, like training, of the ML life cycle may not be covered in these frameworks.
%A wide range of existing frameworks in traditional security (eg \url{https://cheatsheetseries.owasp.org/cheatsheets/Logging_Cheat_Sheet.html}). They are not readily applicable in ML due to the probabilistic nature of the domain (like how SISA is the only method to perform perfect unlearning so far). In the same way we can't readily use normal logging procedures for audit log generation. However, we could use proof of learning algos for audit logs. 

%Since SOTA models can be extremely large, a huge body of works focuses on model compression but models can still be in tens or hundreds of MBs making checkpoints prohibitive as a log solution.
\varun{motivate why checkpoints can be used for logging a bit better; the next para does that well}

%"Logging is the collection of information; auditing is its analysis."
%A bit reducing the audit process but acceptable
%"Last comes auditing. Commercial systems emphasize recovery and accountability. Auditing is the process of analyzing systems to determine what actions took place and who performed them. Hence, commercial systems must allow extensive auditing and thus have extensive logging (the basis for most auditing). Logging and auditing are especially important when programs move from the development system to the production system, since the integrity mechanisms typically do not constrain the certifier. Auditing is, in many senses, external to the model." bishop
%Basically external is when the enforcement arm of the auditor is mandated by someone other than the model owner and internal is when the model owner and regulator enforcement are conflated
%attribution is external under that view while accountability is internal.
%in acountability the model owner proactively makes the model identifiable in case of a problem.
%In attribution the model owner is trying to evade being linked to a specific model
%often, a lot of the research is written under the assumption that the model is productized or whatever and external entities find issues that require resolution. auditing + logging seems to be the only internal concept that’s interesting, that i can think of. anything i am missing?
%I think there is: internal can help exernal. See it as internal ~= whitebox, external ~= blackbox. (edited) 
%Then proof of learning is internal whereas radioactive data is somewhat external
%internal can help external -> that also makes sense. and this concept holds across, right?
%Yep. In financial audit a regulator requires both external and internal audit
%Audit logs may be useful to detect an attack while it is happening, perform post hoc correlation analysis over multiple records (a stronger paradigm then current ML model defenses/cite lucy's work), or enable the reconstruction of event following an attack to identify the \textit{modus operandi} of the attacker and prevent the same attack from reoccurring. 



For ML, the information to be collected greatly differs from traditional event-driven logs used in network security. One may need to collect gradients, weights (which can be in the trillions) etc. Ideally, one would collect all possible information for each single input to the model, however in a real production system, log space is inherently finite. 

%"The first goal is to detect any violations of a stated policy; the second is to detect
%actions that are known to be part of an attempt to breach security." bishop

\subsubsection{Existing work}
6. compare + contrast with logging in practice
The external auditing perspective is common in the literature on security and privacy of ML and is covered in a number of related SoKs\cite{}\adelin{Adi, nicolas, @mohammad: privacy and fairness examples?, could also add milad's paper}. 

Despite the existence of a number of industry ML logging tools and practices exists~\cite{google_monitoring, mlflow_log, fiddler_monitoring_nodate,amazon_log,noauthor_whylogs_2021}, only little academic work has delved into the internal perspective and more specifically ML logging.\adelin{I have not checked bias and fairness lit} The Proof of Learning framework from Jia\textit{et al.}~\cite{jia2021proof} can be thought to provide a form of training time log enabling internal audit against model extraction attacks\adelin{@mohammad please verify this}. In that perspective a model weights, X, Y are saved. Concurrently in the audio domain, after suggesting an audio biometrics incident investigation use case for ML pipeline logs (similar to Transition-Based Auditing which targets known attempts to breach security~\cite{bishop}), \textit{Travers et al.} introduce \textit{surreptitious adversarial examples}, a new class of attack targeting simultaneously both the ML model and the underlying log analysis system. They instantiate this class with a joint optimization attack. 

\subsubsection{Open issues}
 2. why is logging for mL hard --$>$ this is also a broad discussion;
   5. how should it be logged (storage + computation costs); 
 
We identify 2 major open issues with ML logging, respectively log sanitization and storage overhead.

Since logs may be accessed by auditors, they represent a privacy and security risk and must be sanitized~\cite{bishop}. In the case of ML, such risks include model inversion and membership inference techniques. This is problematic since techniques such as DP target the training phase rather than already existing sets of weights\cite{}\adelin{Would appreciate help in finding the correct citation}. 
%complex as Proof of Learning Logs are essentially a snapshot of a model while spectrogram logs could be inverted 

Overhead is already a major issue in non-ml audit log systems~\cite{bates_trustworthy_nodate,owasp_logging} for which each individual record is small; the problem is only accentuated for audit logs of ML models and systems. 

The common log formats like Common Event Format (CEF, used in syslog) and Common Log File System (CLFS, used in Windows event logs) are inappropriate for ML. These formats are extremely compact (\textit{e.g.} an entry, a single log record, consists of just time, event type, name, extension) and the extra data stored in the extension tends to be short (for instance limited to src attacker ip and dst target ip). Hence, a dedicated yet efficient log format must be designed from ground up for ML logging. %One way to reformulate this is to state the logging problem as an optimization problem over a set of metrics that act as proxies, or correlate, to some task (debugging, security etc). 

% \adelin{It seems that you are confusing 2 concepts. Log based auditing/monitoring (internal) and external auditing. They are related but not the same.  Internal information helps speed up external audit but is not required in the same way whitebox is great for security analysis but adversaries may operate in a blackbox paradigm. Happy to help formalize/write this now that I have time.}

% \adelin{The paper would benefit throughout from an internal vs external audit perspective as explained in slack: 
% Basically external is when the enforcement arm of the auditor is mandated by someone other than the model owner and internal is when the model owner and regulator enforcement are conflated
% Adelin:shell:  5 hours ago
% attribution is external under that view while accountability is internal.
% in acountability the model owner proactively makes the model identifiable in case of a problem.
% In attribution the model owner is trying to evade being linked to a specific model
% Varun  5 hours ago
% that makes sense, but i don’t think there’s anything interesting/unique to talk about when we are discussing “internal” related concepts right? often, a lot of the research is written under the assumption that the model is productized or whatever and external entities find issues that require resolution. auditing + logging seems to be the only internal concept that’s interesting, that i can think of. anything i am missing?
% Adelin:shell:  5 hours ago
% I think there is: internal can help exernal. See it as internal ~= whitebox, external ~= blackbox. (edited) 
% Then proof of learning is internal whereas radioactive data is somewhat external
% Varun  4 hours ago
% internal can help external -> that also makes sense. and this concept holds across, right?
% Adelin:shell:  4 hours ago
% Yep. In financial audit a regulator requires both external and internal audit
% It could help with the compliance thing: a lot of techniques which are hard externally may be easy internally. Hence we could argue that a regulator doesn't legally enforce external audit but legally requires internal techniques. It;s easier to check that internal techniques are properly implemented (hence the results are correct) than to actually do the external check in a few cases}



==> Model%20Governance%20SoK%20draft/Contents/users/anvith.tex <==
%OLD UNLEARNING BLURB

\nicolas{anvith this is for you}

\anvith{I've written up this section in paragraphs for now; I think later we'll drop the separate paragraph structure and keep it as one continuous block of text, but for now I think it helps breakdown the structure for the section while we continue to edit it}

\paragraph{Motivation} After having trained a model $\model$ we might have reason to try and forget the effect of a particular datapoint on the model. This could be for privacy reasons; a user may revoke an entity's access to their data and now the entity is accountable for forgetting their data. Alternatively this could be for security reasons; it may be found after the fact that a model was poisoned through certain datapoints and now needs to forget these datapoints to patch the security breach. Thus a part of the lifecycle of a machine learning model is the handling of such requests, and the process of trying to forget a data point is what is called machine unlearning. \nicolas{NP let's expand this paragraph a bit to discuss what patching would look like. we should probably also discuss things like fine tuning etc. in this section somewhere}


\paragraph{Formally Defining Unlearning} At a high-level an exact unlearning process is one which takes the distribution of models returned by a training algorithm trained on $D$, which we'll call $H_D$, to the distribution of models returned by the same training algorithm when trained on $D' = D/\mathbf{x}^*$, which we'll call $H_{D'}$. More formally, if $U$ is a function (that could be random) which takes a model $\model \in H_D$ and returns another model $\model'$, and $S = U(\mathcal{H}_D)$ we say $U$ is an exact unlearning process for $\mathbf{x}^*$ iff $S = \mathcal{H}_{D'}$. 

Note in practice a model can be thought of as either a specific set of weights for an architecture or as a function (these two views are clearly not equivalent as we can have the same function even though we've permuted the weights). Thus one would need to specify what the equivalence is taken over. \anvith{could cite my submitted paper here for the definitions}:\nicolas{NP I don't think we will actually need these definitions standing out like this, we can probably switch to some text in the para that says you can operate over distribution of weights or distributions of outputs. otherwise it will be too obvious that we are the ones writing the sok}\anvith{yeah I agree; I've commented it out for now, and I think the above text is sufficient}

%\begin{enumerate}
%\itemsep0em
%\item [{\bf Def 1}] $d_{\weights}(S,\mathcal{H}_{D'}) = 0$ where $d_{\weights}$ is a metric measuring the difference in the \textit{distribution of weights}
%\item [{\bf Def 2}] $d_{out}(S,\mathcal{H}_{D'}) = 0$ where $d_{out}$ is a metric measurin difference in the distribution of input-output maps, or simply difference in the \textit{distribution of outputs}
%\end{enumerate}


\paragraph{Quintessential example of unlearning} Currently the only process for exact unlearning a deep neural network is naively retraining, where one simply obtains a model $\model''$ by retraining on $D'$ (note this is exact as we return the distribution $H_D'$). The issue is that training itself is expensive and having to retrain doubles (or more depending on how often one needs to unlearn) the cost of deployment of the model. There are methods that make the cost for retrainining cheaper, in particular SISA \cite{bourtoule2019machine}, but it requires changes to the training pipeline and can still be quite expensive.\nicolas{we need more papers cited here than just SISA.}

\anvith{for me: describe the examples here a little more}
\paragraph{Approximate Unlearning} In response to the issues of cost people have turned to more approximate notions of unlearning where we no longer require to exactly reproduce the distribution of $H_{D'}$, and also take leeway with what metric they use to defining unlearning (shifting from looking at similarity in distributions to measures of desirable traits of unlearning). For example, one approach is to measure/minimize the difference in weights from the output of $U$ on some $\model \in H_D$ and a single point in $H_D'$ (typically obtained by naively retraining) \cite{deltagrad,abadi2016deep}, or using membership inference to see how much the model leaks the information of having trained on $X*$ \cite{baumhauer2020machine,graves2020amnesiac,scrubbingv2,golatkar2020eternal}. That said several pieces of work do indeed focus on metrics that capture (to varying extents) the similarity in the distribution of weights \cite{scrubbingv2,golatkar2020eternal,guo2019certified,sekhari2021remember}

\anvith{for me: go into more specific examples of the issues of equivalence here}
\paragraph{Issues with approximate unlearning} The main issue with the work on approximate unlearning is that none of these metrics are necessarily equivalent. This poses the problem that for governance, when we wish to regulate what being sufficiently unlearnt means, we cannot simply use any of these approximate unlearning metrics and expect it to cover all the metrics used to characterize unlearning. Facing this challenge there is a need for a comprehensive single metric (whether new or singled out from past-work) to focus on when wanting to make claims of being sufficiently/approximately unlearnt.


\paragraph{Issues with Exact unlearning} Furthermore, even in the case of exact unlearning, one can still leak private information about the users who requested deletion by the mere fact that a user's decision to delete their data isn't necessarily random and could be based on model behaviour; Gupta et al. \ref{gupta2021adaptive} showed that SISA (an exact unlearning method) can leak information about users who deleted their data by the well-observed correlation between performance and being in the training data. The fix to this would be to give provable privacy guarantees on the information one could attain from the model, such as DP-guarantees, which is what Gupta et al. \ref{gupta2021adaptive} formally show.


\anvith{should I go into more detail about the issues of equivalence? like give specific examples? }
\nicolas{NP yes I think that would be interesting for now. I would also add other issues such as the ones pointed in this recent paper https://arxiv.org/pdf/2106.04378.pdf. also look at the related work in this paper and check if we can also discuss some of that related work here }
\anvith{I remember reading this before; I'll add this issue too; ad for other citations I was looking and we pretty much cited most of them (but I might've missed some so I'll keep looking)}

==> Model%20Governance%20SoK%20draft/Contents/users/anvith_assurance.tex <==
% \noindent{\bf Compliance:} This is the process of ensuring that ML models can be legally regulated.\adelin{This definition of compliance is factually incorrect. Compliance goes beyond legal into adequation with industry standards/frameworks at the risk of seeing licenses for a particular business line revoked. e.g PCI-DSS forcredit card.}\adelin{Note to self to provide a good definition of compliance/maybe group key concept definitions in III/II. discussion should delve into the hurdles of GRC for ML} In particular, one \varun{who?} needs to ensure that the ML model can forego the influence of a particular data-point (or subset of data) on demand. This is necessitated by recent regulation such as the GDPR~\cite{}, CCPA~\cite{}, or PIPEDA~\cite{}\adelin{Note to self to propose modification to include framework like PCI-DSS/ abstract the writing away from privacy alone. Might not be what nicolas wants}. \adelin{Machine unlearning feels a bit out of place here. Basically the problem of this paragraph is that it conflates privacy regulation compliance and compliance which is far far broader (both outside of privacy and of regulations)}


%however there has yet been no work on such a verification procedure. In fact, it would seem that such a process may be impossible\adelin{untrue for SISA: See discussion at the end of \cite{bourtoule2019machine} on how it is possible to prove SISA.}, at least if it depends on logging \cite{future anvith paper}. \anvith{@Varun added the last two sentences, and the last sentence just for reference on why POUL doesn't work. I guess it's not ideal that I haven't written the paper yet...}  %Recent work \varun{@anvith: proof of unlearning bit.}

% \anvith{@Mohammed certified processes or things that give guarantees: }
% \noindent{\bf Fairness:} \textcolor{olive}{Assurance of fairness during the training of a model can be given by implementing algorithms that provably result in fair models. 
% prepocessing \cite{feldman2015certifying}, in-processing \cite{celis2019classification,zemel2013learning,ruoss2020learning}, post-processing \cite{didn't find any}
% }

%Fairness constraints are a way to ensure equitable decisions while training the models (in-processing). Finally, existing legislation may require a ratio quota (post-processing). 

% \url{https://towardsdatascience.com/algorithms-for-fair-machine-learning-an-introduction-2e428b7791f3}

% \nicolas{moved this paragraph from the risks section because discusses techniques to improve fairness. Mohammad merge? NP follow up: i just removed because already covered in assurance for training data}
% The study and mitigation of the said biases in decision making systems, studied in the growing field of algorithmic fairness has shown that, only with respect to model training, biases may be tackled in three major ways. First, biases can be mitigated by resampling data used in the training of models (pre-processing)\adelin{what about post processing? What happens if on the contrary preprocessing inserts bias?}. 

% NP removed for scope 
% \noindent{\bf Explainability:} Most importantly, ML models should not be treated as black-box technologies; understanding the process (or reasoning) behind their prediction outcomes is essential for many real-world applications~\cite{}.\adelin{Explanability is very close to forensics in fact: in one case the focus is model security in the other it is fairness etc. Logging is one way to do this. I don't see why the 2 concepts are separated. Would love to cite the work with gabe here...} By definition, one requires explanation {\em post-hoc} (\ie to explain a model prediction, or some specific behaviour).\adelin{\cite{travers2021exploitability} for logging used by defenders at financial institution for forensics } To this end, explainability methods are focused as such.\adelin{sentence just before is strange} Explainability by itself comes in two flavors: (a) one can explain an outcome with respect to specific features of the input, and (b) one can explain the outcome by understanding its interaction with different model parameters.\adelin{see my discussion above as to how this seems reductive of the impact of explainability}\adelin{should bring out some of my Statement of Purpose here} In the context of vision applications, saliency maps are commonly used techniques to ascertain 




% \newpage
% \nicolas{varun: take a stab at coming up with some structure for this, it will be the crux}\adelin{@varun:let me know if you want a rubber duck}



% \subsubsection{items to cover}



% \begin{enumerate}
% \item legal discussion of accountability based on some content in \url{https://officialblogofunio.com/2019/04/29/a-short-introduction-to-accountability-in-machine-learning-algorithms-under-the-gdpr/}
% \item cross reference a lot of stuff from the access control bit
% \item discussion around who can access model and when (standard white-list vs. black-list)
% \item GDPR compliance: unlearning approaches \adelin{again feels weird to reduce GDPR compliance to unlearning, without considering data, how it is organized, classified etc, privacy etc}
% \item deepfake generation/detection + attribution
% \item if model is used for transfer learning, what to do then?
% \item who designed the algorithm that was used for training the model? who collected the data? all of this should be logged
% \item transparency in decision making
% \item explainable AI + efforts in this space
% \end{enumerate}


% a second plan found elsewhere initially

% \begin{enumerate}
% \item Phase 2: training
% \item ensure that training has occurred correctly (if performed in a decentralized manner)
% \item ensure that the model learnt is performant + encodes some information about the true owner (watermarking)
% \item ensuring that the privacy of the training data is preserved (\ie DP training)
% \item ensure that subgroups are not disadvantaged -- algorithmic fairness
% \item ensure that training data isn't memorized -- data de-duplication (new carlini paper)
% \end{enumerate}

% Having covered various rudiments related to dataset creation, attribution also covers important facets in the training process. We discuss those next.

% \paragraph{Algorithmic Choice \& Fairness} Recent research has     demonstrated 

% \paragraph{Integrity of Computation}

% \paragraph{Data Privacy}

% \paragraph{Ownership Encoding}

% \paragraph{Memorization}

% \subsubsection{Formalizing the Game between ML Principals}

% \nicolas{Anvith this is for you}

% \anvith{Below is the newer stuff, which I expect will get changed once @Mohammed has time}

% \anvith{first the mathy version of the formalism I had in mind}

% \mohammad{This can be made into a Stackelberg competition extensive-form game.}\adelin{agreed on stackelberg games. Main problem is that they require a ton of background of their own}\adelin{happy to help on stackelberg as well}

% \anvith{I've commented the below out as I don't think it's particularly relevant now, @Mohammed see my comment for flow in the slack thread}

\iffalse
The three ML principals are the model owners, the users, and the regulators, and each return a vector of values that the other's interact with (these are the strategies). 

Say there are $n$ metrics associated with a model. The model gives it's n-vector of values on each metric, which we call $\mathbf{m}$. The user gives its weighted preference for each metric $\mathbf{p}$.\adelin{Problem: implicit assumption that the model owner and user agree on the metric.if they completely disagree then those vectors would be "disjoint" (non zero only where the other is 0) and the dot product collapses to 0} The regulator gives its thresholding for each metric $\mathbf{t}$ (for example minimum fairness, minimum privacy, etc.).\adelin{How is this threshold defined?}

The benefit for the model owner is $\mathbf{m} \cdot \mathbf{p}$,\adelin{see the above if the end user and model owner's objective don't align this collapses to 0} the cost for the model owner is $\mathbf{m} \cdot \mathbf{c} + || \mathbf{m} - \mathbf{t}||_{1}$ where $\mathbf{c}$ represents the cost vector for the metrics (\ie a more accurate model costs more).\adelin{Where do you place the fact that a model may be impossible to realize given the regulator constraints? KKT?}

The benefit for the user is simply $||\mathbf{p}||_{1} + \omega \mathbf{p} \cdot \mathbf{p}_0 $ (\ie would like the best at everything but has a preference $\mathbf{p}_0$) and the cost is $\alpha(\mathbf{m} \cdot \mathbf{c} + || \mathbf{m} - \mathbf{t}||_{1})$, \ie proportional to the cost of the model owner (as that cost is passed down to the model user).

The benefit for the regulator is $\mathbf{t} \cdot \mathbf{p}$ (\ie aligns with the user) and the costs are $||\mathbf{t} - \mathbf{m}_{0}||_{2} + \alpha(\mathbf{m} \cdot \mathbf{c} + || \mathbf{m} - \mathbf{t}||_{1})$ where $\mathbf{m}_0$ is some baseline vector representing what all the model owners can reasonably achieve. 


\anvith{now the wordy version}
\adelin{@anvith: }

There are three main principals we're focused on, the model owner, the user, and the regulator. They each have their own goals, and their own costs which they try and balance. For simplicity we can imagine that with any ML model there are a finite number of metrics associated with it which is all that any of these principals are interested in.

The user wants the best model on all metrics\adelin{assumes that all principals have the same expectation domain and that all principals are honest}, however we can imagine that they have certain metrics they prefer more. These preferences are passed along to both the regulator and owner. The owner tries to produce a model good at everything, but now with a preference for those metrics users care about, and regulators try and make the minimum allowable thresholds high on everything, but with a preference for what users prefer.

\anvith{@Varun new discussion on this}
This is a bit ideal and assumes the user understands how the various metrics compare in order to have preferences, and this assumption isn't necessarily always the case. For example consider $(\epsilon,\delta)$-DP as a privacy metric. A user may value privacy highly, but does this mean they would want to make the DP bounds as low as possible if the benefits to privacy aren't as substantial as the costs to performance? That is, though various aspects of a model are quantified in terms of some metric, not all these metrics may easily scale to the values the user cares about. How informed/knowledgeable the user is about the metrics would then dictate their decision, and this more generally shows the issue with metrics that don't easily translate to user-friendly information (as users may not understand what metrics to prefer). We highlight this as an interaction model owners have with the user (the picking of the metrics to use) and how this influences what the user would prefer and thus what the model owner would design for.

In fact at some level we can assume that the model owner and regulator have the same interaction; a model owner may be technically justified in claiming a metric satisfies some more abstract value (privacy, fairness, etc.) however if the justification is not easily understood then it may be they would still be charged for not satisfying certain criteria. The reverse situation could also happen, where a regulator is convinced that a metric represents some value, even though at a more technical level it doesn't.

So in general the choice of the metrics by all the principals is itself a great challenge. Nevertheless, in the case all principals have come to agree on certain metrics and that the user has a well-defined preference for some of them, we can expect a model owner to incur certain additional costs to improve on those specific metrics, and certain metrics may be more expensive than others. It may in fact be that certain combinations of metrics are more costly than others, or even impossible \adelin{or even impossible}. Sticking to the example of DP, consider trying to train with tight DP guarantees while still having reasonable performance, which often requires aditional costs in the form of additional pipeline changes \cite{papernot2017practical,papernot2018scalable} or collecting more data \cite{google thingy} \anvith{@anyone, more citations?}. . These costs are then passed onto the user as they are eventually the ones paying for the model, and these costs may further be passed onto the regulator themselves as users usually don't like expensive models and the regulators are at some level liable to the users wants\adelin{a bit of wishful thinking in this last sentence ;-p Very good points are made though}).It's perhaps not also unreasonable to imagine a regulator faces costs for having thresholds far above what is feasible for model owners (say expecting $\epsilon =0.1$ DP and $99\%$ accuracy) and that a model owner incurs other costs for every metric they have under the thresholds set by the regulator (with the possibility that being far under is far worse than simply being a little under)


Nevertheless, observe how all these entities interact to influence each other's benefits and costs, and how at times they are seemingly contradictory. The example with DP and performance show how having a preference for both would also introduce undesirable costs to the users. What this is to say is there will necessarily be a balancing act between the costs and the benefits for all entities involved. Computer science research for governance, which is what we focus on here, is about reducing the costs associated for all principals (in particular the model owner), and finding justifiable metrics to parametrize certain qualities of a model. \anvith{@anyone, is the last statement justified}

%where as we expect legal/governing\adelin{same disclaimer as above to remove the legal element which both reduces the scope and is not our call} bodies will decide how to balance the benefits and risks with current technologies.

\anvith{@Mohammed, this said, if we can solve the game that would be pretty pretty cool}

\anvith{also @Mohammed, I'm definitely not saying this is the game we actually care about, I might have completely forgotten certain aspects}

\fi

% \anvith{Below is my old stuff which I've commented out for now}

\iffalse

Rough Structure:
\begin{enumerate}
    \item List main principals (Owners,Users) and duality (possibly adversarial possibly not)
    \item define the interactions of interest (owner facing possibly adv user, owner facing possibly adv owner, user facing possibly adv owner): note here adversarial just means having some property that is against something the other principal wants
    \item remark how the resolving above claims is accountability
\end{enumerate}

\anvith{@Varun I guess I'll define the principals, but we'll probably adapt this once 3.B is done}

With ML there are two main principals: the model owners and the users, where the user could be someone who supplied data or interacts with the final model. Furthermore both the owners and users could possibly be adversarial to other principals (where here we mean adversarial not only in intent, but that they exhibit properties that are not desirable for other principals). Note that we typically have only two types of interactions between principals: owners interacting with users (via training and deploying a model), and owner interacting with other owners (when designing and training a model). Users interacting with other users would be outside the context of ML. \anvith{right?}


The main interactions we are interested with governance are those when the possibility of being adversarial is raised, and there are (among the two only allowed interactions defined above) only three forms of such claims: an owner who claims a user was adversarial (\ie claim the user poisoned their dataset), a user who claims an owner is adversarial (\ie their model isn't fair), and an owner who claims another owner is adversarial (\ie the person stole their model). 

Accountability in ML seeks to resolve these claims.

\anvith{Opinions?}

\fi

%\paragraph{Data Integrity Assurance} certificates of data sanitization

%\paragraph{Data Confidentiality Assurance} \anvith{@varun relevant?}

%\paragraph{Data Fairness Assurance} datasheet for datasets



%Once the data has been collected and pre-processed, it must be served to the learning algorithm at training time and to the model for inference. While this step of the ML pipeline has received relatively little attention, recent work demonstrated how an adversary able to reorder the data without modifying it can achieve the same effect than a poisoning attack which would require modifying some of the training points~\cite{shumailov2021manipulating}. This highlights the need to ensure that proper randomness is employed by the training algorithm when sampling training data for stochastic gradient descent. This would prevent the adversary from reordering data. Indeed, analog to the role it plays in cryptography, randomness is fundamental to the generalization guarantees of stochastic gradient descent~\cite{}. Similarly, when training a model with differentially private stochastic gradient descent, the theoretical guarantee of privacy stems in part from a property known as privacy amplification by subsampling which again requires that one ensures that minibatches of data are sampled uniformly at random from the training set during gradient descent. These issues are made more difficult to address in the distributed setting, where data may be stored and processed by multiple workers before it is analyzed by the training algorithm. 

%\textcolor{olive}{Thus for the assurance of proper data servinging we need assurances of random sampling of batches; this is an open problem for the ML community to address}


%\nicolas{inference over encrypted data?}

%It is worth to note that these works above differ from other data poisoning defenses because of the certification mechanisms they proposed, which is essential for the methods to be used for assurance. 

% \varun{missing discussion around robustness techniques for evasion -- just need to add madry + kolter's certificate + greg yang's generalization of kolter's work.}


% \nicolas{ADdd PoL to discuss this: ensure that training has occurred correctly (if performed in a decentralized manner)}

% \varun{this bit could include some content from decentralized/federated learning + can include works like capc and the dp algorithms for fl + fl attacks} 

% \varun{to do: compress}
% Model owners wish to ensure that ML models only learn {\em what is necessary} from the data to be performant. Often, this requirement is interpreted as ensuring that the ML model does not learn sensitive attributes from the data that was used to train it. Recall the privacy risks we have described in \S~\ref{ssec:risks}: adversaries exploit this {\em memorization effect}\footnote{Feldman argues that such forms of memorization are essential for learning~\cite{feldman2020does}.} to learn more about the training data. 

%These attacks are prevalent in DL models, and are classified into two categories: (a) membership inference attacks: where the adversary tries to infer if a data point was used during training~\cite{pmlr-v139-choquette-choo21a, shokri2017membership}, or (b) model inversion: where the adversary attempts to reconstruct the data used to train the model~\cite{fredrikson2015model,carlini2019secret,carlini2020extracting}. \varun{can potentially condense these definitions of memb inf and model inv. as they are defined earlier}


% One could ensure that the training data is obscured (in an attempt to preserve its confidentiality), and attempt to learn from such data~\cite{huang2020instahide,yala2021neuracrypt}\footnote{This form of encryption is not cryptographically secure, as noted by the authors of~\cite{huang2011adversarial}.}. However, follow-up research demonstrates that such forms of instance-hiding is insecure and can be inverted~\cite{carlini2020attack}. This suggests that a more {\em formal} definition of what it means to obscure (or encrypt) training data (such that utilitarian learning can be performed) is needed.

\iffalse 

\subsubsection{Data collection}

As alluded to earlier, preparing a ML model for deployment is a complicated procedure and involves several phases. At the earliest stage, extreme care must be placed in collecting the required data for training the model. Often, practitioners assume that the data provided is {\em ideal} for training models. In this section, we will begin by providing various other factors (in no particular order) that one should consider during data collection.

% Nicolas removed because this is for the previous section - not assurance \paragraph{Data Attribution} Data attribution is the process where one can identify the entity responsible for data sourcing. \varun{add a couple of lines on why this is important + relevant references}

\anvith{currently using numbers as I documented the papers in a seperate google sheet}

\paragraph{Bias Alleviation} To ensure that the model learnt is unbiased, one needs to begin at the grass roots level and ensure that the data being collected is free of any bias. Bias alleviation comes in many forms; ensuring that features relevant to specific sub-groups are correctly managed (or engineered) is an important component of bias alleviation~\cite{2,3,8}. \varun{populate more.}

\paragraph{Concept Shifts} Another common assumption is that the training and testing data are from the same distribution. However, this may not be the case~\cite{lu2018learning}. Concept (or dataset) shifts can occur for a variety of reasons \varun{populate}

\paragraph{Subgroup Representation} Many datasets, such as those commonly used for vision tasks~\cite{deng2009imagenet}, are known to improperly represent specific subgroups~\cite{6}. This results in severe detrimental implications in downstream applications. \varun{expand}

\paragraph{Data Sanitization} If created in an unchecked manner, datasets can contain various artifacts that are detrimental to the model's ultimate performance. For example, data poisoning attacks, where adversarial entities encode human imperceptible information into the data items result in models that are poorly performant (\ie poor generalization)~\cite{}, or models that misclassify specific target inputs~\cite{}. 


\subsubsection{Data serving}

Once the data has been collected and pre-processed, it must be served to the learning algorithm at training time and to the model for inference. While this step of the ML pipeline has received relatively little attention, recent work demonstrated how an adversary able to reorder the data without modifying it can achieve the same effect than a poisoning attack which would require modifying some of the training points~\cite{shumailov2021manipulating}. This highlights the need to ensure that proper randomness is employed by the training algorithm when sampling training data for stochastic gradient descent. This would prevent the adversary from reordering data. Indeed, analog to the role it plays in cryptography, randomness is fundamental to the generalization guarantees of stochastic gradient descent~\cite{}. Similarly, when training a model with differentially private stochastic gradient descent, the theoretical guarantee of privacy stems in part from a property known as privacy amplification by subsampling which again requires that one ensures that minibatches of data are sampled uniformly at random from the training set during gradient descent. These issues are made more difficult to address in the distributed setting, where data may be stored and processed by multiple workers before it is analyzed by the training algorithm. 


\nicolas{inference over encrypted data?}

\fi


==> Model%20Governance%20SoK%20draft/Contents/users/nick.tex <==
% Nicolas: the below was merged



% \subsection{Ownership Claim of ML Models}
% \nick{This section is meant to describe and discuss the first component of our approach}

% The very first step to ML governance is to allow the actors to claim ownership of their ML models in a unforgeable and undeniable manner. This requires us to understand (a) what it means by owning a ML model, (b) why and how does adversary infringe the ownership, and (c) how can the model owners create claims that are robust against such infringement. 

% \subsubsection{ML Ownership}
% \paragraph{Functionality} As intellectual properties, the value of ML models comes from their functionalities (e.g., the ability to classify hand-written digits). This is also usually the target of ML model thieves. However, functionality is a very abstract concept. The model owner cannot frame the functionality of his/her model in a way that can be compared with others and used as a claim.

% \paragraph{Parameters} When people implement ML models, they usually use the word "model" to refer to the function composed of operations (i.e., architecture of the model) and parameters (e.g., weights and bias). With these pieces of information, one can obtain the model and use it for inference. The issue with this is that despite one set of parameters map to certain functionality, the reverse is not true: mapping from functionality to sets of parameters is 1-to-N (i.e., models with different parameters can have the same functionality). This leads to a line of attacks on model ownership: model extraction attacks~\cite{tramer2016stealing} which tries to steal the functionality of ML models but not the exact parameters (so it is harder to be caught). It will be discussed with more details in Section~\ref{sec:model_extractio}. 

% \paragraph{Training-time Information} This is intuited by the fact that all ML models are trained, and only the trainer of the model has done the computation on training. Since there exists some information during training that are not included in the final model for inference (e.g. intermediate checkpoints, training data, etc.), ownership claims can be made once we show an unforgeable connection between these information and the trained ML model. One representative example is the Proof-of-Learning~\cite{jia2021proof} which can be used as a claim robust against model extraction attacks. 
% However, here it is assumed the trainer of the model is the owner of the model, so there might be some improvements needed when this is not the case (e.g., the trainer sells the model to another party).


% \subsubsection{Infringement of ML Ownership}
% \label{sec:model_extraction}

% The attacks targeting ownership of ML models are known as model extraction attacks~\cite{tramer2016stealing}. \textit{Jagielski et al.} has categorized these attacks by their objectives~\cite{matthew2020high}. Some attacks are designed to achieve high \textit{accuracy}. This is usually the case when the adversary want to use ML models for their utility, but is unwilling/unable to collect training data and/or spend computational cost on training the models. Other attacks focus on high \textit{fidelity} (i.e., performing functionally similarly to the victim model). Such attacks can serve as a reconnaissance step to other attacks. For example, the adversary can create adversarial examples by the stolen copy to attack the victim model. These adversarial attacks can be more easily transferred to the victim model since the two models are functionally similar. 

% In this paper, we categorize model extraction attacks from another perspective: the threat model, i.e., what information the adversary has. Mostly the adversary has the black-box access to the victim model, i.e., he/she can query the model with inputs of his/her choice, and get predictions from the adversary. In addition, some work assumes access to unlabelled in-distribution data. Despite not many, there are also works not needing the query access, but some other information.

% \paragraph{Query Access}
% The most common threat model assumes the adversary having query access to the model. This is a realistic assumption since companies such as Google trains ML models and provides the access to them as a service. With this access, a naive adversary could query the model with infinite number of queries and eventually learn the exact behavior of the victim model. However, this naive approach is both financially and computationally costly, since querying victim model is not for free and training costs increases linearly with respect to amount of training data. Thus the works assuming this threat model usually aim to synthesizes data that reveals more information about the victim model to improve query efficiency. For example, Papernot et al.~\cite{papernot2017practical} proposes Jacobian-based Dataset Augmentation (JDBA) to find data that are near the decision boundaries. The adversary computes the direction to the decision boundaries by the extracted model's Jacobian matrix, and augment the synthesized data in that direction. Recently, Truong et al. introduced a GAN-like method named Data Free Model Extraction (DFME)~\cite{truong2021datafree}, which uses a generative model to generate data that the victim and extracted models have the largest disagreement on. In other words, JDBA maximizes information extracted from the victim model, whereas DFME maximize information extracted from the victim model that are not learned by the extracted model yet.

% \paragraph{Unlabelled In-distribution Data}
% In addition to the query access, some threat models also assume am unlabelled dataset from a similar distribution to the victim model's training dataset. This assumption is valid since online ML services usually state what tasks they could be used for (e.g. classifying digits). Then it is relatively easy for the adversary to collect some publicly available data related to the tasks (e.g. searching images of digits by Google). The goal of using such unlabelled data is also for query efficiency: the adversary wants to (a) select the data points that trains the extracted model faster by techniques such as Active Learning, as discussed by Chandrasekaran et al.~\cite{varun2020exploring}, and (b) leverage the rest of unlabelled data to help training by semi-supervised learning techniques such as MixMatch~\cite{berthelot2019mixmatch, matthew2020high}.

% \paragraph{Other Information}
% Batina et al. proposes a method named CSI-NN to extract DNNs under a very different threat model~\cite{batina2019csi}. The adversary takes advantage of side-channel information such as  timing and electromagnetic emanation and is shown to be capable of extracting the architecture and weight parameters of fully-connected DNNs or Convolutional Neural Networks.  


% \subsubsection{Protect ML Ownership}
% \label{sec:ownership_claim}
% Many researches have been done on how to protect ML models from the infringement of ownership. In high level, there are two streams of defenses. The model owners either (a) try to prevent the adversary from learning enough information to build an extracted model, or (b) keep records of training or embedding secrets into DNNs during training, and use them as ownership claims if the models are stolen.

% \paragraph{Restrict Information Leakage}
% As mentioned in Section~\ref{sec:model_extraction}, the adversary's goal is to extract the model with as less queries as possible. Thus the defender could aim the opposite: restrict the information leaked by each query so the adversary has to make more queries. This could be done by having less significant digits in the outputs, or even adding noise to the outputs of the models~\cite{tramer2016stealing}. However, this does not make model extraction impossible unless the outputs are completely random, in which case the model's utility is seriously harmed. 

% In stead of perturbing the outputs, other works first detect if a query may contribute to model extraction, and then either reject the query or even ban the user who submitted this query~\cite{}. This is intuited by the use of synthetic dataset in many attacks, which are likely to be from a different distribution than the training dataset. However, by construction, such defenses are vulnerable against attacks using unlabelled in-distribution data~\cite{}. 
 
% \paragraph{Ownership Claim}
% Ownership claims are usually based on objects constructed during training. Later if a model is stolen, the model owner is able to use the objects to claim the ownership of the stolen model. We categorize the claims into two types: (a) watermarking modifies the training process to embed a secret into the DNNs' functionality, whereas (b) dataset inference and Proof-of-Learning takes information during training but do not interfere with the training.

% \textbf{Watermarking} in ML is firstly introduced to protect the exact parameters of models~\cite{adi2018turning}. A watermarked DNN has special reaction to a set of designed triggers only known to the model owner. However, it has been shown to be vulnerable against model extraction attacks because they do not target the exact parameters. Jia et al.~\cite{jia2020entangled} indicate the reason is that the watermarked task (i.e. reacts differently to triggers) is disentangled from the model's primary task. The proposed solution is to modify the loss function to encourage similar set of neurons to handle both tasks. It is shown to be robust against model extraction attacks even if the adversary has the same amount of knowledge on the training distribution as the model trainer. However, it comes at the cost of slight utility drop.

% \textbf{Dataset Inference}~\cite{maini2021dataset} is intuited by the fact that the extracted model is either trained on data labelled by the victim model, or data from the training distribution of the victim model. Therefore, the model owners only need to keep their training data, and are able to claim ownership of a stolen model if it has very high confidence on data points that are in-distribution for the victim model. In other words, Dataset Inference is able to detect if two models are trained on the same dataset. Therefore, the drawback is that Dataset Inference cannot protect ownership of DNNs trained on public datasets. 
% \nick{@Mohammad you are the expert of this, feel free to modify/extend this paragraph}

% \textbf{Proof-of-Learning (PoL)}~\cite{jia2021proof} keeps records of not only training dataset, but also the orders they are fed into the model, intermediate checkpoints, hyperparameters, etc.--essentially everything needed to reproduce the training steps. Most of these are not included in the released DNN model so the adversary cannot reverse engineer them, while they are necessary in the process of training a randomly initialized model to the released version. The model owner will then be differentiated from the adversary by the capability of reproducing the victim/stolen model. The adversary is not capable to do so because the cumulative noise in DNN training and high dimensionality of the parameter space make it impossible to get the same model twice without intermediate training information. Despite requiring the most information and largest cost of claiming ownership (since reproducing a DNN is costly), PoL is the most trustworthy and hardest to countermeasure ownership claim.


==> Model%20Governance%20SoK%20draft/Contents/users/thudi+jia.tex <==
%was in accountability

\begin{enumerate}
\item general anomaly detection + prevention \adelin{My audio paper\cite{travers2021exploitability} and attacks on logging by surreptious AEs. add what varun said: so when you’re writing logging, you need to first establish (a) how generic logging can help ascertain internal leakage, and (b) what ML specific logging can help with}
\item extraction + how it can be prevented \adelin{Carlini on stateful detection of AEs at distillation time?} \nick{some stuff I wrote for the ownership may be useful for this item}
\item membership inference + how it can be prevented
\item model inversion \nick{I moved this in front of the data reconstruction attacks in FL since I feel it's more well-known and somewhat related to the next point. Feel free to change it back if you think that's better.}
\item data reconstruction attacks in FL settings through gradient observation
\item verified inference (i.e., is the output for inference correct) \nick{I described verified inference in section 6C. @Nicolas do you think it's better to leave it there or move to here?}
\item \url{https://medium.com/acing-ai/continuous-monitoring-for-data-projects-11fb1c00c7a4}
\end{enumerate}

\paragraph{MI and Prevention}\anvith{below is my blurb on it}

Membership inference was introduced by Shokri et al. \cite{shokri2017membership} as a means of predicting if a datapoint was used in the training set of a model; their initial attack showed that it was possible to train a classifier that could, if given the outputs (i.e., confidence vector) the victim model gave for a datapoint, discern if that datapoint was used in the training set or not. It was later shown that one only needs the confidence score on the specific label the victim model predicted to infer membership \cite{salem2018ml}, then that one in fact just needs the output label for membership inference \cite{choquette2021label}.

Various defences to membership inferences have been proposed \cite{shokri2017membership,nasr2018machine,jia2019memguard} broadly focusing on the problem of overfitting and robustness and how it relates to membership inference \cite{yeom2018privacy}, however most have been shown insufficient. For example, the Privacy Risk Score proposed by Song et al. \cite{song2019privacy} was shown to still strongly correlate with membership inference even when such defences were employed.

As of now the only defence that is guaranteed to work is training a differentially private model; Yeom et al. \cite{yeom2018privacy} showed how DP guarantees translate to bounds on membership inference accuracy, and Erlingsson et al. \cite{erlingsson2019we} provided even tighter bounds. \anvith{@Nicolas I mean it would be cool if I could also cite myself and say state of the art, but as the paper isn't public/finished I guess I can't}

\paragraph{Model Inversion}
Model inversion is another type of attacks that infringe privacy of training data of ML models. Being different from membership inference, instead of telling if a data point is part of the training dataset, model inversion aims to reconstruct data points that are likely from the training dataset~\cite{fredrikson2014privacy}. Fredrikson \etal~\cite{fredrikson2015model} first applied this attack to DNNs by taking the intuition that data from the training distribution usually can be classified by the model more confidently. In other words, DNNs usually overfit to training data. The reconstruction is done by optimizing an input with respect to the model's confidence (sometimes) following by sharpening and denoising. 

Yang \etal~\cite{yang2019neural} takes a very different path: an inversion model is trained to reconstruct the inputs to the victim model by using the victim model's prediction vectors. Training the inversion model is essentially transfer learning that transfers the knowledge of the victim model to an auto-encoder. Here the inversion model is the decoder, and the encoder is the victim model which is already trained and contains parameters not revealed to the adversary. It is worth to note that transfer learning is closely related to generalization--only a well-generalized model can be transferred well to a different task. Thus the authors argue instead of leveraging overfitting, this work is based on generalization and only generalized knowledge learned from the training dataset can be transferred to the inversion model. Zhang \etal~\cite{zhang2020the} also uses generative model for model inversion while GAN is used instead of auto-encoder. The victim model is used as a secondary discriminator--the generator is trained to maximize the confidence scores of the generated images.

While these two recent model inversion attacks are based on generative model, it is interesting that the most recent defending technique is also using generative model~\cite{yang2020defending}: an auto-encoder called purifier is trained to reconstruct the prediction vectors of both members and non-members of the training dataset so that the reconstructed predictions form a single cluster. Then an inversion model (e.g. the generator of Zhang \etal~\cite{zhang2020the}) is followed and the purifier is trained to minimize its performance. Now this is becoming an arms race between the adversary and the defender: the defender optimizes to minimize performance of the attacks, then the adversary can still use the defender's model as encoder/discriminator to implement more powerful attacks, and so on. 
\nick{it would actually be very interesting to see what will be left after a few rounds of this -- could it be data points that perfectly represent the task distribution since all overfitted information might be removed during this process}


\paragraph{Privacy Leakage in Collaborative/Federated Learning}
When the data contains private information and/or one individual's does not have enough data to train a model, collaborative learning can be used. Multiple participants get model parameters from the central server, computing and pushing the gradients on their own data to the server so that their own training data is not directly revealed to others. When it comes to federated learning~\cite{}, secure aggregation protocols are used to aggregate gradients of different participants. However, researches has been done to show that collaborative/federated learning is actually more vulnerable against privacy attacks such as membership inference and reconstruction. This is because in the collaborative learning setting, if the adversary is one participant or even the central server, he/she (a) has white-box access to the model (i.e. knows the exact parameters and architecture), (b) has some degree of knowledge about the gradient updates, and (c) is able to actively participate in the training process.

In the membership inference setting, Melis \etal\cite{melis2019exploiting} and later Nasr \etal~\cite{nasr2019comprehensive} make use of both gradients and embeddings outputed by intermediate hidden layers. Besides, Nasr \etal propose an autoencoder to learn what they called membership embedding, following by a cluster algorithm to deal with the unsupervised setting (i.e. when there is no labelled membership data). Note here the adversary does not need to know other participants' gradients since they have the model and data points that he/she want to know the membership of, which are enough for computing the gradients. It is observed that embeddings and gradients of later layers reveal more information about the training dataset. Nasr \etal~\cite{nasr2019comprehensive} also makes the observations that the magnitude of gradients with respect to a data point is dependent on the magnitude of loss computed on it, and loss of a non-member from the same distribution decreases gradually during training. Thus the adversary can purposely apply gradient ascent to increase the loss of a data point, and then a sudden decrease in its loss means this data point is a member.

The model inversion or reconstruction attacks in the federated learning setting can be also achieved by GAN-based methods, despite comparing to the centralized learning setting described in the previous section, the attacks here are usually adaptive. For example, Hitaj \etal~\cite{hitaj2017deep} proposes to use the collaboratively learned (victim) model as the discriminator and train a generator to reconstruct data belonging to one class of the training data, while also uses the generated data to train the victim model but with wrong labels. The authors claim by doing so the victim model needs to spend more effort on classifying data of the corresponding class, and thus learns and reveals more information about data from this class. Song and Wang \etal~\cite{wang2019beyond, song2020analyzing} further adapt the GAN-based attack to target user-level privacy, i.e., reconstructing a data point from a certain participant's training set. mGAN-AI is proposed in their more recent work~\cite{song2020analyzing}. The discriminator is trained on 3 loss functions for the following 3 tasks: (a) classification task (same as~\cite{hitaj2017deep}), (b) discriminating real/fake inputs so the generator can generate more realistic data, and (c) predicting if the inputs are from the victim participants or not. Besides, as response to anonymous gradient updates of federated learning, the authors introduced a siamese network to learn and differentiate representations of data from different participants.




==> Model%20Governance%20SoK%20draft/Contents/users/thudi_mi.tex <==
\paragraph{MI and Prevention
}\anvith{below is my blurb on it}

%Membership inference was introduced by Shokri \etal \cite{shokri2017membership} as a means of predicting if a datapoint was used in the training set of a model (using shadow model training). It was later shown that one only needs the confidence score on the specific label the victim model predicted to infer membership \cite{salem2018ml} (further supported by theory developed by Salayrolles \etal \cite{sablayrolles2019white}), then that one in fact just needs the output label for membership inference \cite{choquette2021label,li2020label}.

%Various defences to membership inferences have been proposed \cite{shokri2017membership,nasr2018machine,jia2019memguard} broadly focusing on the problem of overfitting and robustness and how it relates to membership inference \cite{yeom2018privacy}, however most have been shown insufficient. For example, the Privacy Risk Score proposed by Song \etal \cite{song2019privacy} was shown to still strongly correlate with membership inference even when such defences were employed. 

%As of now the only defence that is guaranteed to work is training a differentially private model; Yeom \etal \cite{yeom2018privacy} showed how DP guarantees translate to bounds on membership inference accuracy, and Erlingsson \etal \cite{erlingsson2019we} provided even tighter bounds. \anvith{@Nicolas I mean it would be cool if I could also cite myself and say state of the art, but as the paper isn't public/finished I guess I can't}

\anvith{@Varun below is newer version, above commented out is old version}

Membership inference was first introduced by Shokri \etal \cite{shokri2017membership} as a means of predicting if a datapoint was used in the training set of a model, where they proposed a black-box attack that just needed the outputs of a model on a datapoint to infer membership. Following this significant amount of work has gone into further improving, understanding and simplifying black-box attacks against membership inference \cite{salem2018ml,choquette2021label,song2019privacy,li2020label,jayaraman2020revisiting,truex2019demystifying}, and also proposing and discussing the utility of white-box attack which leverage any knowledge to be gained by a model's weights \cite{sablayrolles2019white,leino2020stolen} or even what membership information may be gained when the individual gradient updates are leaked or the adversary is allowed to manipulate the training algorithm \cite{song2017machine,nasr2019comprehensive}.

Various defences to membership inferences have been proposed \cite{shokri2017membership,jia2019memguard,nasr2018machine} broadly focusing on the problem of overfitting how it relates to membership inference \cite{yeom2018privacy}, but these are often insufficient to cover all possible attacks \cite{choquette2021label,song2019privacy,leino2020stolen}. In fact other aspects of a model, such as being robust to adversarial examples, have been shown to further exacerbate the ability for an adversary to employ MI \cite{song2019membership,song2019privacy}.

%amongst the specific scenario the attack is operating under, model type, 

The one known defence that is guaranteed to work is DP, and work has shown and further improved on bounds on MI accuracy given DP guarantees \cite{yeom2018privacy,erlingsson2019we,jayaraman2020revisiting}, but it should be noted that DP often comes with a undesirable trade-off with utility \cite{rahman2018membership} however future work may be able to improve this trade-off.


\paragraph{Model Inversion}
Model inversion is another type of attacks that infringe privacy of training data of ML models. Being different from membership inference, instead of telling if a data point is part of the training dataset, model inversion aims to reconstruct data points that are likely from the training dataset~\cite{fredrikson2014privacy}. Fredrikson \etal~\cite{fredrikson2015model} first applied this attack to DNNs by taking the intuition that data from the training distribution usually can be classified by the model more confidently. In other words, DNNs usually overfit to training data. The reconstruction is done by optimizing an input with respect to the model's confidence (sometimes) following by sharpening and denoising. 

Yang \etal~\cite{yang2019neural} takes a very different path: an inversion model is trained to reconstruct the inputs to the victim model by using the victim model's prediction vectors. Training the inversion model is essentially transfer learning that transfers the knowledge of the victim model to an auto-encoder. Here the inversion model is the decoder, and the encoder is the victim model which is already trained and contains parameters not revealed to the adversary. It is worth to note that transfer learning is closely related to generalization--only a well-generalized model can be transferred well to a different task. Thus the authors argue instead of leveraging overfitting, this work is based on generalization and only generalized knowledge learned from the training dataset can be transferred to the inversion model. Zhang \etal~\cite{zhang2020the} also uses generative model for model inversion while GAN is used instead of auto-encoder. The victim model is used as a secondary discriminator--the generator is trained to maximize the confidence scores of the generated images.

While these two recent model inversion attacks are based on generative model, it is interesting that the most recent defending technique is also using generative model~\cite{yang2020defending}: an auto-encoder called purifier is trained to reconstruct the prediction vectors of both members and non-members of the training dataset so that the reconstructed predictions form a single cluster. Then an inversion model (e.g. the generator of Zhang \etal~\cite{zhang2020the}) is followed and the purifier is trained to minimize its performance. Now this is becoming an arms race between the adversary and the defender: the defender optimizes to minimize performance of the attacks, then the adversary can still use the defender's model as encoder/discriminator to implement more powerful attacks, and so on. 
\nick{it would actually be very interesting to see what will be left after a few rounds of this -- could it be data points that perfectly represent the task distribution since all overfitted information might be removed during this process}


\paragraph{Privacy Leakage in Collaborative/Federated Learning}
When the data contains private information and/or one individual's does not have enough data to train a model, collaborative learning can be used. Multiple participants get model parameters from the central server, computing and pushing the gradients on their own data to the server so that their own training data is not directly revealed to others. When it comes to federated learning~\cite{konevcny2015federated}, secure aggregation protocols are used to aggregate gradients of different participants. However, researches has been done to show that collaborative/federated learning is actually more vulnerable against privacy attacks such as membership inference and reconstruction. This is because in the collaborative learning setting, if the adversary is one participant or even the central server, he/she (a) has white-box access to the model (i.e. knows the exact parameters and architecture), (b) has some degree of knowledge about the gradient updates, and (c) is able to actively participate in the training process.

In the membership inference setting, Melis \etal\cite{melis2019exploiting} and later Nasr \etal~\cite{nasr2019comprehensive} make use of both gradients and embeddings outputed by intermediate hidden layers. Besides, Nasr \etal propose an autoencoder to learn what they called membership embedding, following by a cluster algorithm to deal with the unsupervised setting (i.e. when there is no labelled membership data). Note here the adversary does not need to know other participants' gradients since they have the model and data points that he/she want to know the membership of, which are enough for computing the gradients. It is observed that embeddings and gradients of later layers reveal more information about the training dataset. Nasr \etal~\cite{nasr2019comprehensive} also makes the observations that the magnitude of gradients with respect to a data point is dependent on the magnitude of loss computed on it, and loss of a non-member from the same distribution decreases gradually during training. Thus the adversary can purposely apply gradient ascent to increase the loss of a data point, and then a sudden decrease in its loss means this data point is a member.

The model inversion or reconstruction attacks in the federated learning setting can be also achieved by GAN-based methods, despite comparing to the centralized learning setting described in the previous section, the attacks here are usually adaptive. For example, Hitaj \etal~\cite{hitaj2017deep} proposes to use the collaboratively learned (victim) model as the discriminator and train a generator to reconstruct data belonging to one class of the training data, while also uses the generated data to train the victim model but with wrong labels. The authors claim by doing so the victim model needs to spend more effort on classifying data of the corresponding class, and thus learns and reveals more information about data from this class. Song and Wang \etal~\cite{wang2019beyond, song2020analyzing} further adapt the GAN-based attack to target user-level privacy, i.e., reconstructing a data point from a certain participant's training set. mGAN-AI is proposed in their more recent work~\cite{song2020analyzing}. The discriminator is trained on 3 loss functions for the following 3 tasks: (a) classification task (same as~\cite{hitaj2017deep}), (b) discriminating real/fake inputs so the generator can generate more realistic data, and (c) predicting if the inputs are from the victim participants or not. Besides, as response to anonymous gradient updates of federated learning, the authors introduced a siamese network to learn and differentiate representations of data from different participants.



==> Model%20Governance%20SoK%20draft/Contents/users/varun_accountability_orig.tex <==
% \newpage
\section{Holding ML Principals Accountable}
\label{sec:accountability}

Identities, as established in \S~\ref{sec:ownership}, serve multiple purposes~\cite{bishop}; one of them being {\em accountability}. In conjunction with traditional access control mechanisms, the notion of identity provided by data and  model ownership in the context of ML allows us to establish the responsibility of principals interacting with a ML system. This is defined as accountability, and is different from the {\em process} of ascertaining accountability which we define as {\em attribution}. Indeed, accountability is essential when ML models produce {\em undesirable} behaviors (\ie failures) such as the ones discussed in \S~\ref{}. Some of these failure modes will be known and need to be attributed to a principal (we outline these earlier in \S~\ref{}). This is similar to how malware analysis will seek to identify whether a malware originated from a state actor or not. Principals held responsible could be the model owner, but also end users (\eg if they are attempting to steal a model, or to have it produce an incorrect prediction with an adversarial example). Other failure modes of the model may be initially unknown but uncovered by external scrutiny of a ML pipeline: \eg by a regulator through an auditing process discussed later in this section. 


% To better understand accountability and attribution, we begin by discussing the failure modes associated with ML models.


% In the following, we discuss two classes of failures. First, failures that are already known and which we would like to attribute to a specific principal (\eg the end user of a generative ML model is held responsible for a deepfake image found on the Internet). Second, we discuss progress in auditing ML systems, which will enable a party who is not the model owner (\eg a regulator) to identify possible model failures not necessarily known or discovered ``by chance'' by the model's end users.

% \nicolas{an important observation we need to make is that model owners are not always the ones that need to be held accountable - for instance in deepfakes the GAN may have been created for good but used for bad }\adelin{This to me is attribution while the above is accountability. I would rather say that attribution/accountability are two facets of the same coin. When we try to tie a malicious actor to the system they used it's attribution. When we try to enforce good practices in governance (ie from semi-trustworthy model owners), the same techniques are called accountability. Said in another way: accountability is proactive internal audit/goodwill, while attribution is an external process.}

% \newpage
% \section{Monitoring}
\iffalse

\subsection{Anomalous Events}

Recall that accountability is required when an anomalous event occurs. These events can broadly be classified as {\em failures}, or {\em threats}. Failure events are those which result in deviant model performance (\eg poor generalization); such events violate the integrity of the model. Threats are those events which result in learning sensitive/proprietary information about the model or the data used to train it; such events violate the confidentiality of the model (and training data). We first discuss failure events.

%\noindent{\bf Failures}

%\vspace{1mm}
\noindent{\bf Known Failures} ML models are known to be brittle; data used to train models should possess specific properties and must be processed in specific ways to enable effective training (\S~\ref{subsec:data_ownership}). This is done to ensure that models are resilient to {\em outliers} (data-points that are outside the range of those expected); since outliers are not representative of the underlying data distribution, any model learnt using this data will not be ideal~\cite{gudivada2017data,cortes1995limits}. Another problem that one should be aware of is that of {\em concept drifts} (where the distribution of data changes over time). \anvith{following is new and feels very forced, in particular the last citation, I think it was before without it (we talk about this stuff anyways later)} Different approaches have been proposed for dealing with learning under such situations: Lu \etal \cite{lu2018learning} reviewed past approaches, and new approaches have worked on understanding how better to adapt \cite{kumar2020understanding}. \varun{loads of relevant papers: \url{https://cs.stanford.edu/~pliang/papers/}; also check out ludwig schmidt's work}. Collectively, both these issues result in the model being unable to generalize. \varun{@anvith: can you use google doc to add papers from percy + ludwig which are relevant to this topic?} \anvith{added a couple papers on concept drift, I only found two relevant papers from percy liang which I added to the google sheet (but I could be slighlty blind), and from that I think only one really fits with the discussion and even then not really}

%\adelin{how are induced failures not "known"?} 
%\vspace{1mm}
\noindent{\bf Adversary-induced Failures} This class of failures stems from adversarial interaction \ie the adversary maliciously modifies data-points to cause negative effects. Collectively, these attacks impact the {\em integrity} of the trained model: the outputs it produce can not be trusted.

%\anvith{I guess below is not specific to DNNs?} \anvith{not too sure for some of these citations/statements leaving this for later}

At training time, adversaries incorporate data poisons (which are specifically perturbed data-points) which result in poor generalization (\ie indiscriminate poisoning attacks~\cite{munoz2017towards}), or targeted misclassification (\ie targeted poisoning attacks~\cite{munoz2017towards}). Poisoning adversaries can assume that the data collector uses the labels provided with the poisons~\cite{}, or can also specify their own labels~\cite{}. The former is known to be ineffective for heavily parameterized models~\cite{}, while the latter is effective across the spectrum. Poisoning is effective across a range of learning paradigms~\cite{} (\varun{include latest carlini ssl work}), and across different threat models~\cite{}. Poisoning attacks are fundamentally different from backdoors; in the latter, a specific {\em trigger} pattern induces a misclassification, and can be added to {\em any input} whilst poisoning ensures misclassification of inputs belonging to a particular class.

At inference time, adversaries can strategically modify inputs (whilst ensuring that they are indistinguishable from their benign counterparts). This induces a misclassification~\cite{szegedy2013intriguing}. These evasion attacks are known to be effective across a wide range of hypothesis classes~\cite{szegedy2013intriguing,goodfellow20vernekar2019analysisexplaining,shafahi2018adversarial,papernot2016limitations}, and learning paradigms~\cite{} \anvith{not too clear what you mean by learning paradigms, like unsupervised learning?}\varun{or re-inforcement learning, online learning etc.}. While it was initially demonstrated for vision~\cite{szegedy2013intriguing}, evasion has been demonstrated for a wide variety of domains including audio~\cite{carlini2018audio,yakura2018robust,qin2019imperceptible} and text~\cite{ebrahimi2017hotflip,alzantot2018generating,garg2020bae,zhao2017generating}. Research has demonstrated that such attacks can be physically realized~\cite{kurakin2016adversarial,yakura2018robust}\varun{add slap attack from usenix 2021}. Additionally, research has also demonstrated that samples generated for evasion preserve input semantics~\cite{qin2019imperceptible,alzantot2018generating} \varun{add papers with sanjit seshia + chandrasekaran and seshia + dreossi + jha; also bo li has a bunch of papers to generate "semantic adversarial examples"}.

%\adelin{What's the relationship with accountability? I can see a relationship with attribution as in: how do we attribute these attacks to the corresponding threat actor but none to accountability.}

%\vspace{1mm}
\noindent{\bf Human Failures} \varun{what was i thinking when i wrote this?}

%\noindent{\bf Threats}

We now focus on threats. Model extraction attacks are those that violate parameter confidentiality, and are discussed in detail in \S~\ref{subsec:model_ownership}. Other threats are discussed below. 

%\vspace{1mm}
\noindent{\bf Membership Inference} In a membership inference attack (MIA), an adversary wishes to determine if a given data-point was used to train the model. In the original attack, adversaries were assumed to have access to confidence information from the black-box model~\cite{shokri2017membership} \anvith{which was shown sufficient to determine membership}. \anvith{can remove following line, doesn't feel necessary} The authors noticed that the model was more confident when processing data it was trained with. Following this, a large volume of research has further improved (and simplified) black-box attacks \varun{@Anv T: Simplify how?}\anvith{gave suggesting for previous sentence, for following could combine white-box and gradient into a blanket statement of "more information to the adversary"; for adversarial robustness we could just drop it and mention it somewhere else about the tradeoff between different metrics}~\cite{salem2018ml,choquette2021label,song2019privacy,li2020label,jayaraman2020revisiting,truex2019demystifying}. Research has also demonstrated effective white-box attacks which further leverage information held in model parameters~\cite{sablayrolles2019white,leino2020stolen,song2017machine,nasr2019comprehensive}, or gradient updates~\cite{melis2019exploiting}. Research has also demonstrated that adversarial robustness exacerbates the success of membership inference~\cite{song2019membership,song2019privacy}, though the reasons for this are unclear \anvith{disagree with last claim, the motivation was that having trained to be adversarially robust means training on many similar datapoints and thus strengthening the signal of that datapoint (motivation the authors stated) unless I'm missing something}.

Yeom \etal~\cite{yeom2018privacy} draw the connection between the efficacy of MIA and overfitting. Based on this insight, various (now broken) defences have been proposed~\cite{shokri2017membership,jia2019memguard,nasr2018machine}. For example the privacy risk score proposed by Song \etal \cite{song2021systematic} was shown to still strongly correlate with membership even after various defences were employed. \varun{add a line on why these defenses are broken}\anvith{added PRS as an example of attack that breaks them} However, Yeom \etal~\cite{yeom2018privacy} note that training the model to obtain DP also reduces an MIA's efficacy; these authors and others~\cite{erlingsson2019we,jayaraman2020revisiting,sablayrolles2019white} draw theoretical connections between the efficacy of the attack and the privacy budget ($\varepsilon$) (in particular bounding the efficacy of such an attack). Thus, as of now, the one guaranteed defence against an MIA is DP. \varun{takeaway of this connection?}\anvith{added, is that this shows DP as the main valid defence}. \varun{missing discussion around privacy risk score}\anvith{added in discussion about why defences broken}

%\vspace{1mm}
\noindent{\bf Attribute Inference} Attribute inference attacks (AIA) are those where an adversary attempts to impute missing values in a partially populated record using access to a ML model. \varun{talk about this @AT, @HJ} \anvith{added one paper to google sheets, seems that this is in general related to data reconstruction}
%https://arxiv.org/abs/1805.04810 --> use this paper

%\vspace{1mm}
\noindent{\bf Data Reconstruction} Model inversion attacks aim to reconstruct data-points that are {\em likely} from the training dataset. In the classification setting, Fredrikson \etal~\cite{fredrikson2015model} achieve this using confidence information from the prediction vectors (based on the same overfitting assumption made in MIA). With a similar intuition, Yang \etal~\cite{yang2019neural} use an auto-encoder to reconstruct the input from the confidence vectors, while Zhang \etal~\cite{zhang2020the} use GANs to aid reconstruction. \varun{only 3 attacks for model inversion?} Note that the aforementioned attacks are possible when the model is fully trained. More recent attacks (applicable in distributed training regimes, such as federated learning~\cite{konevcny2015federated}\footnote{Federated learning is a paradigm where multiple clients jointly learn a model by training a local model on their private datasets and sharing gradients which are aggregated at a central entity.}) enable successful reconstruction from gradients~\cite{geiping2020inverting,nasr2019comprehensive,melis2019exploiting, hitaj2017deep,wang2019beyond, song2020analyzing}.\varun{more papers can be added here}  

DP training is proposed as a technique to defend against data reconstruction. In the federated learning setting, this has been studied and deemed effective~\cite{}; the same can be observed for model inversion attacks~\cite{}. 

\varun{currently missing attacks on fairness}

\fi

\subsection{Attribution}
\label{subsec:attribution}

Recall that we define attribution as the process/mechanism used to identify principals responsible for model failures. Detecting known failure events is a well studied problem in ML literature and in what follows we discuss detection of the failures discussed earlier in \S~\ref{}. \nicolas{there is a mismatch right now - attribution is not just detection of failure, it is also telling who is  responsible for the failure}


% \begin{enumerate}
% \item discussion around outlier detection
% \item concept drift detection
% \item detection of adversarial examples (adelin's work for example) \nick{currently working on this}
% \item detection of poisoning/backdooring attacks (sanghyun hong + nicolas papernot)

% \nick{the two items below is pretty much the same as "Assurance to Model Owners" in assurance.tex}
% \item detecting model extraction (lucy's work)
% \item add a sentence stating that it's hard to detect inference + reconstruction as it is passive
% \end{enumerate}

\vspace{0.5mm}
\noindent{\bf Outliers:} Outlier detection for DNNs at test time was first introduced by Hendrycks \etal \cite{hendrycks2016baseline} where they showed that thresholding outputs provided a sufficient baseline as in-distribution and out-of-distribution points often yielded different outputs. Following this considerable work has gone into making a DNNs predictions on OOD examples and in distributions example more different \cite{meinke2019towards,liang2017enhancing,lee2017training,lee2018simple,hein2019relu,hendrycks2018deep,ren2019likelihood,lakshminarayanan2016simple,vyas2018out}, often by making the predictions on OOD examples more uniform (\ie no high confidences in contrast to in-distribution points) \cite{meinke2019towards,lee2017training,hein2019relu,hendrycks2018deep,lakshminarayanan2016simple,vyas2018out} and/or introducing other metrics on the outputs of DNNs under which OOD and in distribution are more seperated \cite{liang2017enhancing,lee2018simple,ren2019likelihood,serra2019input,hsu2020generalized}. Alternatively, others have considered training models to also output a confidence score associated to their prediction (or make the predictions explicitly confidence scores) which can be use to tell how likely the input was out of distribution \cite{devries2018learning,vernekar2019analysis,malinin2018predictive} or introduce another confidence metric based on other information such as the internal representations of the model, distribution of point in the training set, alongside statistical tests to understand how related an input is to what was seen in the training set \cite{raghuram2021general,sastry2019detecting,jiang2018trust,papernot2018deep,jha2019attribution}.

All these have seen varying degrees of success, however there are yet no formal gurantees for a method to always work, with their being results showing why output based methods won't always work \cite{hein2019relu,vernekar2019analysis} (though more recently Meinke \etal \cite{meinke2019towards} analytically showed that their approach should work better than previous approaches).



%The need for outlier detection is prevalent whenever out-of-distribution inputs to a system can cause significant harm, and thus various general statistical methods have been used for the task of discerning whether a datapoint belongs to a distribution or not \cite{barnett1984outliers}. \anvith{maybe give some stats based examples} Nevertheless alternatives more tailored to the context of ML datasets (and the high dimensionality) have also been proposed: Escalante \etal \cite{escalante2005comparison} give a comparison of different approaches for outlier detection in ML datasets.\anvith{maybe give some examples not mentioned above}

\noindent{\bf Concept Drift:} Lu \etal \cite{lu2018learning} summarized much of the past work of concept drift detection for ML into three broad themes of Error Rate based detection (which use a model's deteriorating performance as a base indicator of shifts) \cite{gama2004learning,gama2006learning,baena2006early,frias2014online,liu2017fuzzy,xu2017dynamic,huang2006extreme,ross2012exponentially,nishida2007detecting,bifet2007learning,bifet2009adaptive,bifet2009improving,bifet2009new,gomes2017adaptive}, Data Distribution based detection (which try and discern differences in the distribution of previous and new inputs) \cite{kifer2004detecting,dasu2006information,song2007statistical,lu2016concept,shao2014prototype,qahtan2015pca,gu2016concept,bu2016pdf,bu2017incremental,liu2017regional}, and Multiple Hypothesis Test Drift Detection (which differ from the previous two by utilizing more than one test to discern drift) \cite{alippi2012just,alippi2013just,wang2015concept,zhang2017three,du2015selective,maciel2015lightweight,alippi2016hierarchical,yu2017concept,raza2015ewma,yu2018request}. More recent work has looked at detecting drift in specific features \cite{kulinski2021feature}, and improving data distribution based detection \cite{yang2021cade}.

%Similar to outlier detection, concept drift detection is about understanding when the past dataset used to train a model is now an outlier to the current dataset the model experiences. One can take different approaches to detecting whether concept drift has occured, whether it is by looking at how the accuracy of a model changes over time or by running statistical test not too dissimilar than those for outlier detection; Lu \etal \cite{lu2018learning} describe and compare in detail different approaches relevant for ML.




\noindent{\bf Adversarial Examples:} Adversarial examples are data points that are slightly perturbed from natural data, and could cause ML models to misclassify~\cite{goodfellow2014explaining}. The defenses for adversarial examples can be categorized into training-time and inference-time defenses. The former usually aims to make the model to correctly classify adversarial examples (\eg adversarial training~\cite{}), whereas the latter tries to detect adversarial examples and reject them. We will discuss the inference-time defenses in this section.

In high level, all detection techniques can be seen to have two stages: preprocessing and detecting. The defenders would first preprocess the inputs in a way that adversarial examples can be more easily differentiated from natural data. This could be done by taking the representations in hidden layer~\cite{gong2017adversarial, lu2017safetynet, wong2018provable, Feinman2017DetectingAS}, transforming the inputs~\cite{tian2018detecting, xu2018feature, roth2019the}, applying dimensionality reduction techniques~\cite{li2017adversarial, hendrycks2017early, bhagoji2017dimensionality}, or even modeling the inputs from steganalysis point of view~\cite{liu2019detection}. Then in the detecting stage, the most commonly used techniques include trained classifiers (supervised)~\cite{hendrik2017on,grosse2017statistical,gong2017adversarial,lu2017safetynet,tian2018detecting,li2017adversarial,bhagoji2017dimensionality}, statistical tests to distinguish distributions of adversarial and natural examples (unsupervised)~\cite{grosse2017statistical,hendrycks2017early,Feinman2017DetectingAS,liu2019detection,roth2019the}, and agreement of predictions on multiple inputs where some of them may be adversarial~\cite{tian2018detecting,xu2018feature,wong2018provable}. It is worth to note that most of these defenses do not require significant change in the training procedures so they are not mutually exclusive. Thus in practice, if affordable, a defender may want to use an ensemble of several detection mechanisms.

Carlini \etal~\cite{carlini2017adversarial} has shown that some of the detecting methods can be bypassed by stronger attacks and identifying intrinsic properties that differentiate adversarial examples from natural data remains as an open problem. More recent works~\cite{lu2017safetynet,tian2018detecting,xu2018feature,liu2019detection,roth2019the,wong2018provable} are demonstrated to be robust against stronger and stronger attacks, but it is still unclear if there exists an optimal defense or this is just another army race between the defender and the adversary.

% binary classifieclear if r on inputs~\cite{hen, but it is still undrik2017on}
% N+1 class + Maximum Mean Discrepancy (MMD) test~\cite{grosse2017statistical}
% binary classifier on hidden layers~\cite{gong2017adversarial}

% safetynet: binary detector on discrete generated by quantizing activations of hidden layers~\cite{lu2017safetynet}
% binary classifier on predictions of several transformed images~\cite{tian2018detecting}

% PCA + cascade classifier~\cite{li2017adversarial}
% adversarial examples place a higher weight on the larger principal components than natural images~\cite{hendrycks2017early}
% PCA + binary classifier~\cite{bhagoji2017dimensionality}

% Feature squeezing: reduce degree of freedom at input space and check the difference between the predictions on original and reduced images~\cite{xu2018feature}

% distribution of outputs of last hidden layer~\cite{Feinman2017DetectingAS}

% detect steganography: dependency/differences between adjacent pixels modeled as a higher order Markov chain~\cite{liu2019detection}
% adding noise to adversarial examples incurs greater change in the logits~\cite{roth2019the}

% add outbound to the logit and assert the prediction doesn't change, \ie filter out any points that's too close to decision boundaries~\cite{wong2018provable}

\noindent{\bf Data Poisoning:} Data poisoning attacks~\cite{Rubinstein2009antidote,Shafahi2018poison,Jagielski2018Manipulating,liu2017neural,Chen2017TargetedBA} target the integrity of ML models. The adversary insert a small set of carefully crafted data to the training dataset, and aim to influence the model's performance. A special case of data poisoning is backdoor attacks~\cite{Shafahi2018poison,liu2017neural,Chen2017TargetedBA}, where at inference time the adversary would react abnormally to data points containing a designed trigger (the reaction is also designed by the adversary, \eg misclassify to a certain class).

Since the goal is attribution, we only focus on detection techniques for data poisoning in this section. These techniques either aim to (a) detect if there are poisoned data in the training dataset, or (b) detect if a trained model is poisoned. To the best of our knowledge, the only techniques belongs to the former are using anomaly/outlier detection ~\cite{liu2017neural,Chen2017TargetedBA}, but their performance is not too great. Most researches in this field prefer the latter. Given a trained model, people try to find the relation between poisoned data and special behaviors in the representation space (or activations of hidden layers) ~\cite{tran2018spectral,chen2019detecting,liu2019abs}, or investigate the gradients (gradients of poisoned data tend to have different magnitude and orientation~\cite{Hong2020on}). Some other works exploit more abstract behavior of ML model. Kolouri \etal~\cite{kolouri2020universal} constructs images called Universal Litmus Patterns and trains a detector on the model's output on these images to detect poisoned model. Wang \etal~\cite{wang2019neural} and Chen \etal~\cite{chen2019deepinspect} observed the change in decision boundaries due to data poisoning and proposed detection mechanisms accordingly. 

Despite most of the techniques for detecting poisoned models are empirically shown to be successful, they do not prevent the poisoned data to be used for training--this makes it harder to certify that the effect of backdoors are completely removed. Thus we want to ask the following question: is it possible to introduce techniques (other than anomaly detection) that can detect poisoned data before training? If not, can we introduce a more formal metric to quantify the effects of data poisong rather than sorely relying on classification accuracy?


\noindent{\bf Detection of Model Extractions}
Model extraction attacks the confidentiality of the ML models as described in \S~\ref{subsec:model_ownership}. Here we foucs on detecting/defending model extraction attacks during inference time. To do so, the high level idea is to restrict the amount of information about the model leaked to the adversary. This can be done by first identifying special characteristics of queries contributing to model extraction. And then depending on how confident the service provider is about the the identification, he/she can either (a) if confident enough, reject all such queries, or (b) with less confidence, adding perturbations to the predictions to these queries to give less or even wrong information about the model to the adversary. PRADA proposed by Juuti \etal~\cite{juuti2019prada} falls into the former, where they identify adversary by the distribution of distances between queries. This is intuited by the fact that synthetic queries usually do not form an normal distribution. In the second category, Sanjay \etal~\cite{kariyappa2020defending} purposely give incorrect predictions to out-of-distribution queries; Zheng \etal~\cite{zheng2019bdpl} protect data points near the decision boundaries by differential privacy since they suspect the model extraction adversary are more interested in such points; and Tribhuvanesh \etal~\cite{tribhuvanesh2020prediction} outputs predictions (usually with correct top-1 labels) that try the best to mislead gradient-based optimization algorithms (\eg SGD) so it becomes hard for the adversary to train an extracted model. It is worth to note that the two categories are not mutually exclusive. For example, if PRADA~\cite{juuti2019prada} detects user that is likely to be an adversary, instead of rejecting all his/her queries, the service provider can also use Tribhuvanesh \etal~\cite{tribhuvanesh2020prediction}'s work to confuse the adversary's stolen model since some information about the victim model may be already extracted before the detection. Despite these methods work well against most model extraction attacks, there is still an exception: if an adversary leverages public data instead of synthetic data and use the victim model as an labelling oracle (\ie only using the top-1 prediction), none of the above defenses would work without suffering significant accuracy drop. The adversary does need to spend much higher cost in this scenario, but they still benefit from the extraction since it is still cheaper than collect labelled data by themselves, and now they have white-access to the stolen model which enabling them to benefit by applying other types of attacks. Thus the open question here is if it is possible to defend this most powerful extraction attacks (\eg by quantifying the information leakage and stop responding to a user if certain threshold is reached \nick{not sure if we should have this example--feel free to remove it if it leaks too much info about lucy's work}), and if not, what degree of attribution should/can be required by the model owners? 

\noindent{\bf Detection of Privacy Attacks}
Membership inference and model inversion both target the confidentiality of the ML model's training data. We have discussed these attacks and corresponding defenses in \S~\ref{}. However, unlike model extraction attacks, there currently does not exist any inference-time detection for these two privacy attacks, \eg algorithms detecting suspicious queries that may contribute to these attacks. This may be a result that (a) the number of queries required by the privacy attacks is significantly less than what required by model extraction attacks, since the information of a data point is less than the information of the entire model; and (b) the characteristics of queries for privacy attacks are not well-studied. Thus it remains an open problem on inventing test-time defenses that can be used to achieve attribution, otherwise the defenses have to be implemented at training time.

\noindent{\bf Detection of generative modeling} Generative modeling has revolutionised content generation routines~\cite{}, bringing a myriad of problems to the table. Recent work has highlighted that GAN produced content has been used in information campaigns~\cite{},

At the same time, training data of generative can compromise confidentiality of underlying training data~\cite{}. 

Detection of bias with GANs (recent twitter competition)


\input{Contents/users/adelin}

\subsection{Accountability}

\varun{make blanket statement about accountability here (\ie it is model owner's problem if any of these issues occur) + discuss (a) baiwu’s work here, and (b) @Nick Jia did some research from the policy/legal side (recall our discussion of smart cars + who is responsible if it crashes) — we can add this too. we can phrase this as a broader open question that the community should address}

==> Model%20Governance%20SoK%20draft/macros.tex <==
\usepackage{cite}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{bbold}
\usepackage{soul}
\usepackage{booktabs}
\usepackage{float}
\usepackage{tcolorbox}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{mathrsfs}
\usepackage{hyperref}
\usepackage{url}
\usepackage[inline]{enumitem}

\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc, babel, decorations.text, fit}
\usetikzlibrary{positioning, intersections}
\usepgflibrary{shapes.arrows}

\usepackage{pgfplots}
\usepackage{pgfplots,pgfplotstable}
%\pgfplotsset{compat=1.16} Nicolas disabled this to work remotely through git but feel free to renable

\usepackage{amsthm}
\usepackage{algorithm,algpseudocode}
\usepackage{dsfont}
\usepackage{subfig}
\usepackage{mwe}
\usepackage{wrapfig}
\usepackage{lipsum}
\usepackage{framed}
\usepackage{svg}
\usepackage{multirow}
%\usepackage{subcaption}
\usepackage{soul}
\usepackage{wasysym}

\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{indentfirst}
%\usepackage{booktabs}
\usepackage[nottoc]{tocbibind}
\usepackage[colorinlistoftodos,disable]{todonotes}
%\usepackage{xcolor} 
%\usepackage{float}
%\usepackage{hyperref}
% \usepackage{amssymb}
% \usepackage{amsmath}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}


% \usepackage{caption}
% \captionsetup[subfigure]{labelformat=parens,labelsep=space,font=small}
% \usepackage{subfig}

% \newcommand{\chris}[1]{\textcolor{red}{Chris: #1}}
% \newcommand{\lucas}[1]{\textcolor{orange}{Lucas: #1}}
% \newcommand{\nick}[1]{\textcolor{olive}{Nick: #1}}
% \newcommand{\adelin}[1]{\textcolor{purple}{Adelin: #1}}
% \newcommand{\nicolas}[1]{\textcolor{cyan}{Nicolas: #1}}
% \newcommand{\todo}[1]{\textcolor{purple}{TO DO: #1}}
% \newcommand{\varun}[1]{\textcolor{blue}{Varun: #1}}

% COMMENTS
\ifdraft
\newcommand{\anvith}[1]{\textcolor{blue}{Anvith: #1}}
\newcommand{\mohammad}[1]{\textcolor{teal}{MY: #1}}
\newcommand{\nick}[1]{\textcolor{olive}{HJ: #1}}
\newcommand{\adelin}[1]{\textcolor{purple}{AT: #1}}
\newcommand{\nicolas}[1]{\textcolor{red}{Nicolas: #1}}
% \newcommand{\todo}[1]{\textcolor{red}{TO DO: #1}}
\newcommand{\varun}[1]{\textcolor{red}{Varun: #1}}
\newcommand{\jonas}[1]{\textcolor{orange}{Jonas: #1}}
\newcommand{\new}[1]{\textcolor{black}{#1}}
\newcommand{\roei}[1]{\textcolor{purple}{Roei: #1}}
\else
\newcommand{\anvith}[1]{}
\newcommand{\mohammad}[1]{}
\newcommand{\nick}[1]{}
\newcommand{\adelin}[1]{}
\newcommand{\nicolas}[1]{}
% \newcommand{\todo}[1]{}
\newcommand{\varun}[1]{}
\newcommand{\jonas}[1]{}
\newcommand{\new}[1]{}
\newcommand{\roei}[1]{}
\fi


\newcommand{\ie}{\textit{i.e.,}\@\xspace}
\newcommand{\eg}{\textit{e.g.,}\@\xspace}
\newcommand{\etal}{\textit{et al.}\@\xspace}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\SISA}{\textbf{SISA} training\xspace}
\newcommand{\model}{M\xspace}
\newcommand{\weights}{\textbf{w}\xspace}
\newcommand{\graybox}[1]{\tikz[baseline=(X.base)]\node [draw=black,fill=gray!40,semithick,rectangle,inner sep=2pt, rounded corners=3pt] (X) {#1};}


\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


==> Model%20Governance%20SoK%20draft/tikz_preamble.tex <==
%!TeX root = game.tex
\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc, babel, decorations.text}
\usetikzlibrary{positioning}
\usepgflibrary{shapes.arrows}
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.text}    
\usetikzlibrary{intersections}

\makeatletter
\tikzset{arc style/.initial={}}
\pgfdeclareshape{half circle}{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]

  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{east}
  % can add more anchors if necessary

  \inheritbackgroundpath[from=circle]

  \beforebackgroundpath{
    % get and set options
    \pgfkeys{/tikz/arc style/.get=\tmp}
    \expandafter\tikzset\expandafter{\tmp}
    \tikz@options

    % get radius length and center coordinates
    \radius \pgf@xa=\pgf@x
    \centerpoint \pgf@xb=\pgf@x \pgf@yb=\pgf@y

    % draw arc
    \advance\pgf@yb by \pgf@xa
    \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpatharc{90}{-90}{\pgf@xa}
    % change the last line to the following line if you want the half circle rotated in the other direction
    % \pgfpatharc{90}{270}{\pgf@xa}

    % \pgfusepath{draw}
    \pgfusepath{fill}
  }
}
\makeatother

\newcommand*\emptycirc[1][1ex]{\tikz\draw[thick] (0,0) circle (#1);} 
\newcommand*\halfcirc[1][1ex]{%
  \begin{tikzpicture}
  \draw[fill] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
  \draw[thick] (0,0) circle (#1);
  \end{tikzpicture}}
\newcommand*\fullcirc[1][1ex]{\tikz\fill (0,0) circle (#1);} 

\newcommand\citefull[1]{
\begin{tikzpicture}
  \node[draw=gray, thick, circle, fill=black!70, opacity=0.2, text opacity=1, draw opacity=1, inner sep=0,outer sep=0] (0,0) {\cite{#1}};
  \end{tikzpicture}
}
\newcommand\citehalf[1]{
\begin{tikzpicture}
%  \node[draw, thick, circle, opacity=0.2, text opacity=1, text align=center, inner sep=0,outer sep=0] (0,0) {\cite{#1}};

  \node[
    half circle,
    % fill=gray!20,  % can fill the circle if needed
    % minimum width=2cm,
    inner sep=0,outer sep=0,
    fill=black, 
    opacity=0.1,
    text opacity=1,
    draw opacity=1,
    draw=gray,
    thick,
    arc style={thick}
    ] {\cite{#1}};
  \end{tikzpicture}}

\newcommand{\decision}[7][]{
	%	#1: action-set-label
	%	#2: actor-label
	%	#3: point-x
	%	#4: point-y
	%	#5: radius
	%	#6: degree
	%   #7: spacing two action-set-label
	%	\begin{tikzpicture}
	\draw[thick] ([shift=(-1*#6:#5)]#3,#4) arc (-1*#6:#6:#5);	
	\draw[] (#3,#4) -- ++(-1*#6:#5) (#3, #4) -- ++(#6:#5);
	\node(regulator)[circle, fill=black, label={[font=\footnotesize, align=center, rounded corners, fill=white, fill opacity=0.7, text opacity=1]#2}] at (#3, #4) {};
	\node at (#3, #4 + #7) {\scriptsize #1};
	%		\draw[thick] (#2,#3) -- ++(-44.83:#4 +.424cm) (#2, #3) -- ++(44.83:#4 + 0.424cm);
	%		\draw[thick] (#2+#4,#3) [partial ellipse=-90:90:0.3cm and #4];
	%	\end{tikzpicture}
}
\newcommand{\decisionD}[7][{{"Action 1"}}]{
	%   #1: action-labels
	%	#2: actor-label
	%	#3: point-x
	%	#4: point-y
	%	#5: radius
	%	#6: degree
	%	#7: number of actions
	\foreach \x in {0,...,#7}
		\draw (#3,#4) -- ++( +{\x} * #6/#7 - #6/2:#5) node [midway, below, sloped] {\scriptsize \pgfmathparse{#1[\x]}\pgfmathresult};
	\node(regulator)[circle, fill=black, label={[font=\footnotesize, align=center, rounded corners, fill=white, fill opacity=0.7, text opacity=1]#2}] at (#3, #4) {};
}

\tikzset{
	partial ellipse/.style args={#1:#2:#3}{
		insert path={+ (#1:#3) arc (#1:#2:#3)}
	}
}

%\tikzset{
%	decision/.style={
%		path picture={
%			\node[circle, fill=black, label={[xshift=-0.5cm]\decision@actor}] at (0, 0) {};
%			%	\draw[thick] ([shift=(-30:1cm)]0,0) arc (-30:+30:1cm);
%			\draw[thick] (0,0) -- ++(-44.83:1.424cm) (0, 0) -- ++(44.83:1.424cm);
%			\draw[thick] (1,0) [partial ellipse=-90:90:0.3cm and 1cm];
%		},
%	},
%decision actor/.store in=\decision@actor,
%decision actor=Actor,
%}
